ddml: Double/debiased machine learning in Stata

We introduce the package ddml for Double/Debiased Machine Learning (DDML) in Stata. Estimators of causal parameters for five different econometric models are supported, allowing for flexible estimation of causal effects of endogenous variables in settings with unknown functional forms and/or many exogenous variables. ddml is compatible with many existing supervised machine learning programs in Stata. We recommend using DDML in combination with stacking estimation which combines multiple machine learners into a final predictor. We provide Monte Carlo evidence to support our recommendation.

==> Applications/logs/interactive_crossfit.log.tex <==
. quietly ddml crossfit 
{\smallskip}


==> Applications/logs/interactive_start.log.tex <==
. use "sipp1991.dta", clear
{\smallskip}
. global Y net_tfa
{\smallskip}
. global X age inc educ fsize marr twoearn db pira hown
{\smallskip}
. global D e401
{\smallskip}


==> Applications/logs/interactive_timer.log.tex <==
. timer list
   1:    691.43 /        1 =     691.4330
   2:     21.30 /        1 =      21.3000
{\smallskip}


==> Applications/logs/iv_ivlasso.log.tex <==
. ivlasso $Y ($X) ($D = $Z)
1.  (PDS/CHS) Selecting HD controls for dep var net_tfa...
Selected: age inc twoearn pira
3.  (PDS) Selecting HD controls for endog regressor p401...
Selected: inc twoearn db pira hown
5.  (PDS/CHS) Selecting HD controls/IVs for endog regressor p401...
Selected: inc db pira e401
6a. (CHS) Selecting lasso HD controls and creating optimal IV for endog regressor p401...
Selected: inc educ twoearn db pira hown
6b. (CHS) Selecting post-lasso HD controls and creating optimal IV for endog regressor p401...
Selected: inc educ twoearn db pira hown
7.  (CHS) Creating orthogonalized endogenous regressor p401...
{\smallskip}
{\smallskip}
Estimation results:
{\smallskip}
Specification:
Regularization method:                 lasso
Penalty loadings:                      homoskedastic
Number of observations:                9,915
Endogenous (1):                        p401
High-dim controls (9):                 age inc educ fsize marr twoearn db pira hown
Selected controls, PDS (6):            age inc twoearn db pira hown
Selected controls, CHS-L (7):          age inc educ twoearn db pira hown
Selected controls, CHS-PL (7):         age inc educ twoearn db pira hown
Unpenalized controls (1):              _cons
High-dim instruments (1):              e401
Selected instruments (1):              e401
{\smallskip}
Structural equation:
{\smallskip}
IV using CHS lasso-orthogonalized vars
\HLI{13}{\TOPT}\HLI{64}
     net_tfa {\VBAR} Coefficient  Std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        p401 {\VBAR}   8278.685    1797.89     4.60   0.000     4754.885    11802.48
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
IV using CHS post-lasso-orthogonalized vars
\HLI{13}{\TOPT}\HLI{64}
     net_tfa {\VBAR} Coefficient  Std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        p401 {\VBAR}   8544.016   1797.428     4.75   0.000     5021.122    12066.91
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
IV with PDS-selected variables and full regressor set
\HLI{13}{\TOPT}\HLI{64}
     net_tfa {\VBAR} Coefficient  Std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        p401 {\VBAR}   8420.673   1798.673     4.68   0.000     4895.339    11946.01
         age {\VBAR}    671.029    57.8319    11.60   0.000     557.6805    784.3774
         inc {\VBAR}   .9034016   .0283988    31.81   0.000     .8477409    .9590623
     twoearn {\VBAR}  -19288.68   1293.173   -14.92   0.000    -21823.26   -16754.11
          db {\VBAR}   -4755.26   1291.513    -3.68   0.000     -7286.58   -2223.941
        pira {\VBAR}    28911.8   1450.411    19.93   0.000     26069.05    31754.55
        hown {\VBAR}   797.0986   1298.687     0.61   0.539    -1748.282    3342.479
       _cons {\VBAR}  -44184.22   2435.374   -18.14   0.000    -48957.46   -39410.98
\HLI{13}{\BOTT}\HLI{64}
Standard errors and test statistics valid for the following variables only:
    p401
\HLI{78}


==> Applications/logs/iv_ivreg2.log.tex <==
. ivreg2 $Y $X ($D = $Z), robust
{\smallskip}
IV (2SLS) estimation
\HLI{20}
{\smallskip}
Estimates efficient for homoskedasticity only
Statistics robust to heteroskedasticity
{\smallskip}
                                                      Number of obs =     9915
                                                      F( 10,  9904) =   107.57
                                                      Prob > F      =   0.0000
Total (centered) SS     =  4.00041e+13                Centered R2   =   0.2348
Total (uncentered) SS   =  4.32349e+13                Uncentered R2 =   0.2920
Residual SS             =  3.06120e+13                Root MSE      =    55565
{\smallskip}
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        p401 {\VBAR}   8502.323   2192.535     3.88   0.000     4205.034    12799.61
         age {\VBAR}   630.0183   55.21924    11.41   0.000     521.7906     738.246
         inc {\VBAR}   .9265484   .1107111     8.37   0.000     .7095586    1.143538
        educ {\VBAR}  -617.5012    337.431    -1.83   0.067    -1278.854    43.85145
       fsize {\VBAR}  -1014.935   384.9964    -2.64   0.008    -1769.514   -260.3556
        marr {\VBAR}   893.3085   1732.216     0.52   0.606    -2501.773     4288.39
     twoearn {\VBAR}  -19278.86   2525.998    -7.63   0.000    -24229.73      -14328
          db {\VBAR}  -4552.834   1311.777    -3.47   0.001    -7123.869   -1981.799
        pira {\VBAR}   29114.81   1801.951    16.16   0.000     25583.05    32646.57
        hown {\VBAR}   1087.157   956.7152     1.14   0.256    -787.9705    2962.284
       _cons {\VBAR}  -33151.53    4401.75    -7.53   0.000     -41778.8   -24524.26
\HLI{13}{\BOTT}\HLI{64}
Underidentification test (Kleibergen-Paap rk LM statistic):           3173.401
                                                   Chi-sq(1) P-val =    0.0000
\HLI{78}
Weak identification test (Cragg-Donald Wald F statistic):              1.3e+04
                         (Kleibergen-Paap rk Wald F statistic):       7550.520
Stock-Yogo weak ID test critical values: 10\% maximal IV size             16.38
                                         15\% maximal IV size              8.96
                                         20\% maximal IV size              6.66
                                         25\% maximal IV size              5.53
Source: Stock-Yogo (2005).  Reproduced by permission.
NB: Critical values are for Cragg-Donald F statistic and i.i.d. errors.
\HLI{78}
Hansen J statistic (overidentification test of all instruments):         0.000
                                                 (equation exactly identified)
\HLI{78}
Instrumented:         p401
Included instruments: age inc educ fsize marr twoearn db pira hown
Excluded instruments: e401
\HLI{78}


==> Applications/logs/iv_timer.log.tex <==
. timer list
   1:    231.91 /        2 =     115.9555
   2:      0.86 /        1 =       0.8610
{\smallskip}


==> Applications/logs/ivhd_crossfit.log.tex <==
. qui ddml crossfit
{\smallskip}


==> Applications/logs/ivhd_extract.log.tex <==
. ddml extract, show(pystacked)
{\smallskip}
pystacked weights for Dpystacked (price)
             learner          h   resample     fold_1     fold_2     fold_3     fold_4
      ols          1          0          1  6.684e-14          0          0          0
  lassocv          2          0          1          0  4.548e-15  7.464e-14  7.390e-14
  ridgecv          3          0          1          0  3.781e-15  4.426e-14  4.281e-14
       rf          4          0          1  1.484e-13          0          0          0
       rf          5          0          1  1.058e-14  .28753859  .12885457  .01217774
       rf          6          0          1  .54450007  .29654961   .1429607  .41307432
gradboost          7          0          1  9.917e-14          0          0          0
gradboost          8          0          1  .42496365  .34078594  .67207761  .40296011
gradboost          9          0          1  .03053628  .07512585  .05610712  .17178783
      ols          1          0          2  3.753e-14  1.951e-14  8.458e-15          0
  lassocv          2          0          2          0          0          0  1.906e-14
  ridgecv          3          0          2  3.736e-15          0          0          0
       rf          4          0          2  4.377e-14  2.355e-14  9.454e-15  8.245e-15
       rf          5          0          2  2.510e-14  .15096782   .1507388  .19000524
       rf          6          0          2  .47768407  .29323724  .34918543  .30700964
gradboost          7          0          2  3.863e-14  6.476e-14  2.048e-14          0
gradboost          8          0          2  .19211242  .34790628  .48310231  .37343217
gradboost          9          0          2  .33020351  .20788865  .01697345  .12955296
      ols          1          0          3          0  2.365e-14          0          0
  lassocv          2          0          3  5.195e-14          0  1.155e-14  1.310e-13
  ridgecv          3          0          3  5.447e-14          0  9.093e-15  1.300e-13
       rf          4          0          3          0  4.650e-15  .02549704          0
       rf          5          0          3  .22500438  .44070099          0  .13281869
       rf          6          0          3  .17262943  .18583176  .38859744  .46657304
gradboost          7          0          3          0  2.758e-14          0          0
gradboost          8          0          3  .32781693  .32457454  .38030769  .09129508
gradboost          9          0          3  .27454926   .0488927  .20559782  .30931319
      ols          1          0          4          0  7.972e-15  5.848e-14  2.414e-13
  lassocv          2          0          4  7.882e-14          0          0          0
  ridgecv          3          0          4  8.737e-14  3.380e-16          0          0
       rf          4          0          4          0  6.054e-15  6.531e-14  2.286e-13
       rf          5          0          4  .15661663  .66423415  .19952232  7.794e-14
       rf          6          0          4  .27320783          0  .35255999  .43340414
gradboost          7          0          4          0  1.581e-14  1.000e-13  2.103e-13
gradboost          8          0          4  .45378153  .14094054   .1551841  .40417273
gradboost          9          0          4  .11639402  .19482531  .29273359  .16242313
      ols          1          0          5  2.863e-13  1.976e-13  4.497e-14          0
  lassocv          2          0          5          0          0  7.364e-16  7.497e-16
  ridgecv          3          0          5          0          0  1.142e-14          0
       rf          4          0          5  4.904e-13  1.950e-13  5.850e-14          0
       rf          5          0          5  2.266e-13  8.896e-14  1.612e-14  4.480e-14
       rf          6          0          5  .40352103  .41762186  .47606692    .345412
gradboost          7          0          5  2.841e-13  2.512e-13  4.131e-14          0
gradboost          8          0          5  .53638017   .5362937  .40476106  .25564384
gradboost          9          0          5   .0600988  .04608444  .11917202  .39894416
      ols          1          1          1  1.395e-14  1.308e-14          0  2.454e-14
  lassocv          2          1          1          0          0  6.495e-14          0
  ridgecv          3          1          1          0          0          0          0
       rf          4          1          1  1.684e-14  6.365e-15          0  1.695e-14
       rf          5          1          1  1.064e-14  4.402e-15          0  3.166e-14
       rf          6          1          1  .52544402  .54673383  .55758541  .54746448
gradboost          7          1          1  3.074e-14  3.281e-14          0  6.191e-14
gradboost          8          1          1  .27636376  .32777462  .44241459   .1019554
gradboost          9          1          1  .19819222  .12549156          0  .35058012
      ols          1          1          2  1.890e-14          0          0  2.433e-14
  lassocv          2          1          2          0  1.453e-14  1.921e-14          0
  ridgecv          3          1          2          0  1.345e-14          0          0
       rf          4          1          2  6.878e-14          0          0  4.421e-14
       rf          5          1          2  1.242e-14          0          0  2.425e-14
       rf          6          1          2  .63158939  .46019162  .67722071   .5963667
gradboost          7          1          2  8.386e-14          0          0  5.125e-14
gradboost          8          1          2  .18130958          0  .00503874  .20209727
gradboost          9          1          2  .18710103  .53980838  .31774055  .20153603
      ols          1          1          3  4.428e-14  7.797e-14          0  3.553e-14
  lassocv          2          1          3          0          0  2.117e-14          0
  ridgecv          3          1          3          0          0          0          0
       rf          4          1          3  5.864e-14  1.771e-13          0  2.056e-13
       rf          5          1          3  .23294913  6.323e-14          0  1.154e-13
       rf          6          1          3  .49402119   .5043501  .65317815  .45072162
gradboost          7          1          3  1.111e-13  1.534e-13          0  7.567e-14
gradboost          8          1          3  .13551556  .15765004  .24873979  .38365681
gradboost          9          1          3  .13751411  .33799986  .09808206  .16562157
      ols          1          1          4          0  5.684e-15          0          0
  lassocv          2          1          4  2.901e-15          0  5.543e-15  1.428e-14
  ridgecv          3          1          4          0          0  1.413e-15  9.116e-15
       rf          4          1          4          0  1.800e-14          0          0
       rf          5          1          4          0  .40703772          0          0
       rf          6          1          4  .47610824  .15098834  .57694413  .64042859
gradboost          7          1          4          0  8.781e-15          0          0
gradboost          8          1          4   .3362379   .3848424  .37241209   .1331677
gradboost          9          1          4  .18765385  .05713154  .05064378  .22640371
      ols          1          1          5  6.976e-15  2.936e-14          0          0
  lassocv          2          1          5          0          0  5.581e-15  1.014e-14
  ridgecv          3          1          5          0  1.395e-14          0  4.614e-15
       rf          4          1          5  2.163e-15  4.729e-14          0          0
       rf          5          1          5          0  1.451e-14          0          0
       rf          6          1          5  .60649867  .55522268  .63512311  .61897587
gradboost          7          1          5  2.785e-15  4.921e-14          0          0
gradboost          8          1          5  .17806008  .42621093  .08264572   .2486208
gradboost          9          1          5  .21544125  .01856639  .28223117  .13240333
{\smallskip}
mean stacking weights across folds/resamples for Dpystacked (price)
final stacking estimator: nnls1
               learner        h=0/1  mean_weight        rep_1        rep_2        rep_3        rep_4
      ols            1            0    4.964e-14    1.671e-14    1.637e-14    5.913e-15    7.697e-14
  lassocv            2            0    2.235e-14    3.827e-14    4.765e-15    4.862e-14    1.970e-14
  ridgecv            3            0    1.936e-14    2.271e-14    9.339e-16    4.839e-14    2.193e-14
       rf            4            0    .00127485    3.709e-14    2.125e-14    .00637426    7.500e-14
       rf            5            0      .136959    .10714273    .12292797    .19963101    .25509327
       rf            6            0    .33698133    .34927118     .3567791    .30340792    .26479299
gradboost            7            0    5.766e-14    2.479e-14    3.097e-14    6.895e-15    8.152e-14
gradboost            8            0    .36242462    .46019683     .3491383    .28099856    .28851972
gradboost            9            0    .16236021    .08338927    .17115464    .20958825    .19159401
      ols            1            1    1.473e-14    1.289e-14    1.081e-14    3.945e-14    1.421e-15
  lassocv            2            1    7.915e-15    1.624e-14    8.434e-15    5.293e-15    5.681e-15
  ridgecv            3            1    2.127e-15            0    3.362e-15            0    2.632e-15
       rf            4            1    3.309e-14    1.004e-14    2.825e-14    1.103e-13    4.499e-15
       rf            5            1    .03199934    1.168e-14    9.168e-15    .05823728    .10175943
       rf            6            1    .54525784    .54430694     .5913421    .52556777    .46111733
gradboost            7            1    3.308e-14    3.137e-14    3.378e-14    8.504e-14    2.195e-15
gradboost            8            1    .23123569    .28712709     .0971114    .23139055    .30666503
gradboost            9            1    .19150713    .16856597     .3115465     .1848044    .13045822
{\smallskip}
                 rep_5
      ols    1.322e-13
  lassocv    3.715e-16
  ridgecv    2.854e-15
       rf    1.860e-13
       rf    9.411e-14
       rf    .41065545
gradboost    1.441e-13
gradboost    .43326969
gradboost    .15607486
      ols    9.084e-15
  lassocv    3.929e-15
  ridgecv    4.642e-15
       rf    1.236e-14
       rf    3.629e-15
       rf    .60395508
gradboost    1.300e-14
gradboost    .23388438
gradboost    .16216054
{\smallskip}
pystacked MSEs for Dpystacked (price)
             learner          h   resample     fold_1     fold_2     fold_3     fold_4
      ols          1          0          1  27.654481   29.47464  28.076006  28.292504
  lassocv          2          0          1  20.780887   21.44238  20.218993  20.356871
  ridgecv          3          0          1  20.179493  21.062222  19.752622  19.799632
       rf          4          0          1  13.540421  11.062124  11.857453  12.304421
       rf          5          0          1  10.926145  9.6122685  10.332944  10.316119
       rf          6          0          1  10.826797  9.8640383  10.621712   10.42188
gradboost          7          0          1  12.749382  11.573561  11.422589   11.99231
gradboost          8          0          1  11.170893  10.248572  9.0459769  10.032442
gradboost          9          0          1  12.279593  11.190689  10.267115   10.82207
      ols          1          0          2  27.342604  29.242327  28.519793  28.113878
  lassocv          2          0          2  20.236814  21.552063  20.532669  20.725354
  ridgecv          3          0          2  19.851486  21.129351  19.890586  20.227042
       rf          4          0          2  11.856152  11.645507   12.14447  10.532635
       rf          5          0          2  9.9546666  10.063705  10.333647  9.3995318
       rf          6          0          2   10.00466  10.259627  10.535332  9.6186064
gradboost          7          0          2  12.350401  11.766486  11.808571  11.187471
gradboost          8          0          2  9.9845744   9.981562  10.394957  9.5578438
gradboost          9          0          2  10.373852   10.45938  11.720774  10.347383
      ols          1          0          3  28.483671  28.220269  27.794446  28.355478
  lassocv          2          0          3  20.706932  20.933363  20.164788   21.14066
  ridgecv          3          0          3  20.047456  20.388242  19.712999  20.598241
       rf          4          0          3  12.392987  10.714619  10.470942  12.474003
       rf          5          0          3  10.731924  9.4142366  10.022865  10.497886
       rf          6          0          3  11.033408   9.685917   10.11181  10.546024
gradboost          7          0          3  12.249821  11.380249  10.863989  13.017474
gradboost          8          0          3  10.283103  10.254523   9.590783  11.704499
gradboost          9          0          3  10.836977  10.952117  10.156521  11.498166
      ols          1          0          4  26.182723  26.122852  31.036622  30.088722
  lassocv          2          0          4  18.846666  19.635204  22.203237  22.061741
  ridgecv          3          0          4  18.158635  19.263575  21.478245  21.573939
       rf          4          0          4  11.198913    10.2039  11.833033  12.116289
       rf          5          0          4  9.5518372  8.8908281  10.544445  10.520794
       rf          6          0          4  9.7681868  9.5142767  10.695039  10.520121
gradboost          7          0          4  10.632549  11.341962  12.565013   12.29816
gradboost          8          0          4  9.2552235  10.096884  11.012963  10.238549
gradboost          9          0          4  10.206638  10.462664  11.385693  11.075024
      ols          1          0          5  28.002889  27.843241  28.336435  29.554557
  lassocv          2          0          5  20.673262  19.515762  21.444228   21.98044
  ridgecv          3          0          5  20.077262  18.961966  21.041321  21.482864
       rf          4          0          5  12.700752  10.731134  11.970013  11.130054
       rf          5          0          5  10.863181  9.5542647  10.812182  10.058931
       rf          6          0          5   10.87005  9.3778468  10.725386  10.283375
gradboost          7          0          5   11.83682  10.816203  12.259205  11.614315
gradboost          8          0          5  10.180115  8.8842654  10.668941  9.3581671
gradboost          9          0          5  11.125289  10.288168  11.719986  9.5814888
      ols          1          1          1  21.161373  23.002806  22.144975  22.450373
  lassocv          2          1          1  21.517796  23.438622  21.811291  22.728793
  ridgecv          3          1          1  21.114174  23.120955  21.670865  22.451824
       rf          4          1          1  10.596617  10.761174  11.984298  12.148231
       rf          5          1          1  10.293998  10.353702  11.257095  11.824558
       rf          6          1          1  10.065955  10.127618  10.815018  11.491516
gradboost          7          1          1  11.822402  12.491456  12.793693  13.552266
gradboost          8          1          1  10.322247  10.471967  11.100629  11.920162
gradboost          9          1          1  10.899859   11.55421  12.757301   12.17326
      ols          1          1          2  22.276165  22.599173  22.066726  21.396679
  lassocv          2          1          2  22.572917  22.894809   22.61149  21.549111
  ridgecv          3          1          2  22.314561  22.722995  22.256802  21.298698
       rf          4          1          2  11.822971  13.130768  11.140799  11.576661
       rf          5          1          2  10.843904  12.372549  10.332201  10.687975
       rf          6          1          2  10.458186  11.897665  9.9338061  10.236337
gradboost          7          1          2  13.048976  14.086309  12.664215  12.863244
gradboost          8          1          2  11.243313  12.370801  11.417371  10.632601
gradboost          9          1          2  11.916084   11.63065  11.295453  11.699322
      ols          1          1          3  22.500642  21.806585  22.658255  21.618007
  lassocv          2          1          3  22.896531  22.017153  22.995685  21.916387
  ridgecv          3          1          3  22.586509  21.840362  22.723985  21.676416
       rf          4          1          3  11.561736  11.040638  11.230166  14.566843
       rf          5          1          3  10.773021  10.224218  10.391431  13.633686
       rf          6          1          3  10.727285  9.9748633  9.9991408  12.699042
gradboost          7          1          3  13.313758  11.833133  11.979319  13.993391
gradboost          8          1          3   11.87109  10.208898  10.911126  12.545464
gradboost          9          1          3   12.75979  10.467039   11.63129  13.214775
      ols          1          1          4  20.397679  20.255451  23.355458  24.589219
  lassocv          2          1          4  20.606957  20.243186  24.038802  24.802947
  ridgecv          3          1          4  20.460036  20.131445  23.677855  24.438116
       rf          4          1          4  12.367744  11.912322  10.748732  13.424128
       rf          5          1          4  11.741177  10.609353  10.249128  11.940283
       rf          6          1          4  11.279838  10.629504  9.7533319  11.674355
gradboost          7          1          4  13.022409  12.198312  12.069799  14.335446
gradboost          8          1          4  11.270713   10.89693  10.223859   12.75706
gradboost          9          1          4  12.015865   11.56573  10.879138  13.048922
      ols          1          1          5  21.510681  22.848224   21.52014  23.805464
  lassocv          2          1          5  22.085136  23.029649  22.000039  24.287342
  ridgecv          3          1          5  21.680404  22.847699  21.661545  23.986492
       rf          4          1          5  12.405853  11.388676  11.746738  12.853652
       rf          5          1          5  11.614172  10.579658  11.011248   11.99732
       rf          6          1          5  11.341593  10.218715  10.636312  11.499519
gradboost          7          1          5  13.402173  12.815227   12.68463   14.21706
gradboost          8          1          5  12.185735  10.521822  11.456374  12.264315
gradboost          9          1          5  12.434926  11.805344   11.97433  13.320151
{\smallskip}
mean stacking MSEs across folds/resamples for Dpystacked (price)
final stacking estimator: nnls1
             learner      h=0/1   mean_MSE      rep_1      rep_2      rep_3      rep_4      rep_5
      ols          1          0  28.336907  28.374408   28.30465  28.213466   28.35773   28.43428
  lassocv          2          0  20.757616  20.699783  20.761725  20.736436  20.686712  20.903423
  ridgecv          3          0  20.233859  20.198492  20.274616  20.186735  20.118599  20.390853
       rf          4          0  11.643991  12.191105  11.544691  11.513138  11.338034  11.632988
       rf          5          0   10.12012  10.296869  9.9378876  10.166728   9.876976   10.32214
       rf          6          0  10.264205  10.433607  10.104556   10.34429  10.124406  10.314164
gradboost          7          0  11.786327  11.934461  11.778232  11.877883  11.709421  11.631636
gradboost          8          0  10.097242  10.124471  9.9797343  10.458227  10.150905  9.7728722
gradboost          9          0  10.837479  11.139867  10.725347  10.860945  10.782505  10.678733
      ols          1          1  22.198204  22.189882  22.084686  22.145872  22.149452  22.421127
  lassocv          2          1  22.502232  22.374126  22.407082  22.456439  22.422973  22.850542
  ridgecv          3          1  22.233087  22.089454  22.148264  22.206818  22.176863  22.544035
       rf          4          1  11.920437   11.37258    11.9178  12.099846  12.113232   12.09873
       rf          5          1  11.136534  10.932338  11.059157  11.255589  11.134985  11.300599
       rf          6          1   10.77298  10.625027  10.631498  10.850083  10.834257  10.924035
gradboost          7          1  12.959361  12.664954  13.165686    12.7799  12.906491  13.279773
gradboost          8          1  11.329624  10.953751  11.416022  11.384144  11.287141  11.607061
gradboost          9          1  11.952172  11.846157  11.635378  12.018223  11.877414  12.383688
{\smallskip}
pystacked weights for Ypystacked (y)
             learner   resample     fold_1     fold_2     fold_3     fold_4
      ols          1          1  .02202723  8.415e-17  .03194791  .02210337
  lassocv          2          1  5.803e-17  .05592933  .02710254  .04877038
  ridgecv          3          1          0  1.055e-16          0  2.231e-17
       rf          4          1  .20477644  6.721e-17          0          0
       rf          5          1  .37862077  .67378601  .29330412  .40736099
       rf          6          1  .12736549  .03051162  .49695337  .30645129
gradboost          7          1          0  2.033e-16  7.458e-17  7.591e-17
gradboost          8          1  .13039564  .23490441  9.124e-17  .12035177
gradboost          9          1  .13681443  .00486862  .15069207   .0949622
      ols          1          2  8.326e-17  .02594304  6.043e-17  .08519234
  lassocv          2          2  1.611e-16  .00911441  .03450593  .00863408
  ridgecv          3          2          0  8.400e-17          0  1.497e-17
       rf          4          2  9.381e-18  2.132e-17          0  1.007e-16
       rf          5          2  .86481125  .51371989  .81637981  .27370295
       rf          6          2  2.683e-17   .1709433          0  .42081202
gradboost          7          2          0  1.438e-16  1.618e-17  4.317e-16
gradboost          8          2  .03266687  .14828883  4.321e-17  2.964e-17
gradboost          9          2  .10252189  .13199054  .14911426  .21165861
      ols          1          3  .04156773  8.362e-17   .0121596  .03518175
  lassocv          2          3  .02826987  1.137e-16  .08922384    .013682
  ridgecv          3          3  3.282e-17          0          0          0
       rf          4          3          0          0  5.183e-17          0
       rf          5          3  .44475936  .32407368   .6391443  .64935249
       rf          6          3  .10700981  .47780913  7.759e-18  .23503784
gradboost          7          3  3.646e-16          0  2.048e-18  5.417e-18
gradboost          8          3  .12052244  .19811719  .25501523  1.409e-17
gradboost          9          3  .25787079  7.952e-18  .00445703  .06674593
      ols          1          4  .03986904          0  6.433e-18  .06724546
  lassocv          2          4          0  .05117027  .02202308  .03878502
  ridgecv          3          4  4.955e-17  2.907e-17  3.878e-17          0
       rf          4          4  6.798e-17          0  2.501e-17  5.476e-18
       rf          5          4  .08385711  .42550742  7.273e-18  .12189666
       rf          6          4  .62795296  .36651882  .74850206  .50205943
gradboost          7          4  2.548e-18  1.345e-16  1.950e-16          0
gradboost          8          4  .24832089  .10231305    .128582  .20571685
gradboost          9          4          0  .05449045  .10089286  .06429659
      ols          1          5  .04589659  .08541394  2.761e-17  .05163815
  lassocv          2          5  2.271e-17  1.786e-16  2.407e-17  .00656744
  ridgecv          3          5          0          0          0          0
       rf          4          5          0          0  6.834e-17  2.824e-17
       rf          5          5   .0468433  .13915837  .13708515  .29685229
       rf          6          5  .72092177  .62946341  .72197713    .439907
gradboost          7          5          0          0  2.939e-18          0
gradboost          8          5  .17478222  7.024e-17  .03789115  .03885859
gradboost          9          5  .01155612  .14596429  .10304658  .16617653
{\smallskip}
mean stacking weights across folds/resamples for Ypystacked (y)
final stacking estimator: nnls1
               learner  mean_weight        rep_1        rep_2        rep_3        rep_4        rep_5
      ols            1    .02830931    .01901963    .02778385    .02222727    .02677863    .04573717
  lassocv            2    .02168891    .03295056     .0130636    .03279393    .02799459    .00164186
  ridgecv            3    1.885e-17    3.195e-17    2.474e-17    8.206e-18    2.935e-17            0
       rf            4    .01023882    .05119411    3.284e-17    1.296e-17    2.462e-17    2.415e-17
       rf            5     .3765108    .43826797    .61715347    .51433246     .1578153    .15498478
       rf            6    .35650982    .24032044    .14793883    .20496419    .56125832    .62806733
gradboost            7    8.263e-17    8.845e-17    1.479e-16    9.303e-17    8.301e-17    7.347e-19
gradboost            8    .10883636    .12141295    .04523892    .14341371     .1712332    .06288299
gradboost            9    .09790599    .09683433    .14882132    .08226844    .05491997    .10668588
{\smallskip}
pystacked MSEs for Ypystacked (y)
             learner   resample     fold_1     fold_2     fold_3     fold_4
      ols          1          1  1.4827709  1.4349885  1.3873566  1.4282659
  lassocv          2          1  1.4111108   1.372651  1.3297418  1.3625248
  ridgecv          3          1  1.4072944  1.3711798  1.3275575  1.3612455
       rf          4          1  1.0712646  1.0798987  1.0705231  1.1133639
       rf          5          1  1.0672267  1.0497036  1.0384382  1.0956218
       rf          6          1  1.0712603  1.0542989  1.0356276  1.0948973
gradboost          7          1  1.1926089  1.1656195  1.1781034  1.2249308
gradboost          8          1  1.1605596  1.1450167  1.1800479  1.2117121
gradboost          9          1  1.2343191   1.271138  1.2369229  1.3052664
      ols          1          2   1.444982  1.4332438  1.4321659  1.4200244
  lassocv          2          2  1.3833966  1.3613969  1.3676779  1.3727712
  ridgecv          3          2  1.3804042  1.3574348  1.3650675  1.3739719
       rf          4          2  1.0222948   1.067037  1.0903366  1.1290256
       rf          5          2  .99914798  1.0395607  1.0629904  1.1085011
       rf          6          2  1.0115102   1.041034  1.0735818  1.1045563
gradboost          7          2  1.1650101  1.1659375   1.202585  1.2422536
gradboost          8          2  1.1457473  1.1289804   1.201178  1.2381242
gradboost          9          2  1.2159442  1.1982492  1.2650998  1.2796193
      ols          1          3  1.4538827  1.4369906   1.432628  1.4144385
  lassocv          2          3  1.3929116  1.3743319  1.3603001  1.3630955
  ridgecv          3          3  1.3866661  1.3712834  1.3558462  1.3620922
       rf          4          3  1.1078367  1.0749438  1.1203955  1.0738667
       rf          5          3  1.0934883  1.0408964  1.0987215  1.0559025
       rf          6          3  1.0926234   1.038093    1.10441   1.059375
gradboost          7          3  1.1958944  1.1825328  1.1940647  1.1937909
gradboost          8          3  1.1522011  1.1525331  1.1879412  1.2311183
gradboost          9          3  1.1965188  1.2662236  1.3007124  1.3115696
      ols          1          4  1.4072616  1.4200592  1.4857461  1.4266816
  lassocv          2          4  1.3622675   1.359327   1.414404  1.3675166
  ridgecv          3          4  1.3561355  1.3603213  1.4133621  1.3654617
       rf          4          4  1.0822153   1.051135  1.1059597  1.1415179
       rf          5          4  1.0693647  1.0401612  1.0888105  1.1257355
       rf          6          4  1.0606432  1.0390026  1.0770688   1.120391
gradboost          7          4   1.165315  1.1673118  1.2233451   1.214115
gradboost          8          4  1.1527045  1.1743078  1.1942292  1.2060976
gradboost          9          4  1.2714072  1.2637465  1.2946546  1.2999481
      ols          1          5  1.4030444  1.4548078  1.4003274  1.4774769
  lassocv          2          5  1.3421787  1.4303355  1.3279418  1.4089542
  ridgecv          3          5   1.342048  1.4306611  1.3258379  1.4070088
       rf          4          5  1.0947016  1.1744779  1.0363535  1.1083325
       rf          5          5  1.0593981  1.1424968  1.0125396  1.0931793
       rf          6          5  1.0504572  1.1335157   1.006371    1.08935
gradboost          7          5  1.1864413  1.2631328  1.1570015  1.2139525
gradboost          8          5  1.1761265  1.2832805  1.1515926  1.2232834
gradboost          9          5  1.2697923  1.3520211  1.2257009  1.2808853
{\smallskip}
mean stacking MSEs across folds/resamples for Ypystacked (y)
final stacking estimator: nnls1
             learner   mean_MSE      rep_1      rep_2      rep_3      rep_4      rep_5
      ols          1  1.4338571  1.4333455   1.432604  1.4344849  1.4349371  1.4339141
  lassocv          2  1.3732418  1.3690071  1.3713107  1.3726598  1.3758788  1.3773525
  ridgecv          3   1.371044  1.3668193  1.3692196   1.368972  1.3738201   1.376389
       rf          4   1.090774  1.0837626  1.0771735  1.0942607  1.0952069  1.1034664
       rf          5  1.0690942  1.0627476  1.0525501  1.0722521   1.081018  1.0769035
       rf          6  1.0679034   1.064021  1.0576706  1.0736253  1.0742764  1.0699235
gradboost          7  1.1946973  1.1903157  1.1939465  1.1915707  1.1925217  1.2051321
gradboost          8  1.1848391  1.1743341  1.1785075  1.1809485  1.1818347  1.2085708
gradboost          9   1.266987  1.2619116  1.2397281  1.2687561  1.2824391  1.2820999
{\smallskip}


==> Applications/logs/ivhd_qddml.log.tex <==
. qui qddml $Y ($Xaug) ($D = $Zaug), model(fiv)
{\smallskip}


==> Applications/logs/ivhd_timer.log.tex <==
. timer list
   1:   2157.89 /        1 =    2157.8940
   2:     28.95 /        1 =      28.9480
{\smallskip}


==> Applications/logs/late_timer.log.tex <==
. timer list
   1:    184.34 /        1 =     184.3420
   2:     28.27 /        1 =      28.2750
{\smallskip}


==> Applications/logs/partial_2_add.log.tex <==
. *** add learners for E[Y|X]
. ddml E[Y|X]: reg $Y $X
Learner Y1_reg added successfully.
{\smallskip}
. ddml E[Y|X]: pystacked $Y c.($X)\#\#c.($X), type(reg) m(lassocv)
Learner Y2_pystacked added successfully.
{\smallskip}
. ddml E[Y|X]: pystacked $Y $X, type(reg) m(rf)
Learner Y3_pystacked added successfully.
{\smallskip}
. *** add learners for E[D|X]
. ddml E[D|X]: reg $D $X
Learner D1_reg added successfully.
{\smallskip}
. ddml E[D|X]: pystacked $D c.($X)\#\#c.($X), type(reg) m(lassocv)
Learner D2_pystacked added successfully.
{\smallskip}
. ddml E[D|X]: pystacked $D $X, type(reg) m(rf)
Learner D3_pystacked added successfully.


==> Applications/logs/partial_2_estimate.log.tex <==
. qui ddml crossfit
{\smallskip}
. ddml estimate, robust
{\smallskip}
DDML estimation results:
spec  r     Y learner     D learner         b        SE
 opt  1  Y2_pystacked  D2_pystacked 10005.974(1331.384)
opt = minimum MSE specification for that resample.
{\smallskip}
Min MSE DDML model
y-E[y|X]  = Y2_pystacked_1                         Number of obs   =      9915
D-E[D|X,Z]= D2_pystacked_1
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   10005.97   1331.384     7.52   0.000      7396.51    12615.44
       _cons {\VBAR}  -31.83575   532.7731    -0.06   0.952    -1076.052     1012.38
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
{\smallskip}


==> Applications/logs/partial_2_init.log.tex <==
. set seed 42
{\smallskip}
. ddml init partial, kfolds(4)


==> Applications/logs/partial_2_start.log.tex <==
. use "sipp1991.dta", clear
{\smallskip}
. global Y net_tfa
{\smallskip}
. global X age inc educ fsize marr twoearn db pira hown
{\smallskip}
. global D e401
{\smallskip}


==> Applications/logs/partial_abbrev_add.log.tex <==
. *** add learners for E[Y|X]
. ddml E[Y|X]: reg $Y $X
Learner Y1_reg added successfully.
{\smallskip}
. ddml E[Y|X]: pystacked $Y c.($X)\#\#c.($X), type(reg) m(lassocv)
Learner Y2_pystacked added successfully.
{\smallskip}
. *** add learners for E[D|X]
. ddml E[D|X]: reg $D $X
Learner D1_reg added successfully.
{\smallskip}
. ddml E[D|X]: pystacked $D c.($X)\#\#c.($X), type(reg) m(lassocv)
Learner D2_pystacked added successfully.


==> Applications/logs/partial_abbrev_crossfit.log.tex <==
. ddml crossfit
Cross-fitting E[y|X] equation: net_tfa
Cross-fitting fold 1 2 3 4 ...completed cross-fitting
Cross-fitting E[D|X] equation: e401
Cross-fitting fold 1 2 3 4 ...completed cross-fitting


==> Applications/logs/partial_abbrev_describe.log.tex <==
. ddml describe
{\smallskip}
Model:                  partial, crossfit folds k=4, resamples r=1
Mata global (mname):    m0
Dependent variable (Y): net_tfa
 net_tfa learners:      Y1_reg Y2_pystacked
D equations (1):        e401
 e401 learners:         D1_reg D2_pystacked
{\smallskip}


==> Applications/logs/partial_abbrev_estimate.log.tex <==
. ddml estimate, robust  
{\smallskip}
{\smallskip}
Model:                  partial, crossfit folds k=4, resamples r=1
Mata global (mname):    m0
Dependent variable (Y): net_tfa
 net_tfa learners:      Y1_reg Y2_pystacked
D equations (1):        e401
 e401 learners:         D1_reg D2_pystacked
{\smallskip}
DDML estimation results:
spec  r     Y learner     D learner         b        SE 
 mse  1  Y2_pystacked  D2_pystacked  9788.291 (1339.797)
mse = minimum MSE specification for that resample.
{\smallskip}
Min MSE DDML model
y-E[y|X]  = y-Y2_pystacked_1                       Number of obs   =      9915
D-E[D|X]  = D-D2_pystacked_1 
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   9788.291   1339.797     7.31   0.000     7162.337    12414.24
       _cons {\VBAR}   90.93481   534.8139     0.17   0.865    -957.2813    1139.151
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
{\smallskip}


==> Applications/logs/partial_abbrev_estimate_all.log.tex <==
. ddml estimate, robust allcombos
{\smallskip}
{\smallskip}
Model:                  partial, crossfit folds k=4, resamples r=1
Mata global (mname):    m0
Dependent variable (Y): net_tfa
 net_tfa learners:      Y1_reg Y2_pystacked
D equations (1):        e401
 e401 learners:         D1_reg D2_pystacked
{\smallskip}
DDML estimation results:
spec  r     Y learner     D learner         b        SE 
   1  1        Y1_reg        D1_reg  5986.657 (1523.694)
   2  1        Y1_reg  D2_pystacked  9563.875 (1389.172)
   3  1  Y2_pystacked        D1_reg  9175.519 (1371.065)
*  4  1  Y2_pystacked  D2_pystacked  9788.291 (1339.797)
* = minimum MSE specification for that resample.
{\smallskip}
Min MSE DDML model
y-E[y|X]  = y-Y2_pystacked_1                       Number of obs   =      9915
D-E[D|X]  = D-D2_pystacked_1 
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   9788.291   1339.797     7.31   0.000     7162.337    12414.24
       _cons {\VBAR}   90.93481   534.8139     0.17   0.865    -957.2813    1139.151
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
{\smallskip}


==> Applications/logs/partial_abbrev_init.log.tex <==
. set seed 123
{\smallskip}
. ddml init partial, kfolds(4)


==> Applications/logs/partial_abbrev_reg.log.tex <==
. gen double Y1_resid = $Y - Y1_reg
{\smallskip}
. gen double D1_resid = $D - D1_reg
{\smallskip}
. reg Y1_resid D1_resid,  robust
{\smallskip}
Linear regression                               Number of obs     =      9,915
                                                F(1, 9913)        =      15.44
                                                Prob > F          =     0.0001
                                                R-squared         =     0.0023
                                                Root MSE          =      55891
{\smallskip}
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
    Y1_resid {\VBAR} Coefficient  std. err.      t    P>|t|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
    D1_resid {\VBAR}   5986.657   1523.694     3.93   0.000     2999.906    8973.407
       _cons {\VBAR}   10.74705   561.2911     0.02   0.985    -1089.498    1110.992
\HLI{13}{\BOTT}\HLI{64}


==> Applications/logs/partial_abbrev_start.log.tex <==
. use "sipp1991.dta", clear
{\smallskip}
. global Y net_tfa
{\smallskip}
. global X age inc educ fsize marr twoearn db pira hown
{\smallskip}
. global D e401
{\smallskip}


==> Applications/logs/partial_drop.log.tex <==
. ddml drop


==> Applications/logs/partial_pdslasso.log.tex <==
. pdslasso $Y $D (c.($X)\#\#c.($X)), robust
1.  (PDS/CHS) Selecting HD controls for dep var net_tfa...
Selected: c.age\#c.age c.age\#c.inc c.age\#c.educ c.age\#c.pira c.inc\#c.pira c.inc\#c.hown c.fsize\#c.twoearn
          c.marr\#c.twoearn
2.  (PDS/CHS) Selecting HD controls for exog regressor e401...
Selected: inc db c.inc\#c.hown c.educ\#c.hown c.marr\#c.hown c.twoearn\#c.hown c.db\#c.db
{\smallskip}
{\smallskip}
Estimation results:
{\smallskip}
Specification:
Regularization method:                 lasso
Penalty loadings:                      heteroskedastic
Number of observations:                9,915
Exogenous (1):                         e401
High-dim controls (54):                age inc educ fsize marr twoearn db pira hown c.age\#c.age c.age\#c.inc
                                       c.age\#c.educ c.age\#c.fsize c.age\#c.marr c.age\#c.twoearn c.age\#c.db
                                       c.age\#c.pira c.age\#c.hown c.inc\#c.inc c.inc\#c.educ c.inc\#c.fsize
                                       c.inc\#c.marr c.inc\#c.twoearn c.inc\#c.db c.inc\#c.pira c.inc\#c.hown
                                       c.educ\#c.educ c.educ\#c.fsize c.educ\#c.marr c.educ\#c.twoearn c.educ\#c.db
                                       c.educ\#c.pira c.educ\#c.hown c.fsize\#c.fsize c.fsize\#c.marr
                                       c.fsize\#c.twoearn c.fsize\#c.db c.fsize\#c.pira c.fsize\#c.hown
                                       c.marr\#c.marr c.marr\#c.twoearn c.marr\#c.db c.marr\#c.pira c.marr\#c.hown
                                       c.twoearn\#c.twoearn c.twoearn\#c.db c.twoearn\#c.pira c.twoearn\#c.hown
                                       c.db\#c.db c.db\#c.pira c.db\#c.hown c.pira\#c.pira c.pira\#c.hown
                                       c.hown\#c.hown
Selected controls (14):                inc db c.age\#c.age c.age\#c.inc c.age\#c.educ c.age\#c.pira c.inc\#c.pira
                                       c.inc\#c.hown c.educ\#c.hown c.fsize\#c.twoearn c.marr\#c.twoearn
                                       c.marr\#c.hown c.twoearn\#c.hown c.db\#c.db
Unpenalized controls (1):              _cons
{\smallskip}
Structural equation:
{\smallskip}
OLS using CHS lasso-orthogonalized vars
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   6513.581   1501.738     4.34   0.000     3570.229    9456.932
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
OLS using CHS post-lasso-orthogonalized vars
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   6906.158   1469.777     4.70   0.000     4025.448    9786.867
\HLI{13}{\BOTT}\HLI{64}
{\smallskip}
OLS with PDS-selected variables and full regressor set
\HLI{18}{\TOPT}\HLI{64}
                  {\VBAR}               Robust
          net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{18}{\PLUS}\HLI{64}
             e401 {\VBAR}   6967.053   1398.607     4.98   0.000     4225.834    9708.273
              inc {\VBAR}  -1.120043   .3229324    -3.47   0.001    -1.752979    -.487107
               db {\VBAR}          0  (omitted)
                  {\VBAR}
      c.age\#c.age {\VBAR}  -4.847538   2.409461    -2.01   0.044    -9.569995   -.1250808
                  {\VBAR}
      c.age\#c.inc {\VBAR}   .0309783   .0085412     3.63   0.000      .014238    .0477187
                  {\VBAR}
     c.age\#c.educ {\VBAR}  -.3655992   8.272851    -0.04   0.965    -16.58009    15.84889
                  {\VBAR}
     c.age\#c.pira {\VBAR}   95.45902   124.3888     0.77   0.443    -148.3385    339.2565
                  {\VBAR}
     c.inc\#c.pira {\VBAR}   .5652377   .1216932     4.64   0.000     .3267233     .803752
                  {\VBAR}
     c.inc\#c.hown {\VBAR}   .5378702   .0902354     5.96   0.000     .3610121    .7147283
                  {\VBAR}
    c.educ\#c.hown {\VBAR}  -475.1051   191.6666    -2.48   0.013    -850.7646   -99.44552
                  {\VBAR}
c.fsize\#c.twoearn {\VBAR}   -704.981   542.4461    -1.30   0.194    -1768.156    358.1938
                  {\VBAR}
 c.marr\#c.twoearn {\VBAR}  -603.1194   2270.726    -0.27   0.791     -5053.66    3847.421
                  {\VBAR}
    c.marr\#c.hown {\VBAR}  -1804.657   2228.827    -0.81   0.418    -6173.077    2563.763
                  {\VBAR}
 c.twoearn\#c.hown {\VBAR}  -16960.05   2867.801    -5.91   0.000    -22580.83   -11339.26
                  {\VBAR}
        c.db\#c.db {\VBAR}  -3538.398   1208.534    -2.93   0.003    -5907.082   -1169.715
                  {\VBAR}
            _cons {\VBAR}   6689.737    6097.27     1.10   0.273    -5260.693    18640.17
\HLI{18}{\BOTT}\HLI{64}
Standard errors and test statistics valid for the following variables only:
    e401
\HLI{78}


==> Applications/logs/partial_qddml_replicate.log.tex <==
. global pystacked_opts                                                    || ///
>     method(ols)                                                          || ///
>     m(lassocv) xvars(c.($X)\#\#c.($X))                                     || ///
>     m(ridgecv) xvars(c.($X)\#\#c.($X))                                     || ///
>     m(rf) pipe(sparse) opt(max_features(5))                              || ///
>     m(gradboost) pipe(sparse) opt(n_estimators(250) learning_rate(0.01)) ,  ///
>     njobs(5)
{\smallskip}
. 
. set seed 123
{\smallskip}
. // suppress output with quietly
. qui qddml $Y $D ($X), model(partial) kfolds(4) robust   ///
>         pystacked($pystacked_opts) 
{\smallskip}
. 
. // illustrate replay option
. ddml estimate, spec(ss) rep(1) notable replay
{\smallskip}
Shortstack DDML model
y-E[y|X]  = y-Y_net_tfa_ss_1                       Number of obs   =      9915
D-E[D|X]  = D-D_e401_ss_1 
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   9602.257   1300.825     7.38   0.000     7052.686    12151.83
       _cons {\VBAR}   83.96648   533.9871     0.16   0.875    -962.6289    1130.562
\HLI{13}{\BOTT}\HLI{64}
Stacking final estimator: 
{\smallskip}
{\smallskip}


==> Applications/logs/partial_stack_allstack.log.tex <==
. ddml estimate, robust shortstack poolstack
{\smallskip}
{\smallskip}
Model:                  partial, crossfit folds k=4, resamples r=1
Mata global (mname):    m0
Dependent variable (Y): net_tfa
 net_tfa learners:      Y1_pystacked
D equations (1):        e401
 e401 learners:         D1_pystacked
{\smallskip}
DDML estimation results:
spec  r     Y learner     D learner         b        SE 
  st  1  Y1_pystacked  D1_pystacked  9406.385 (1300.170)
  ss  1  [shortstack]          [ss]  9602.257 (1300.825)
  ps  1   [poolstack]          [ps]  9500.180 (1298.057)
{\smallskip}
Shortstack DDML model
y-E[y|X]  = y-Y_net_tfa_ss_1                       Number of obs   =      9915
D-E[D|X]  = D-D_e401_ss_1 
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
     net_tfa {\VBAR} Coefficient  std. err.      z    P>|z|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
        e401 {\VBAR}   9602.257   1300.825     7.38   0.000     7052.686    12151.83
       _cons {\VBAR}   83.96648   533.9871     0.16   0.875    -962.6289    1130.562
\HLI{13}{\BOTT}\HLI{64}
Stacking final estimator: nnls1
{\smallskip}
{\smallskip}


==> Applications/logs/partial_stack_init.log.tex <==
. set seed 123 
{\smallskip}
. ddml init partial, kfolds(4)
warning - model m0 already exists
all existing model results and variables will
be dropped and model m0 will be re-initialized
{\smallskip}


==> Applications/logs/partial_stack_psweights.log.tex <==
. ddml extract, show(psweights)
{\smallskip}
pool-stacked weights across resamples for e401
final stacking estimator: nnls1
               learner  mean_weight        rep_1
      ols            1    .01402517    .01402517
  lassocv            2    .07247975    .07247975
  ridgecv            3    .45850746    .45850746
       rf            4    .02897607    .02897607
gradboost            5    .42601154    .42601154
{\smallskip}
pool-stacked weights across resamples for net_tfa
final stacking estimator: nnls1
               learner  mean_weight        rep_1
      ols            1    .07029722    .07029722
  lassocv            2    .54372578    .54372578
  ridgecv            3    .28352699    .28352699
       rf            4    .10245001    .10245001
gradboost            5            0            0
{\smallskip}


==> Applications/logs/partial_stack_reg.log.tex <==
. gen double Y1_resid = $Y - Y1_pystacked_L3_1
{\smallskip}
. gen double D1_resid = $D - D1_pystacked_L2_1
{\smallskip}
. reg Y1_resid D1_resid,  robust
{\smallskip}
Linear regression                               Number of obs     =      9,915
                                                F(1, 9913)        =      54.05
                                                Prob > F          =     0.0000
                                                R-squared         =     0.0067
                                                Root MSE          =      53236
{\smallskip}
\HLI{13}{\TOPT}\HLI{64}
             {\VBAR}               Robust
    Y1_resid {\VBAR} Coefficient  std. err.      t    P>|t|     [95\% conf. interval]
\HLI{13}{\PLUS}\HLI{64}
    D1_resid {\VBAR}   9847.256   1339.419     7.35   0.000     7221.724    12472.79
       _cons {\VBAR}   78.69447   534.6452     0.15   0.883    -969.3189    1126.708
\HLI{13}{\BOTT}\HLI{64}


==> Applications/logs/partial_stack_ssweights.log.tex <==
. ddml extract, show(ssweights)
{\smallskip}
short-stacked weights across resamples for e401
final stacking estimator: nnls1
               learner  mean_weight        rep_1
      ols            1            0            0
  lassocv            2    .24106979    .24106979
  ridgecv            3    .34172854    .34172854
       rf            4    .05456544    .05456544
gradboost            5    .36263623    .36263623
{\smallskip}
short-stacked weights across resamples for net_tfa
final stacking estimator: nnls1
               learner  mean_weight        rep_1
      ols            1    .07689168    .07689168
  lassocv            2            0            0
  ridgecv            3    .79121732    .79121732
       rf            4            0            0
gradboost            5      .131891      .131891
{\smallskip}


==> Applications/logs/partial_stack_start.log.tex <==
. use "sipp1991.dta", clear
{\smallskip}
. global Y net_tfa
{\smallskip}
. global X age inc educ fsize marr twoearn db pira hown
{\smallskip}
. global D e401
{\smallskip}


==> Applications/logs/partial_stack_stweights.log.tex <==
. ddml extract, show(stweights)
{\smallskip}
mean stacking weights across folds/resamples for D1_pystacked (e401)
final stacking estimator: nnls1
               learner  mean_weight        rep_1
      ols            1    .01557419    .01557419
  lassocv            2    .10077907    .10077907
  ridgecv            3    .43674242    .43674242
       rf            4    .02946916    .02946916
gradboost            5    .41743516    .41743516
{\smallskip}
mean stacking weights across folds/resamples for Y1_pystacked (net_tfa)
final stacking estimator: nnls1
               learner  mean_weight        rep_1
      ols            1    .09662631    .09662631
  lassocv            2    .46475744    .46475744
  ridgecv            3    .32388159    .32388159
       rf            4    .09392877    .09392877
gradboost            5     .0145518     .0145518
{\smallskip}


==> Applications/logs/partial_timer.log.tex <==
. timer list
   1:     22.74 /        1 =      22.7390
   2:     93.00 /        1 =      93.0050
   3:     50.66 /        1 =      50.6560
   4:     21.82 /        1 =      21.8170
   6:      2.04 /        1 =       2.0380
   7:      0.58 /        1 =       0.5820
   8:     51.72 /        1 =      51.7160
{\smallskip}


==> Cash_transfer/aizer.tex <==
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            &\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}\\
\hline
Accepted    &      0.0157\sym{*}  &      0.0158\sym{*}  &      0.0182\sym{*}  &      0.0154\sym{*}  &      0.0154\sym{*}  \\
            &   (0.00646)         &   (0.00655)         &   (0.00694)         &   (0.00677)         &   (0.00670)         \\
\hline
\(N\)       &        7860         &        7859         &        7859         &        7859         &        7859         \\


==> Cash_transfer/ate.tex <==
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}\\
\hline
ATE         &      0.0133\sym{*}  &      0.0150\sym{*}  &      0.0110         &      0.0124         &      0.0167\sym{**} \\
            &   (0.00594)         &   (0.00666)         &   (0.00747)         &   (0.00965)         &   (0.00607)         \\
\hline
\(N\)       &        7860         &        7859         &        7859         &        7859         &        7859         \\


==> Cash_transfer/atet.tex <==
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}\\
\hline
ATET        &      0.0129\sym{*}  &      0.0149\sym{*}  &     0.00967         &      0.0126         &      0.0173\sym{**} \\
            &   (0.00606)         &   (0.00694)         &   (0.00790)         &    (0.0112)         &   (0.00632)         \\
\hline
\(N\)       &        7860         &        7859         &        7859         &        7859         &        7859         \\


==> Cash_transfer/ateu.tex <==
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{} &\multicolumn{1}{c}{logageatdeath}&\multicolumn{1}{c}{logageatdeath}\\
\hline
ATEU        &      0.0162\sym{**} &      0.0160\sym{*}  &      0.0206\sym{**} &      0.0148\sym{*}  &      0.0145\sym{*}  \\
            &   (0.00566)         &   (0.00631)         &   (0.00690)         &   (0.00677)         &   (0.00647)         \\
\hline
\(N\)       &        7860         &        7859         &        7859         &        7859         &        7859         \\


==> GWG/Average_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 10:07:23 2023
 OLS/logit & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  OLS/logit (simple) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 3 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  

==> GWG/Average_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 10:18:19 2023
 OLS/logit & 0.077 & 0.077 & 0.077 \\ 
  OLS/logit (simple) & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso (extended) & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge (extended) & 0.077 & 0.077 & 0.077 \\ 
  Random forest 1 & 0.077 & 0.077 & 0.077 \\ 
  Random forest 2 & 0.077 & 0.077 & 0.077 \\ 
  Random forest 3 & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 1 & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 2 & 0.077 & 0.077 & 0.077 \\ 
  Neural net 1 & 0.077 & 0.077 & 0.077 \\ 
  Neural net 2 & 0.077 & 0.077 & 0.077 \\ 
  

==> GWG/Average_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 10:07:23 2023
 OLS/logit & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  OLS/logit (simple) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 3 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  

==> GWG/CLS_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.023 & 0.012 & 0.242 &  & 0.014 & 0.001 & 0.257 &  & 0.027 & 0.013 & 0.211 \\ 
  OLS/logit (simple) & 0.004 & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.103 & 0.136 & 0.109 &  & 0.15\phantom{0} & 0.23\phantom{0} & 0.136 &  & 0.03\phantom{0} & 0.076 & 0.047 \\ 
  CV-ridge & 0.189 & 0.04\phantom{0} & 0.064 &  & 0.205 & 0.064 & 0.063 &  & 0.225 & 0.024 & 0.108 \\ 
  CV-lasso (extended) & 0.041 & 0.157 & 0.016 &  & 0.\phantom{000} & 0.078 & 0.\phantom{000} &  & 0.035 & 0.266 & 0.002 \\ 
  CV-ridge (extended) & 0.011 & 0.04\phantom{0} & 0.011 &  & 0.\phantom{000} & 0.019 & 0.\phantom{000} &  & 0.003 & 0.024 & 0.022 \\ 
  Random forest 1 & 0.435 & 0.506 & 0.275 &  & 0.462 & 0.521 & 0.288 &  & 0.483 & 0.507 & 0.28\phantom{0} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.025 & 0.008 & 0.039 &  & 0.\phantom{000} & 0.\phantom{000} & 0.008 &  & 0.011 & 0.003 & 0.022 \\ 
  Gradient boosting 2 & 0.15\phantom{0} & 0.059 & 0.216 &  & 0.165 & 0.071 & 0.23\phantom{0} &  & 0.175 & 0.063 & 0.285 \\ 
  Neural net 1 & 0.013 & 0.022 & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.008 & 0.02\phantom{0} & 0.027 &  & 0.004 & 0.016 & 0.018 &  & 0.01\phantom{0} & 0.023 & 0.023 \\ 
  

==> GWG/CLS_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.014 & 0.001 & 0.257 \\ 
  OLS/logit (simple) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.15\phantom{0} & 0.23\phantom{0} & 0.136 \\ 
  CV-ridge & 0.205 & 0.064 & 0.063 \\ 
  CV-lasso (extended) & 0.\phantom{000} & 0.078 & 0.\phantom{000} \\ 
  CV-ridge (extended) & 0.\phantom{000} & 0.019 & 0.\phantom{000} \\ 
  Random forest 1 & 0.462 & 0.521 & 0.288 \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.\phantom{000} & 0.\phantom{000} & 0.008 \\ 
  Gradient boosting 2 & 0.165 & 0.071 & 0.23\phantom{0} \\ 
  Neural net 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.004 & 0.016 & 0.018 \\ 
  

==> GWG/CLS_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.023 & 0.012 & 0.242 &  & 0.027 & 0.013 & 0.211 \\ 
  OLS/logit (simple) & 0.004 & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.103 & 0.136 & 0.109 &  & 0.03\phantom{0} & 0.076 & 0.047 \\ 
  CV-ridge & 0.189 & 0.04\phantom{0} & 0.064 &  & 0.225 & 0.024 & 0.108 \\ 
  CV-lasso (extended) & 0.041 & 0.157 & 0.016 &  & 0.035 & 0.266 & 0.002 \\ 
  CV-ridge (extended) & 0.011 & 0.04\phantom{0} & 0.011 &  & 0.003 & 0.024 & 0.022 \\ 
  Random forest 1 & 0.435 & 0.506 & 0.275 &  & 0.483 & 0.507 & 0.28\phantom{0} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.025 & 0.008 & 0.039 &  & 0.011 & 0.003 & 0.022 \\ 
  Gradient boosting 2 & 0.15\phantom{0} & 0.059 & 0.216 &  & 0.175 & 0.063 & 0.285 \\ 
  Neural net 1 & 0.013 & 0.022 & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.008 & 0.02\phantom{0} & 0.027 &  & 0.01\phantom{0} & 0.023 & 0.023 \\ 
  

==> GWG/Interactive_mse.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 Interactive & OLS/logit & 0.161 & 0.369 & 0.347 \\ 
  Interactive & OLS/logit (simple) & 0.223 & 0.267 & 0.204 \\ 
  Interactive & CV-lasso & 0.16\phantom{0} & 0.236 & 0.178 \\ 
  Interactive & CV-ridge & 0.161 & 0.237 & 0.18\phantom{0} \\ 
  Interactive & CV-lasso (extended) & 0.161 & 0.238 & 0.18\phantom{0} \\ 
  Interactive & CV-ridge (extended) & 0.161 & 0.336 & 0.194 \\ 
  Interactive & Random forest 1 & 0.161 & 0.23\phantom{0} & 0.176 \\ 
  Interactive & Random forest 2 & 0.171 & 0.258 & 0.19\phantom{0} \\ 
  Interactive & Random forest 3 & 0.179 & 0.274 & 0.199 \\ 
  Interactive & Gradient boosting 1 & 0.16\phantom{0} & 0.239 & 0.183 \\ 
  Interactive & Gradient boosting 2 & 0.161 & 0.254 & 0.196 \\ 
  Interactive & Neural net 1 & 0.241 & 0.349 & 0.263 \\ 
  Interactive & Neural net 2 & 0.176 & 0.643 & 0.357 \\ 
  

==> GWG/Interactive_mse_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.023 & 0.012 & 0.242 &  & 0.027 & 0.013 & 0.211 &  & 0.369 & 0.347 & 0.161 \\ 
  OLS/logit (simple) & 0.004 & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.267 & 0.204 & 0.223 \\ 
  CV-lasso & 0.103 & 0.136 & 0.109 &  & 0.03\phantom{0} & 0.076 & 0.047 &  & 0.236 & 0.178 & 0.16\phantom{0} \\ 
  CV-ridge & 0.189 & 0.04\phantom{0} & 0.064 &  & 0.225 & 0.024 & 0.108 &  & 0.237 & 0.18\phantom{0} & 0.161 \\ 
  CV-lasso (extended) & 0.041 & 0.157 & 0.016 &  & 0.035 & 0.266 & 0.002 &  & 0.238 & 0.18\phantom{0} & 0.161 \\ 
  CV-ridge (extended) & 0.011 & 0.04\phantom{0} & 0.011 &  & 0.003 & 0.024 & 0.022 &  & 0.336 & 0.194 & 0.161 \\ 
  Random forest 1 & 0.435 & 0.506 & 0.275 &  & 0.483 & 0.507 & 0.28\phantom{0} &  & 0.23\phantom{0} & 0.176 & 0.161 \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.258 & 0.19\phantom{0} & 0.171 \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.274 & 0.199 & 0.179 \\ 
  Gradient boosting 1 & 0.025 & 0.008 & 0.039 &  & 0.011 & 0.003 & 0.022 &  & 0.239 & 0.183 & 0.16\phantom{0} \\ 
  Gradient boosting 2 & 0.15\phantom{0} & 0.059 & 0.216 &  & 0.175 & 0.063 & 0.285 &  & 0.254 & 0.196 & 0.161 \\ 
  Neural net 1 & 0.013 & 0.022 & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.349 & 0.263 & 0.241 \\ 
  Neural net 2 & 0.008 & 0.02\phantom{0} & 0.027 &  & 0.01\phantom{0} & 0.023 & 0.023 &  & 0.643 & 0.357 & 0.176 \\ 
  

==> GWG/OLS_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit &  0.022 & -0.01\phantom{0} &  0.206 &  &  0.009 & -0.008 &  0.212 &  &  0.039 & -0.006 &  0.193 \\ 
  OLS/logit (simple) & -0.035 & -0.019 &  0.081 &  & -0.041 & -0.014 &  0.083 &  & -0.072 & -0.019 &  0.075 \\ 
  CV-lasso &  0.007 & -0.024 &  0.326 &  &  0.056 &  0.078 &  0.202 &  & -0.222 & -0.154 &  0.169 \\ 
  CV-ridge &  0.534 &  0.28\phantom{0} &  0.089 &  &  0.462 &  0.295 &  0.105 &  &  0.709 &  0.33\phantom{0} &  0.204 \\ 
  CV-lasso (extended) & -0.028 &  0.251 & -0.189 &  & -0.056 &  0.123 & -0.081 &  &  0.041 &  0.378 & -0.2\phantom{00} \\ 
  CV-ridge (extended) & -0.086 & -0.049 &  0.015 &  & -0.042 & -0.045 &  0.008 &  & -0.149 & -0.075 &  0.024 \\ 
  Random forest 1 &  0.673 &  0.538 &  0.407 &  &  0.693 &  0.539 &  0.411 &  &  0.762 &  0.57\phantom{0} &  0.425 \\ 
  Random forest 2 & -0.098 &  0.383 &  0.112 &  & -0.06\phantom{0} &  0.411 &  0.11\phantom{0} &  & -0.035 &  0.143 &  0.124 \\ 
  Random forest 3 & -0.023 & -0.287 & -0.234 &  & -0.069 & -0.314 & -0.236 &  & -0.163 & -0.13\phantom{0} & -0.267 \\ 
  Gradient boosting 1 &  0.039 & -0.051 &  0.088 &  &  0.039 & -0.042 &  0.087 &  &  0.058 &  0.005 &  0.089 \\ 
  Gradient boosting 2 &  0.084 &  0.045 &  0.154 &  &  0.085 &  0.046 &  0.156 &  &  0.088 &  0.028 &  0.216 \\ 
  Neural net 1 & -0.312 & -0.158 & -1.635 &  &  0.001 &  0.011 & -0.005 &  &  0.001 &  0.028 & -0.052 \\ 
  Neural net 2 & -0.005 &  0.007 &  0.021 &  & -0.004 &  0.011 &  0.019 &  & -0.003 &  0.009 &  0.01\phantom{0} \\ 
  

==> GWG/OLS_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit &  0.009 & -0.008 &  0.212 \\ 
  OLS/logit (simple) & -0.041 & -0.014 &  0.083 \\ 
  CV-lasso &  0.056 &  0.078 &  0.202 \\ 
  CV-ridge &  0.462 &  0.295 &  0.105 \\ 
  CV-lasso (extended) & -0.056 &  0.123 & -0.081 \\ 
  CV-ridge (extended) & -0.042 & -0.045 &  0.008 \\ 
  Random forest 1 &  0.693 &  0.539 &  0.411 \\ 
  Random forest 2 & -0.06\phantom{0} &  0.411 &  0.11\phantom{0} \\ 
  Random forest 3 & -0.069 & -0.314 & -0.236 \\ 
  Gradient boosting 1 &  0.039 & -0.042 &  0.087 \\ 
  Gradient boosting 2 &  0.085 &  0.046 &  0.156 \\ 
  Neural net 1 &  0.001 &  0.011 & -0.005 \\ 
  Neural net 2 & -0.004 &  0.011 &  0.019 \\ 
  

==> GWG/OLS_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit &  0.022 & -0.01\phantom{0} &  0.206 &  &  0.039 & -0.006 &  0.193 \\ 
  OLS/logit (simple) & -0.035 & -0.019 &  0.081 &  & -0.072 & -0.019 &  0.075 \\ 
  CV-lasso &  0.007 & -0.024 &  0.326 &  & -0.222 & -0.154 &  0.169 \\ 
  CV-ridge &  0.534 &  0.28\phantom{0} &  0.089 &  &  0.709 &  0.33\phantom{0} &  0.204 \\ 
  CV-lasso (extended) & -0.028 &  0.251 & -0.189 &  &  0.041 &  0.378 & -0.2\phantom{00} \\ 
  CV-ridge (extended) & -0.086 & -0.049 &  0.015 &  & -0.149 & -0.075 &  0.024 \\ 
  Random forest 1 &  0.673 &  0.538 &  0.407 &  &  0.762 &  0.57\phantom{0} &  0.425 \\ 
  Random forest 2 & -0.098 &  0.383 &  0.112 &  & -0.035 &  0.143 &  0.124 \\ 
  Random forest 3 & -0.023 & -0.287 & -0.234 &  & -0.163 & -0.13\phantom{0} & -0.267 \\ 
  Gradient boosting 1 &  0.039 & -0.051 &  0.088 &  &  0.058 &  0.005 &  0.089 \\ 
  Gradient boosting 2 &  0.084 &  0.045 &  0.154 &  &  0.088 &  0.028 &  0.216 \\ 
  Neural net 1 & -0.312 & -0.158 & -1.635 &  &  0.001 &  0.028 & -0.052 \\ 
  Neural net 2 & -0.005 &  0.007 &  0.021 &  & -0.003 &  0.009 &  0.01\phantom{0} \\ 
  

==> GWG/Single-best_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  OLS/logit (simple) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.06\phantom{0} & 0.03\phantom{0} & 0.79\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 1.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.4\phantom{00} \\ 
  CV-ridge & 0.07\phantom{0} & 0.\phantom{000} & 0.04\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.1\phantom{00} \\ 
  CV-lasso (extended) & 0.02\phantom{0} & 0.06\phantom{0} & 0.03\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.1\phantom{00} \\ 
  CV-ridge (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.01\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 1 & 0.85\phantom{0} & 0.91\phantom{0} & 0.02\phantom{0} &  & 1.\phantom{000} & 1.\phantom{000} & 0.\phantom{000} &  & 1.\phantom{000} & 1.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.\phantom{000} & 0.\phantom{000} & 0.11\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.4\phantom{00} \\ 
  Gradient boosting 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  

==> GWG/Single-best_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  OLS/logit (simple) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.\phantom{000} & 0.\phantom{000} & 1.\phantom{000} \\ 
  CV-ridge & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-ridge (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 1 & 1.\phantom{000} & 1.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  

==> GWG/Single-best_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  OLS/logit (simple) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.06\phantom{0} & 0.03\phantom{0} & 0.79\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.4\phantom{00} \\ 
  CV-ridge & 0.07\phantom{0} & 0.\phantom{000} & 0.04\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.1\phantom{00} \\ 
  CV-lasso (extended) & 0.02\phantom{0} & 0.06\phantom{0} & 0.03\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.1\phantom{00} \\ 
  CV-ridge (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.01\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 1 & 0.85\phantom{0} & 0.91\phantom{0} & 0.02\phantom{0} &  & 1.\phantom{000} & 1.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.\phantom{000} & 0.\phantom{000} & 0.11\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.4\phantom{00} \\ 
  Gradient boosting 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  

==> GWG/regression_results_1.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 19:32:00 2023
estimator & avg & nnls1 & ols & singlebest \\ 
 Regular
stacking & -0.101 & -0.075 & -0.197 & -0.061 \\ 
   & (0.017)* & (0.028)* & (11.894) & (0.069) \\ 
  Short-
stacking & -0.101 & -0.076 & -0.001 & -0.085 \\ 
   & (0.017)* & (0.028)* & (0.184) & (0.065) \\ 
  Pooled
stacking & -0.101 & -0.075 & 0.137 & -0.072 \\ 
   & (0.017)* & (0.027)* & (0.111) & (0.055) \\ 
  

==> GWG/regression_results_2.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 19:32:00 2023
estimator & indiv \\ 
 OLS/logit & -0.12 \\ 
   & (0.094) \\ 
  CV-lasso & -0.067 \\ 
   & (0.063) \\ 
  CV-ridge & -0.064 \\ 
   & (0.09) \\ 
  OLS/logit
(simple) & -0.12 \\ 
   & (0.016)* \\ 
  CV-lasso
(extended) & -0.055 \\ 
   & (0.076) \\ 
  CV-ridge
(extended) & -0.173 \\ 
   & (0.19) \\ 
  Random
forest 1 & -0.079 \\ 
   & (0.023)* \\ 
  Random
forest 2 & -0.105 \\ 
   & (0.016)* \\ 
  Random
forest 3 & -0.11 \\ 
   & (0.015)* \\ 
  Gradient
boosting 1 & -0.075 \\ 
   & (0.021)* \\ 
  Gradient
boosting 2 & -0.044 \\ 
   & (0.044) \\ 
  Neural
net 1 & -0.121 \\ 
   & (0.077) \\ 
  Neural
net 2 & -0.004 \\ 
   & (0.344) \\ 
  

==> Pres_tables/CLS_weights_wopooled_pres.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Mon Aug 28 18:33:42 2023
 OLS/logit & 0.027 & 0.010 & 0.246 &  & 0.037 & 0.009 & 0.218 \\ 
  OLS/logit (simple) & 0.001 & 0.001 & 0.000 &  & 0.000 & 0.000 & 0.000 \\ 
  CV-lasso & 0.111 & 0.136 & 0.109 &  & 0.060 & 0.073 & 0.063 \\ 
  CV-ridge & 0.182 & 0.037 & 0.055 &  & 0.217 & 0.019 & 0.110 \\ 
  CV-lasso (extended) & 0.035 & 0.189 & 0.005 &  & 0.007 & 0.253 & 0.015 \\ 
  CV-ridge (extended) &\mycol 0.010 &\mycol 0.034 &\mycol 0.014 &  &\mycol 0.000 & \mycol 0.028 &\mycol 0.004 \\ 
  Random forest 1 &\mycol 0.440 &\mycol 0.499 &\mycol 0.289 &  &\mycol 0.479 &\mycol 0.498 &\mycol 0.284 \\ 
  Random forest 2 & 0.000 & 0.000 & 0.000 &  & 0.000 & 0.000 & 0.000 \\ 
  Random forest 3 & 0.000 & 0.000 & 0.000 &  & 0.000 & 0.000 & 0.000 \\ 
  Gradient boosting 1 & 0.026 & 0.009 & 0.025 &  & 0.028 & 0.008 & 0.017 \\ 
  Gradient boosting 2 & 0.145 & 0.050 & 0.227 &  & 0.155 & 0.081 & 0.269 \\ 
  Neural net 1 & 0.014 & 0.014 & 0.000 &  & 0.005 & 0.000 & 0.000 \\ 
  Neural net 2 & 0.009 & 0.021 & 0.030 &  & 0.012 & 0.031 & 0.021 \\ 
  

==> Pres_tables/sim_output_dgp0_long_pres.tex <==
&OLS&\mycol -24.8&\mycol 820.2&\mycol 0.95&&\mycol -1.9&\mycol 269.1&\mycol 0.95 \tabularnewline
&PDS-Lasso&-25.4&821.2&0.95&&0.6&269.4&0.95 \tabularnewline
&OLS&-30.5&826.8&0.95&&-2.3&270.5&0.95 \tabularnewline
&Lasso with CV (2nd order poly)&-28.5&830.2&0.96&&-1.5&272.6&0.95 \tabularnewline
&Ridge with CV (2nd order poly)&-25.5&821.1&0.95&&-1.9&275.9&0.95 \tabularnewline
&Lasso with CV (10th order poly)&187.4&1047.6&0.95&&61.4&281.7&0.94 \tabularnewline
&Ridge with CV (10th order poly)&1069.3&1221.0&0.94&&38.1&273.4&0.94 \tabularnewline
&Random forest (low regularization)&-196.5&982.2&0.91&&-33.3&356.7&0.87 \tabularnewline
&Random forest (high regularization)&-28.1&853.1&0.95&&-22.5&288.7&0.94 \tabularnewline
&Gradient boosting (low regularization)&-82.2&825.0&0.95&&-19.4&270.9&0.95 \tabularnewline
&Gradient boosting (high regularization)&28.6&819.6&0.96&&71.4&279.8&0.94 \tabularnewline
&Neural net&309.2&866.0&0.94&&17.4&288.1&0.94 \tabularnewline
&Stacking: CLS&\mycol 8.8&\mycol 829.3&\mycol 0.95&&\mycol -1.5&\mycol 274.4&\mycol 0.95 \tabularnewline
&Stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95 \tabularnewline
&Stacking: OLS&-33.7&874.1&0.94&&2.6&272.0&0.95 \tabularnewline
&Stacking: Single-best&\mycol -28.6&\mycol 823.3&\mycol 0.96&&\mycol -3.5&\mycol 272.1&\mycol 0.95 \tabularnewline
&Short-stacking: CLS&\mycol -23.8&\mycol 817.6&\mycol 0.96&&\mycol -1.5&\mycol 274.3&\mycol 0.95 \tabularnewline
&Short-stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95 \tabularnewline
&Short-stacking: OLS&-27.9&818.1&0.96&&-2.4&274.4&0.95 \tabularnewline
&Short-stacking: Single-best&\mycol -20.7&\mycol 826.0&\mycol 0.96&&\mycol -3.4&\mycol 272.4&\mycol 0.95 \tabularnewline
&Short-stacking: CLS 2&-33.3&819.9&0.95&&-2.2&273.2&0.95 \tabularnewline
&Short-stacking: Single-best 2&-31.3&823.0&0.96&&-4.2&276.0&0.95 \tabularnewline
&Pooled stacking: CLS&-24.8&817.8&0.96&&-1.5&273.4&0.95 \tabularnewline
&Pooled stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95 \tabularnewline
&Pooled stacking: OLS&-48.1&834.6&0.95&&-2.2&272.1&0.95 \tabularnewline
&Pooled stacking: Single-best&-23.0&829.7&0.96&&-3.3&270.9&0.95 \tabularnewline


==> Pres_tables/sim_output_dgp1_long_pres.tex <==
&OLS&\mycol -2587.3&\mycol 2642.4&\mycol 0.58&&\mycol -2644.9&\mycol 2640.5&\mycol 0.\phantom{00} \tabularnewline
&PDS-Lasso&-2598.4&2661.3&0.57&&-2644.1&2638.4&0.\phantom{00} \tabularnewline
&OLS&-2617.9&2622.6&0.58&&-2647.2&2645.8&0.\phantom{00} \tabularnewline
&Lasso with CV (2nd order poly)&746.2&1105.5&0.89&&703.5&714.6&0.61 \tabularnewline
&Ridge with CV (2nd order poly)&801.9&1143.6&0.89&&714.3&725.3&0.60 \tabularnewline
&Lasso with CV (10th order poly)&-4684.7&2111.1&0.90&&-2.1&284.5&0.94 \tabularnewline
&Ridge with CV (10th order poly)&-3070.8&2499.6&0.87&&-1.9&287.5&0.95 \tabularnewline
&Random forest (low regularization)&-64.0&1065.0&0.90&&-43.4&331.8&0.87 \tabularnewline
&Random forest (high regularization)&-133.0&932.3&0.94&&-18.5&272.8&0.94 \tabularnewline
&Gradient boosting (low regularization)&52.4&924.3&0.93&&13.6&267.7&0.95 \tabularnewline
&Gradient boosting (high regularization)&199.8&895.4&0.94&&182.3&319.3&0.93 \tabularnewline
&Neural net&-620.3&1103.6&0.91&&-142.9&292.0&0.92 \tabularnewline
&Stacking: CLS&\mycol 226.8&\mycol 1129.3&\mycol 0.93&&\mycol 24.9&\mycol 262.9&\mycol 0.95 \tabularnewline
&Stacking: Average&-101.7&1102.7&0.93&&60.0&271.9&0.95 \tabularnewline
&Stacking: OLS&871.4&1264.7&0.93&&26.6&265.7&0.94 \tabularnewline
&Stacking: Single-best&\mycol 179.2&\mycol 1016.2&\mycol 0.92&&\mycol 15.0&\mycol 266.4&\mycol 0.95 \tabularnewline
&Short-stacking: CLS&\mycol 221.9&\mycol 897.3&\mycol 0.93&&\mycol 21.9&\mycol 261.7&\mycol 0.95 \tabularnewline
&Short-stacking: Average&-101.7&1102.7&0.93&&60.0&271.9&0.95 \tabularnewline
&Short-stacking: OLS&169.0&888.2&0.93&&15.8&262.5&0.94 \tabularnewline
&Short-stacking: Single-best&\mycol 116.1&\mycol 900.1&\mycol 0.94&&\mycol 15.0&\mycol 266.4&\mycol 0.95 \tabularnewline
&Short-stacking: CLS 2&203.8&892.2&0.93&&18.0&263.1&0.95 \tabularnewline
&Short-stacking: Single-best 2&99.6&906.8&0.93&&13.6&267.7&0.95 \tabularnewline
&Pooled stacking: CLS&251.5&960.1&0.93&&24.8&264.8&0.95 \tabularnewline
&Pooled stacking: Average&-101.7&1102.7&0.93&&60.0&271.9&0.95 \tabularnewline
&Pooled stacking: OLS&376.8&1068.3&0.93&&16.7&266.5&0.94 \tabularnewline
&Pooled stacking: Single-best&131.0&952.0&0.93&&15.0&266.4&0.95 \tabularnewline


==> Pres_tables/sweights_nnls1_grad_nopooled.tex <==
OLS&\mycol 0.011&\mycol 0.015&&\mycol 0.004&\mycol 0.010 \tabularnewline
Lasso with CV (2nd order poly)&0.036&0.059&&0.016&0.038 \tabularnewline
Ridge with CV (2nd order poly)&0.153&0.231&&0.123&0.230 \tabularnewline
Lasso with CV (10th order poly)&0.060&0.076&&0.052&0.063 \tabularnewline
Ridge with CV (10th order poly)&0.074&0.061&&0.061&0.056 \tabularnewline
Random forest (low regularization)&0.042&0.012&&0.043&0.006 \tabularnewline
Random forest (high regularization)&0.021&0.076&&0.014&0.063 \tabularnewline
Gradient boosting (low regularization)&\mycol 0.523&\mycol 0.229&&\mycol 0.615&\mycol 0.346 \tabularnewline
Gradient boosting (high regularization)&0.014&0.192&&0.005&0.139 \tabularnewline
Neural net&0.067&0.049&&0.066&0.050 \tabularnewline


==> Pres_tables/sweights_nnls1_ols_nopooled.tex <==
OLS&\mycol 0.680&\mycol 0.494&&\mycol 0.677&\mycol 0.485 \tabularnewline
Lasso with CV (2nd order poly)&0.096&0.138&&0.114&0.135 \tabularnewline
Ridge with CV (2nd order poly)&0.068&0.058&&0.080&0.069 \tabularnewline
Lasso with CV (10th order poly)&0.030&0.074&&0.022&0.076 \tabularnewline
Ridge with CV (10th order poly)&0.028&0.043&&0.027&0.055 \tabularnewline
Random forest (low regularization)&0.013&0.011&&0.008&0.007 \tabularnewline
Random forest (high regularization)&0.018&0.028&&0.012&0.024 \tabularnewline
Gradient boosting (low regularization)&\mycol 0.028&\mycol 0.045&&\mycol 0.025&\mycol 0.043 \tabularnewline
Gradient boosting (high regularization)&0.020&0.062&&0.019&0.061 \tabularnewline
Neural net&0.019&0.047&&0.016&0.044 \tabularnewline


==> Simul/R_simulations/ae98_covar.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{lrrr}
\toprule
\midrule
Average & \multicolumn{1}{l}{y} & \multicolumn{1}{l}{D} & \multicolumn{1}{l}{Z} \\
\midrule
y     & 0.238721 & -0.034888 & 0.000022 \\
D     & -0.034888 & 0.194645 & 0.000506 \\
Z     & 0.000022 & 0.000506 & 0.000388 \\
      &       &       &  \\
Stacking &       &       &  \\
\midrule
y     & 0.238034 & -0.034845 & 0.000013 \\
D     & -0.034845 & 0.194439 & 0.000131 \\
Z     & 0.000013 & 0.000131 & 0.000255 \\
      &       &       &  \\
Best  &       &       &  \\
\midrule
y     & 0.238059 & -0.034804 & 0.000003 \\
D     & -0.034804 & 0.194692 & 0.000162 \\
Z     & 0.000003 & 0.000162 & 0.000359 \\
\midrule
\bottomrule
\end{tabular}%


==> Simul/R_simulations/ae98_covar_sngl.tex <==
\begin{tabular}{lrrr}
\toprule
\midrule
      & \multicolumn{1}{l}{y} & \multicolumn{1}{l}{D} & \multicolumn{1}{l}{Z} \\
\midrule
Lasso &       &       &  \\
y     & 2.40E-01 & -3.47E-02 & -2.46E-06 \\
D     & -3.47E-02 & 1.95E-01 & 8.41E-06 \\
Z     & -2.46E-06 & 8.41E-06 & 1.35E-05 \\
OLS   &       &       &  \\
y     & 2.40E-01 & -3.46E-02 & -2.03E-06 \\
D     & -3.46E-02 & 1.95E-01 & 4.40E-06 \\
Z     & -2.03E-06 & 4.40E-06 & 1.27E-05 \\
Lasso / OLS &       &       &  \\
y     & 2.40E-01 & -3.47E-02 & -1.50E-05 \\
D     & -3.47E-02 & 1.95E-01 & 5.69E-05 \\
Z     & -1.50E-05 & 5.69E-05 & 7.10E-05 \\
OLS / Lasso &       &       &  \\
y     & 2.40E-01 & -3.47E-02 & 1.97E-07 \\
D     & -3.47E-02 & 1.95E-01 & 5.66E-06 \\
Z     & 1.97E-07 & 5.66E-06 & 1.37E-05 \\
\midrule
\bottomrule
\end{tabular}%


==> Simul/R_simulations/ae98_table.tex <==
\begin{tabular}{lccc} 
\toprule\midrule 
 & Same sex & No signal & Some signal\\
 \midrule
Average (IV) & -0.126 & 3.679 & -0.113\\
 & (0.029) & (1970.886) & (0.038)\\
Average (OIV) & -0.075 & 0.015 & -0.041\\
 & (0.019) & (0.022) & (0.02)\\
Average (OIV, no LIE) & -0.145 & 3.353 & -0.127\\
 & (0.028) & (439.529) & (0.035)\\
OLS & -0.179 & -0.179 & -0.179\\
 & (0.002) & (0.002) & (0.002)\\
SSIV & -0.121 & -1.363 & -0.116\\
 & (0.028) & (244.079) & (0.037)\\
SSIV (s) & -0.127 & -2.3 & -0.12\\
 & (0.029) & (394.027) & (0.037)\\
Single best (IV) & -0.128 & 4.326 & -0.12\\
 & (0.029) & (2352.427) & (0.037)\\
Single best (OIV) & -0.14 & -0.798 & -0.127\\
 & (0.027) & (0.227) & (0.036)\\
Single best (OIV, no LIE) & -0.135 & 0.915 & -0.122\\
 & (0.027) & (281.09) & (0.036)\\
Stacking (IV) & -0.127 & 0.511 & -0.119\\
 & (0.028) & (483.227) & (0.037)\\
Stacking (OIV) & -0.13 & -0.186 & -0.115\\
 & (0.026) & (0.107) & (0.034)\\
Stacking (OIV, no LIE) & -0.142 & 0.812 & -0.134\\
 & (0.029) & (395.206) & (0.04)\\
TSLS & -0.122 & -0.69 & -0.116\\
 & (0.028) & (146.854) & (0.037)\\
XGB (IV) & -0.126 & -1.103 & 3.775\\
 & (0.028) & (0.086) & (1.163)\\
XGB (OIV) & 0.011 & 0.046 & 0.045\\
 & (0.011) & (0.011) & (0.011)\\
XGB (OIV, no LIE) & -0.305 & -0.759 & -0.158\\
 & (0.039) & (0.673) & (1.486)\\
XGB (c, IV) & -0.126 & -0.37 & 0.092\\
 & (0.028) & (0.1) & (0.092)\\
XGB (c, OIV) & -0.077 & -0.061 & -0.058\\
 & (0.011) & (0.011) & (0.011)\\
XGB (c, OIV, no LIE) & -0.222 & -0.196 & -0.088\\
 & (0.042) & (0.329) & (1.39)\\
cv-Lasso (IV) & -0.121 & 1.408 & -0.116\\
 & (0.028) & (104.049) & (0.037)\\
cv-Lasso (OIV) & -0.121 & 0.016 & -0.116\\
 & (0.028) & (0.155) & (0.037)\\
cv-Lasso (OIV, no LIE) & -0.122 & -0.834 & -0.116\\
 & (0.028) & (16.217) & (0.037)\\
cv-Lasso (s, IV) & -0.128 & -0.068 & -0.122\\
 & (0.029) & (202.714) & (0.037)\\
cv-Lasso (s, OIV) & -0.137 & -0.148 & -0.123\\
 & (0.027) & (0.177) & (0.036)\\
cv-Lasso (s, OIV, no LIE) & -0.137 & -0.446 & -0.121\\
 & (0.027) & (23.653) & (0.036)\\
cv-Ridge (IV) & -0.122 & 2.403 & -0.116\\
 & (0.028) & (265.204) & (0.037)\\
cv-Ridge (OIV) & -0.121 & 0.013 & -0.116\\
 & (0.028) & (0.155) & (0.037)\\
cv-Ridge (OIV, no LIE) & -0.122 & -0.102 & -0.116\\
 & (0.028) & (47.405) & (0.037)\\
cv-Ridge (s, IV) & -0.128 & -1.004 & -0.122\\
 & (0.029) & (168.304) & (0.037)\\
cv-Ridge (s, OIV) & -0.137 & -0.134 & -0.122\\
 & (0.027) & (0.174) & (0.036)\\
cv-Ridge (s, OIV, no LIE) & -0.137 & 1.425 & -0.121\\
 & (0.027) & (794.144) & (0.036)\\
\midrule\bottomrule 
\end{tabular}


==> Simul/R_simulations/ae98_table_FS.tex <==
\begin{tabular}{lc} 
\toprule\midrule 
 & No signal\\
 \midrule
Average (OIV) & 0.044\\
 & (0.038)\\
Average (OIV): DZ & 1.306\\
 & (0.044)\\
Average (OIV): yD & -0.179\\
 & (0.002)\\
Average (OIV): yZ & 0.057\\
 & (0.049)\\
Best (OIV) & 0.022\\
 & (0.118)\\
Best (OIV): DZ & 0.451\\
 & (0.045)\\
Best (OIV): yD & -0.179\\
 & (0.002)\\
Best (OIV): yZ & 0.009\\
 & (0.051)\\
Stacking (OIV) & 0.104\\
 & (0.12)\\
Stacking (OIV): DZ & 0.514\\
 & (0.053)\\
Stacking (OIV): yD & -0.179\\
 & (0.002)\\
Stacking (OIV): yZ & 0.054\\
 & (0.06)\\
\midrule\bottomrule 
\end{tabular}

==> Simul/R_simulations/ae98_table_sngl.tex <==
\begin{tabular}{lcccc} 
\toprule\midrule 
 & Lasso & OLS & Lasso / OLS & OLS / Lasso\\
 \midrule
IV coefficient  & -0.348 & -1.461 & -0.271 & 0.033\\
 & (1.472) & (44.021) & (0.157) & (11.04)\\
DZ & 0.61 & 0.325 & 0.801 & 0.405\\
 & (0.233) & (0.25) & (0.1) & (0.237)\\
yD & -0.179 & -0.178 & -0.178 & -0.178\\
 & (0.002) & (0.002) & (0.002) & (0.002)\\
yZ & -0.183 & -0.183 & -0.216 & 0.019\\
 & (0.27) & (0.285) & (0.119) & (0.27)\\
\midrule\bottomrule 
\end{tabular}


==> Simul/R_simulations/ensembles/ae98_ens_1.tex <==
\begin{tabular}{lccccccccc} 
\toprule\midrule 
 & \multicolumn{3}{c}{Weights: Stacking} & \multicolumn{3}{c}{Weights: Single Best} & \multicolumn{3}{c}{MSPE}\\
 \midrule
IV & $Z \vert X$ & $D \vert X$ & $Y \vert X$ & $Z \vert X$ & $D \vert X$ & $Y \vert X$ & $Z \vert X$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.011 & 0.0 & 0.073 & 0.0 & 0.0 & 0.0 & 0.25 & 0.198 & 0.239\\
OLS (s) & 0.113 & 0.307 & 0.062 & 0.0 & 0.119 & 0.0 & 0.25 & 0.195 & 0.24\\
Lasso (s) & 0.007 & 0.22 & 0.007 & 0.0 & 0.409 & 0.0 & 0.25 & 0.195 & 0.24\\
Ridge (s) & 0.005 & 0.238 & 0.012 & 0.0 & 0.472 & 0.0 & 0.25 & 0.195 & 0.24\\
XGB (c) & 0.865 & 0.235 & 0.846 & 1.0 & 0.0 & 1.0 & 0.249 & 0.197 & 0.238\\
 \midrule
Optimal IV & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.073 & 0.0 & 0.07 & 0.0 & 0.0 & 0.0 & 0.197 & 0.005 & 0.239\\
OLS (s) & 0.314 & 0.173 & 0.064 & 0.102 & 0.102 & 0.0 & 0.193 & 0.001 & 0.24\\
Lasso (s) & 0.273 & 0.419 & 0.007 & 0.46 & 0.864 & 0.0 & 0.193 & 0.001 & 0.24\\
Ridge (s) & 0.34 & 0.409 & 0.009 & 0.438 & 0.034 & 0.0 & 0.193 & 0.001 & 0.24\\
XGB (c) & 0.0 & 0.0 & 0.851 & 0.0 & 0.0 & 1.0 & 0.196 & 0.005 & 0.238\\
 \midrule
Optimal IV (no LIE) & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.075 & 0.0 & 0.071 & 0.0 & 0.0 & 0.0 & 0.197 & 0.198 & 0.239\\
OLS (s) & 0.318 & 0.309 & 0.063 & 0.148 & 0.114 & 0.0 & 0.193 & 0.195 & 0.24\\
Lasso (s) & 0.282 & 0.208 & 0.008 & 0.347 & 0.443 & 0.0 & 0.193 & 0.195 & 0.24\\
Ridge (s) & 0.325 & 0.248 & 0.009 & 0.506 & 0.443 & 0.0 & 0.193 & 0.195 & 0.24\\
XGB (c) & 0.0 & 0.234 & 0.849 & 0.0 & 0.0 & 1.0 & 0.196 & 0.197 & 0.238\\
\midrule\bottomrule 
\end{tabular}


==> Simul/R_simulations/ensembles/ae98_ens_2.tex <==
\begin{tabular}{lccccccccc} 
\toprule\midrule 
 & \multicolumn{3}{c}{Weights: Stacking} & \multicolumn{3}{c}{Weights: Single Best} & \multicolumn{3}{c}{MSPE}\\
 \midrule
Optimal IV & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.079 & 0.001 & 0.063 & 0.0 & 0.0 & 0.0 & 0.198 & 0.004 & 0.239\\
OLS (s) & 0.439 & 0.102 & 0.007 & 0.493 & 0.397 & 0.0 & 0.195 & 0.0 & 0.24\\
Lasso (s) & 0.221 & 0.448 & 0.044 & 0.233 & 0.603 & 0.0 & 0.195 & 0.0 & 0.24\\
Ridge (s) & 0.261 & 0.448 & 0.045 & 0.273 & 0.0 & 0.0 & 0.195 & 0.0 & 0.24\\
XGB (c) & 0.0 & 0.0 & 0.841 & 0.0 & 0.0 & 1.0 & 0.197 & 0.004 & 0.238\\
\midrule\bottomrule 
\end{tabular}





% \begin{tabular}{lccccccccc} 
% \toprule\midrule 
%  & \multicolumn{3}{c}{Weights: Stacking} & \multicolumn{3}{c}{Weights: Single Best} & \multicolumn{3}{c}{MSPE}\\
%  \midrule
% IV & $Z \vert X$ & $D \vert X$ & $Y \vert X$ & $Z \vert X$ & $D \vert X$ & $Y \vert X$ & $Z \vert X$ & $D \vert X$ & $Y \vert X$\\
% OLS & 0.917 & 0.0 & 0.072 & 1.0 & 0.0 & 0.0 & 0.004 & 0.198 & 0.239\\
% OLS (s) & 0.075 & 0.318 & 0.073 & 0.0 & 0.12 & 0.0 & 0.004 & 0.195 & 0.24\\
% Lasso (s) & 0.004 & 0.266 & 0.005 & 0.0 & 0.455 & 0.0 & 0.004 & 0.195 & 0.24\\
% Ridge (s) & 0.004 & 0.182 & 0.004 & 0.0 & 0.425 & 0.0 & 0.004 & 0.195 & 0.24\\
% XGB (c) & 0.001 & 0.235 & 0.846 & 0.0 & 0.0 & 1.0 & 0.008 & 0.197 & 0.238\\
%  \midrule
% Optimal IV & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
% OLS & 0.07 & 0.0 & 0.07 & 0.0 & 0.0 & 0.0 & 0.198 & 0.004 & 0.239\\
% OLS (s) & 0.285 & 0.525 & 0.07 & 0.085 & 0.1 & 0.0 & 0.195 & 0.0 & 0.24\\
% Lasso (s) & 0.312 & 0.238 & 0.006 & 0.51 & 0.9 & 0.0 & 0.195 & 0.0 & 0.24\\
% Ridge (s) & 0.333 & 0.238 & 0.006 & 0.405 & 0.0 & 0.0 & 0.195 & 0.0 & 0.24\\
% XGB (c) & 0.0 & 0.0 & 0.847 & 0.0 & 0.0 & 1.0 & 0.196 & 0.004 & 0.238\\
%  \midrule
% Optimal IV (no LIE) & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
% OLS & 0.069 & 0.0 & 0.07 & 0.0 & 0.0 & 0.0 & 0.198 & 0.198 & 0.239\\
% OLS (s) & 0.268 & 0.313 & 0.071 & 0.095 & 0.14 & 0.0 & 0.195 & 0.195 & 0.24\\
% Lasso (s) & 0.295 & 0.258 & 0.005 & 0.405 & 0.495 & 0.0 & 0.195 & 0.195 & 0.24\\
% Ridge (s) & 0.368 & 0.194 & 0.005 & 0.5 & 0.365 & 0.0 & 0.195 & 0.195 & 0.24\\
% XGB (c) & 0.0 & 0.235 & 0.849 & 0.0 & 0.0 & 1.0 & 0.196 & 0.197 & 0.238\\
% \midrule\bottomrule 
% \end{tabular}


==> Simul/R_simulations/ensembles/ae98_ens_3.tex <==
\begin{tabular}{lccccccccc} 
\toprule\midrule 
 & \multicolumn{3}{c}{Weights: Stacking} & \multicolumn{3}{c}{Weights: Single Best} & \multicolumn{3}{c}{MSPE}\\
 \midrule
IV & $Z \vert X$ & $D \vert X$ & $Y \vert X$ & $Z \vert X$ & $D \vert X$ & $Y \vert X$ & $Z \vert X$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.816 & 0.0 & 0.073 & 1.0 & 0.0 & 0.0 & 0.005 & 0.198 & 0.239\\
OLS (s) & 0.176 & 0.303 & 0.065 & 0.0 & 0.079 & 0.0 & 0.005 & 0.195 & 0.24\\
Lasso (s) & 0.002 & 0.226 & 0.008 & 0.0 & 0.421 & 0.0 & 0.005 & 0.195 & 0.24\\
Ridge (s) & 0.002 & 0.236 & 0.007 & 0.0 & 0.5 & 0.0 & 0.005 & 0.195 & 0.24\\
XGB (c) & 0.002 & 0.235 & 0.847 & 0.0 & 0.0 & 1.0 & 0.009 & 0.197 & 0.238\\
 \midrule
Optimal IV & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.076 & 0.0 & 0.073 & 0.0 & 0.0 & 0.0 & 0.198 & 0.005 & 0.239\\
OLS (s) & 0.353 & 0.133 & 0.069 & 0.208 & 0.208 & 0.0 & 0.194 & 0.001 & 0.24\\
Lasso (s) & 0.256 & 0.449 & 0.005 & 0.483 & 0.787 & 0.0 & 0.194 & 0.001 & 0.24\\
Ridge (s) & 0.315 & 0.419 & 0.006 & 0.309 & 0.006 & 0.0 & 0.194 & 0.001 & 0.24\\
XGB (c) & 0.0 & 0.0 & 0.848 & 0.0 & 0.0 & 1.0 & 0.197 & 0.004 & 0.238\\
 \midrule
Optimal IV (no LIE) & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$ & $D \vert X, Z$ & $D \vert X$ & $Y \vert X$\\
OLS & 0.077 & 0.0 & 0.075 & 0.0 & 0.0 & 0.0 & 0.198 & 0.198 & 0.239\\
OLS (s) & 0.359 & 0.327 & 0.064 & 0.247 & 0.174 & 0.0 & 0.194 & 0.195 & 0.24\\
Lasso (s) & 0.289 & 0.233 & 0.005 & 0.494 & 0.416 & 0.0 & 0.194 & 0.195 & 0.24\\
Ridge (s) & 0.276 & 0.205 & 0.011 & 0.258 & 0.41 & 0.0 & 0.194 & 0.195 & 0.24\\
XGB (c) & 0.0 & 0.235 & 0.845 & 0.0 & 0.0 & 1.0 & 0.197 & 0.197 & 0.238\\
\midrule\bottomrule 
\end{tabular}


==> Simul/R_simulations/pvw_sim_coef.tex <==
\begin{tabular}{rlcccrccc}
\toprule
\midrule
      &       & \multicolumn{3}{c}{$n_s = 9915$} &       & \multicolumn{3}{c}{$n_s = 99150$} \\
\cmidrule{3-5}\cmidrule{7-9}\multicolumn{2}{l}{\textit{Panel (A): Linear DGP}} & Bias  & MAB   & Rate  &       & Bias  & MAB   & Rate \\
      &       & (1)   & (2)   & (3)   &       & (4)   & (5)   & (6) \\\midrule
      & OLS   & -89.7 & 825.5 & 0.95  &       & -0.3  & 278.8 & 0.94 \\
\multicolumn{2}{l}{\underline{DDML:}} &       &       &       &       &       &       &  \\
      & cv-Lasso & -88.2 & 787.5 & 0.95  &       & -0.4  & 283.0 & 0.94 \\
      & Random forest & -212.4 & 977.3 & 0.88  &       & -45.9 & 370.7 & 0.84 \\
      & Gradient boosting & -103.6 & 797.5 & 0.95  &       & -7.2  & 274.0 & 0.94 \\
      & Ensemble (average) & -571.7 & 924.5 & 0.83  &       & 29.8  & 322.5 & 0.92 \\
      & Ensemble (stacking) & -112.5 & 851.0 & 0.94  &       & -2.5  & 278.0 & 0.94 \\
      & Ensemble (single-best) & -102.0 & 850.2 & 0.94  &       & -3.3  & 276.6 & 0.94 \\
      &       &       &       &       &       &       &       &  \\
      &       &       &       &       &       &       &       &  \\
\multicolumn{2}{l}{\textit{Panel (B): Non-Linear DGP}} & Bias  & MAB   & Rate  &       & Bias  & MAB   & Rate \\
      &       & (7)   & (8)   & (9)   &       & (10)  & (11)  & (12) \\\midrule
      & OLS   & -2580.0 & 2505.2 & 0.54  &       & -2599.4 & 2586.0 & 0.00 \\
\multicolumn{2}{l}{\underline{DDML:}} &       &       &       &       &       &       &  \\
      & cv-Lasso & -2615.7 & 2563.0 & 0.53  &       & -2604.0 & 2589.1 & 0.00 \\
      & Random forest & -249.5 & 1113.3 & 0.87  &       & -12.2 & 328.2 & 0.90 \\
      & Gradient boosting & -50.7 & 725.0 & 0.94  &       & -0.4  & 288.0 & 0.98 \\
      & Ensemble (average) & -717.8 & 1004.7 & 0.86  &       & -347.3 & 328.1 & 0.88 \\
      & Ensemble (stacking) & 248.8 & 834.5 & 0.94  &       & -1.2  & 283.3 & 0.98 \\
      & Ensemble (single-best) & -38.7 & 791.3 & 0.93  &       & -3.2  & 285.3 & 0.98 \\
\midrule
\bottomrule
\end{tabular}%


==> Simul/R_simulations/pvw_sim_weights.tex <==
\begin{tabular}{lccccc}
\toprule
\midrule
      & \multicolumn{2}{c}{Stacking} &       & \multicolumn{2}{c}{Single-Best} \\
\cmidrule{2-3}\cmidrule{5-6}\textit{Panel (A): Linear DGP} & $Y\vert X$ & $D\vert X$ &       & $Y\vert X$ & $D\vert X$ \\
      & (1)   & (2)   &       & (3)   & (4) \\
\midrule
OLS   & 0.06  & 0.29  &       & 0.00  & 0.23 \\
cv-Lasso & 0.35  & 0.17  &       & 0.47  & 0.27 \\
cv-Ridge & 0.35  & 0.17  &       & 0.43  & 0.27 \\
Series Lasso (w/o interactions) & 0.11  & 0.11  &       & 0.08  & 0.13 \\
Series Lasso (w/ interactions) & 0.07  & 0.13  &       & 0.02  & 0.09 \\
Random forest (low regularization) & 0.01  & 0.01  &       & 0.00  & 0.00 \\
Random forest (high regularization) & 0.01  & 0.01  &       & 0.00  & 0.00 \\
Gradient boosting (low regularization) & 0.03  & 0.05  &       & 0.00  & 0.01 \\
Gradient boosting (high regularization) & 0.02  & 0.05  &       & 0.00  & 0.01 \\
Neural Network & 0.00  & 0.00  &       & 0.00  & 0.00 \\
      &       &       &       &       &  \\
\textit{Panel (B): Non-Linear DGP} & $Y\vert X$ & $D\vert X$ &       & $Y\vert X$ & $D\vert X$ \\
      & (5)   & (6)   &       & (7)   & (8) \\
\midrule
OLS   & 0.00  & 0.02  &       & 0.00  & 0.00 \\
cv-Lasso & 0.01  & 0.00  &       & 0.00  & 0.00 \\
cv-Ridge & 0.01  & 0.00  &       & 0.00  & 0.00 \\
Series Lasso (w/o interactions) & 0.08  & 0.22  &       & 0.04  & 0.16 \\
Series Lasso (w/ interactions) & 0.31  & 0.30  &       & 0.25  & 0.35 \\
Random forest (low regularization) & 0.01  & 0.01  &       & 0.00  & 0.00 \\
Random forest (high regularization) & 0.01  & 0.01  &       & 0.00  & 0.00 \\
Gradient boosting (low regularization) & 0.30  & 0.23  &       & 0.35  & 0.26 \\
Gradient boosting (high regularization) & 0.29  & 0.20  &       & 0.37  & 0.23 \\
Neural Network & 0.00  & 0.00  &       & 0.00  & 0.00 \\
\midrule
\bottomrule
\end{tabular}%


==> Simul/not_selected.tex <==
1000&32951&.1&.1&1.7&895&415&417&415&902&900 \tabularnewline
1000&164755&.1&.1&1.7&258&769&769&769&258&258 \tabularnewline
1000&329509&.1&.1&1.7&2&618&618&618&2&2 \tabularnewline


==> Simul/simAK/not_selected.tex <==
1000&32951&.1&.1&1.7&895&415&417&415&902&900 \tabularnewline
1000&164755&.1&.1&1.7&258&769&769&769&258&258 \tabularnewline
1000&329509&.1&.1&1.7&2&618&618&618&2&2 \tabularnewline


==> Simul/simAK/sim_output_ddml.tex <==
&Lasso with CV&0.086&0.969&0.026&0.946&0.016&0.937 \tabularnewline
&Lasso with CV (all IVs)&0.114&0.970&0.026&0.959&0.013&0.943 \tabularnewline


==> Simul/simAK/sim_output_nolie.tex <==
&Lasso with CV&0.048&0.515&0.015&0.885&0.012&0.894 \tabularnewline
&Lasso with CV (all IVs)&1.303&0.785&0.271&0.017&0.078&0.087 \tabularnewline


==> Simul/simAK/sim_output_ref.tex <==
&TSLS&0.092&0.\phantom{000}&0.058&0.015&0.040&0.076 \tabularnewline
&TSLS (all IVs)&0.099&0.\phantom{000}&0.078&0.\phantom{000}&0.061&0.\phantom{000} \tabularnewline
&LIML&0.087&0.952&0.021&0.970&0.013&0.972 \tabularnewline
&LIML (all IVs)&0.077&0.964&0.014&0.970&0.007&0.966 \tabularnewline
&IV-Lasso&0.089&0.046&0.034&0.663&0.023&0.893 \tabularnewline
&IV-Lasso (all IVs)&0.089&0.226&0.076&0.129&0.066&0.254 \tabularnewline


==> Simul/sim_AE/artificialIV_dgp1.tex <==
&First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
&Index&-&0&.0012&.0127&.0092&.0002&.0092 \tabularnewline
&&(-)&(0)&(0)&(.0246)&(.0003)&(.0005)&(.0003) \tabularnewline
&Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline
&Weeks worked&--119.6848&33.8069&80.3055&36.4932&--83.1191&292.5573&--61.3623 \tabularnewline
&&(2864.082)&(3084.742)&(1277.043)&(514.9237)&(754.2967)&(6046.517)&(1154.677) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp1_all.tex <==
&First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
&Index&-&0&.0012&.0127&.0092&.0002&.0092 \tabularnewline
&&(-)&(0)&(0)&(.0246)&(.0003)&(.0005)&(.0003) \tabularnewline
&Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline
&Weeks worked&--119.6848&33.8069&80.3055&36.4932&--83.1191&292.5573&--61.3623 \tabularnewline
&&(2864.082)&(3084.742)&(1277.043)&(514.9237)&(754.2967)&(6046.517)&(1154.677) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp1_all_pres.tex <==
First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp1_pres.tex <==
First stage&.0004&.0004&.0005&.0035&-.0014&.0004&-.0014 \tabularnewline
&(.011)&(.011)&(.0109)&(.0127)&(.0055)&(.011)&(.0055) \tabularnewline
Employment&--2.6761&1.1148&2.481&1.1053&-.8519&6.8049&-.655 \tabularnewline
&(68.4474)&(35.1599)&(30.8941)&(19.6774)&(21.7516)&(140.802)&(19.196) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp2.tex <==
&First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
&Index&-&0&.0012&.0134&.0093&.0003&.0093 \tabularnewline
&&(-)&(0)&(0)&(.0248)&(.0003)&(.0009)&(.0003) \tabularnewline
&Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline
&Weeks worked&--5.2283&--5.2204&--4.7685&2.3651&-.7736&--5.1799&1.7544 \tabularnewline
&&(5.6945)&(5.7035)&(5.711)&(16.5527)&(6.3336)&(5.691)&(11.6248) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp2_all.tex <==
&First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
&Index&-&0&.0012&.0134&.0093&.0003&.0093 \tabularnewline
&&(-)&(0)&(0)&(.0248)&(.0003)&(.0009)&(.0003) \tabularnewline
&Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline
&Weeks worked&--5.2283&--5.2204&--4.7685&2.3651&-.7736&--5.1799&1.7544 \tabularnewline
&&(5.6945)&(5.7035)&(5.711)&(16.5527)&(6.3336)&(5.691)&(11.6248) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp2_all_pres.tex <==
First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp2_pres.tex <==
First stage&.0828&.0828&.0828&.0723&.0435&.0827&.0235 \tabularnewline
&(.0104)&(.0104)&(.0104)&(.0208)&(.0059)&(.0105)&(.0057) \tabularnewline
Employment&-.1119&-.1116&-.1039&.0235&-.1036&-.1119&-.1338 \tabularnewline
&(.1277)&(.1285)&(.1284)&(.3045)&(.1368)&(.1272)&(.2435) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp3.tex <==
&First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
&Index&-&0&-.0004&-.0003&0&-.0002&0 \tabularnewline
&&(-)&(0)&(.0005)&(.0004)&(.0003)&(.0003)&(.0001) \tabularnewline
&Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline
&Weeks worked&--5.6163&--5.6012&--5.6427&--5.7021&--5.6943&--5.6571&--7.9362 \tabularnewline
&&(4.2916)&(4.3211)&(4.3184)&(4.3223)&(4.3898)&(4.279)&(30.4164) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp3_all.tex <==
&First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
&Index&-&0&-.0004&-.0003&0&-.0002&0 \tabularnewline
&&(-)&(0)&(.0005)&(.0004)&(.0003)&(.0003)&(.0001) \tabularnewline
&Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline
&Weeks worked&--5.6163&--5.6012&--5.6427&--5.7021&--5.6943&--5.6571&--7.9362 \tabularnewline
&&(4.2916)&(4.3211)&(4.3184)&(4.3223)&(4.3898)&(4.279)&(30.4164) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp3_all_pres.tex <==
First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline


==> Simul/sim_AE/artificialIV_dgp3_pres.tex <==
First stage&.0693&.0693&.0693&.0693&.0692&.0693&4.122 \tabularnewline
&(.0066)&(.0066)&(.0066)&(.0066)&(.0068)&(.0066)&(2.6612) \tabularnewline
Employment&-.1286&-.1284&-.1302&-.1311&-.1294&-.1297&-.1849 \tabularnewline
&(.0987)&(.0989)&(.0988)&(.099)&(.102)&(.0982)&(.7653) \tabularnewline


==> Simul/sim_AE/pysw.tex <==
OLS&.401&.321&.449&.223&.832&.842 \tabularnewline
CV-Lasso&.365&.374&.26&.281&.144&.128 \tabularnewline
CV-Ridge&.014&.027&.018&.415&.022&.029 \tabularnewline
XGBoost-c&.22&.278&.273&.082&.001&.002 \tabularnewline


==> Simul/sim_Advantages/sim_mspe_grad.tex <==
&OLS&3.685&0.203&&3.673&0.203 \tabularnewline
&Lasso with CV (2nd order poly)&3.482&0.201&&3.451&0.200 \tabularnewline
&Ridge with CV (2nd order poly)&3.480&0.201&&3.450&0.200 \tabularnewline
&Lasso with CV (10th order poly)&5.955&0.225&&3.423&0.200 \tabularnewline
&Ridge with CV (10th order poly)&7.062&0.235&&3.425&0.200 \tabularnewline
&Random forest (low regularization)&3.795&0.231&&3.515&0.236 \tabularnewline
&Random forest (high regularization)&3.591&0.204&&3.252&0.205 \tabularnewline
&Gradient boosting (low regularization)&3.353&0.200&&3.095&0.198 \tabularnewline
&Gradient boosting (high regularization)&3.405&0.200&&3.216&0.199 \tabularnewline
&Neural net&1.433&0.174&&1.618&0.175 \tabularnewline


==> Simul/sim_Advantages/sim_mspe_ols.tex <==
&OLS&3.095&0.200&&3.089&0.200 \tabularnewline
&Lasso with CV (2nd order poly)&3.097&0.200&&3.089&0.200 \tabularnewline
&Ridge with CV (2nd order poly)&3.101&0.200&&3.089&0.200 \tabularnewline
&Lasso with CV (10th order poly)&3.213&0.202&&3.095&0.200 \tabularnewline
&Ridge with CV (10th order poly)&3.347&0.205&&3.094&0.200 \tabularnewline
&Random forest (low regularization)&3.613&0.233&&3.699&0.239 \tabularnewline
&Random forest (high regularization)&3.183&0.205&&3.197&0.207 \tabularnewline
&Gradient boosting (low regularization)&3.131&0.201&&3.102&0.200 \tabularnewline
&Gradient boosting (high regularization)&3.152&0.202&&3.138&0.200 \tabularnewline
&Neural net&1.238&0.167&&1.248&0.168 \tabularnewline


==> Simul/sim_Advantages/sim_output_dgp0_long.tex <==
&OLS&-24.8&820.2&0.95&&-1.9&269.1&0.95 \tabularnewline
&PDS-Lasso&-25.4&821.2&0.95&&0.6&269.4&0.95 \tabularnewline
&OLS&-30.5&826.8&0.95&&-2.3&270.5&0.95 \tabularnewline
&Lasso with CV (2nd order poly)&-28.5&830.2&0.96&&-1.5&272.6&0.95 \tabularnewline
&Ridge with CV (2nd order poly)&-25.5&821.1&0.95&&-1.9&275.9&0.95 \tabularnewline
&Lasso with CV (10th order poly)&187.4&1047.6&0.95&&61.4&281.7&0.94 \tabularnewline
&Ridge with CV (10th order poly)&1069.3&1221.0&0.94&&38.1&273.4&0.94 \tabularnewline
&Random forest (low regularization)&-196.5&982.2&0.91&&-33.3&356.7&0.87 \tabularnewline
&Random forest (high regularization)&-28.1&853.1&0.95&&-22.5&288.7&0.94 \tabularnewline
&Gradient boosting (low regularization)&-82.2&825.0&0.95&&-19.4&270.9&0.95 \tabularnewline
&Gradient boosting (high regularization)&28.6&819.6&0.96&&71.4&279.8&0.94 \tabularnewline
&Neural net&309.2&866.0&0.94&&17.4&288.1&0.94 \tabularnewline
&Stacking: CLS&8.8&829.3&0.95&&-1.5&274.4&0.95 \tabularnewline
&Stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95 \tabularnewline
&Stacking: OLS&-33.7&874.1&0.94&&2.6&272.0&0.95 \tabularnewline
&Stacking: Single-best&-28.6&823.3&0.96&&-3.5&272.1&0.95 \tabularnewline
&Short-stacking: CLS&-23.8&817.6&0.96&&-1.5&274.3&0.95 \tabularnewline
&Short-stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95 \tabularnewline
&Short-stacking: OLS&-27.9&818.1&0.96&&-2.4&274.4&0.95 \tabularnewline
&Short-stacking: Single-best&-20.7&826.0&0.96&&-3.4&272.4&0.95 \tabularnewline
&Short-stacking: CLS 2&-33.3&819.9&0.95&&-2.2&273.2&0.95 \tabularnewline
&Short-stacking: Single-best 2&-31.3&823.0&0.96&&-4.2&276.0&0.95 \tabularnewline
&Pooled stacking: CLS&-24.8&817.8&0.96&&-1.5&273.4&0.95 \tabularnewline
&Pooled stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95 \tabularnewline
&Pooled stacking: OLS&-48.1&834.6&0.95&&-2.2&272.1&0.95 \tabularnewline
&Pooled stacking: Single-best&-23.0&829.7&0.96&&-3.3&270.9&0.95 \tabularnewline


==> Simul/sim_Advantages/sim_output_dgp1_long.tex <==
&OLS&-2587.3&2642.4&0.58&&-2644.9&2640.5&0.\phantom{00} \tabularnewline
&PDS-Lasso&-2598.4&2661.3&0.57&&-2644.1&2638.4&0.\phantom{00} \tabularnewline
&OLS&-2617.9&2622.6&0.58&&-2647.2&2645.8&0.\phantom{00} \tabularnewline
&Lasso with CV (2nd order poly)&746.2&1105.5&0.89&&703.5&714.6&0.61 \tabularnewline
&Ridge with CV (2nd order poly)&801.9&1143.6&0.89&&714.3&725.3&0.60 \tabularnewline
&Lasso with CV (10th order poly)&-4684.7&2111.1&0.90&&-2.1&284.5&0.94 \tabularnewline
&Ridge with CV (10th order poly)&-3070.8&2499.6&0.87&&-1.9&287.5&0.95 \tabularnewline
&Random forest (low regularization)&-64.0&1065.0&0.90&&-43.4&331.8&0.87 \tabularnewline
&Random forest (high regularization)&-133.0&932.3&0.94&&-18.5&272.8&0.94 \tabularnewline
&Gradient boosting (low regularization)&52.4&924.3&0.93&&13.6&267.7&0.95 \tabularnewline
&Gradient boosting (high regularization)&199.8&895.4&0.94&&182.3&319.3&0.93 \tabularnewline
&Neural net&-620.3&1103.6&0.91&&-142.9&292.0&0.92 \tabularnewline
&Stacking: CLS&226.8&1129.3&0.93&&24.9&262.9&0.95 \tabularnewline
&Stacking: Average&-101.7&1102.7&0.93&&60.0&271.9&0.95 \tabularnewline
&Stacking: OLS&871.4&1264.7&0.93&&26.6&265.7&0.94 \tabularnewline
&Stacking: Single-best&179.2&1016.2&0.92&&15.0&266.4&0.95 \tabularnewline
&Short-stacking: CLS&221.9&897.3&0.93&&21.9&261.7&0.95 \tabularnewline
&Short-stacking: Average&-101.7&1102.7&0.93&&60.0&271.9&0.95 \tabularnewline
&Short-stacking: OLS&169.0&888.2&0.93&&15.8&262.5&0.94 \tabularnewline
&Short-stacking: Single-best&116.1&900.1&0.94&&15.0&266.4&0.95 \tabularnewline
&Short-stacking: CLS 2&203.8&892.2&0.93&&18.0&263.1&0.95 \tabularnewline
&Short-stacking: Single-best 2&99.6&906.8&0.93&&13.6&267.7&0.95 \tabularnewline
&Pooled stacking: CLS&251.5&960.1&0.93&&24.8&264.8&0.95 \tabularnewline
&Pooled stacking: Average&-101.7&1102.7&0.93&&60.0&271.9&0.95 \tabularnewline
&Pooled stacking: OLS&376.8&1068.3&0.93&&16.7&266.5&0.94 \tabularnewline
&Pooled stacking: Single-best&131.0&952.0&0.93&&15.0&266.4&0.95 \tabularnewline


==> Simul/sim_Advantages/sim_output_folds2.tex <==
&OLS&-24.8&820.2&0.95&&-1.9&269.1&0.95&&-2587.3&2642.4&0.95&&-2644.9&2640.5&0.\phantom{00} \tabularnewline
&PDS-Lasso&-25.4&821.2&0.95&&0.6&269.4&0.95&&-2598.4&2661.3&0.95&&-2644.1&2638.4&0.\phantom{00} \tabularnewline
&OLS&-30.5&826.8&0.95&&-2.3&270.5&0.95&&-2617.9&2622.6&0.95&&-2647.2&2645.8&0.\phantom{00} \tabularnewline
&Lasso with CV (2nd order poly)&-28.5&830.2&0.96&&-1.5&272.6&0.95&&746.2&1105.5&0.96&&703.5&714.6&0.61 \tabularnewline
&Ridge with CV (2nd order poly)&-25.5&821.1&0.95&&-1.9&275.9&0.95&&801.9&1143.6&0.95&&714.3&725.3&0.60 \tabularnewline
&Lasso with CV (10th order poly)&187.4&1047.6&0.95&&61.4&281.7&0.94&&-4684.7&2111.1&0.95&&-2.1&284.5&0.94 \tabularnewline
&Ridge with CV (10th order poly)&1069.3&1221.0&0.94&&38.1&273.4&0.94&&-3070.8&2499.6&0.94&&-1.9&287.5&0.95 \tabularnewline
&Random forest (low regularization)&-196.5&982.2&0.91&&-33.3&356.7&0.87&&-64.0&1065.0&0.91&&-43.4&331.8&0.87 \tabularnewline
&Random forest (high regularization)&-28.1&853.1&0.95&&-22.5&288.7&0.94&&-133.0&932.3&0.95&&-18.5&272.8&0.94 \tabularnewline
&Gradient boosting (low regularization)&-82.2&825.0&0.95&&-19.4&270.9&0.95&&52.4&924.3&0.95&&13.6&267.7&0.95 \tabularnewline
&Gradient boosting (high regularization)&28.6&819.6&0.96&&71.4&279.8&0.94&&199.8&895.4&0.96&&182.3&319.3&0.93 \tabularnewline
&Neural net&309.2&866.0&0.94&&17.4&288.1&0.94&&-620.3&1103.6&0.94&&-142.9&292.0&0.92 \tabularnewline
&Stacking: CLS&8.8&829.3&0.95&&-1.5&274.4&0.95&&226.8&1129.3&0.95&&24.9&262.9&0.95 \tabularnewline
&Stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95&&-101.7&1102.7&0.94&&60.0&271.9&0.95 \tabularnewline
&Stacking: OLS&-33.7&874.1&0.94&&2.6&272.0&0.95&&871.4&1264.7&0.94&&26.6&265.7&0.94 \tabularnewline
&Stacking: Single-best&-28.6&823.3&0.96&&-3.5&272.1&0.95&&179.2&1016.2&0.96&&15.0&266.4&0.95 \tabularnewline
&Short-stacking: CLS&-23.8&817.6&0.96&&-1.5&274.3&0.95&&221.9&897.3&0.96&&21.9&261.7&0.95 \tabularnewline
&Short-stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95&&-101.7&1102.7&0.94&&60.0&271.9&0.95 \tabularnewline
&Short-stacking: OLS&-27.9&818.1&0.96&&-2.4&274.4&0.95&&169.0&888.2&0.96&&15.8&262.5&0.94 \tabularnewline
&Short-stacking: Single-best&-20.7&826.0&0.96&&-3.4&272.4&0.95&&116.1&900.1&0.96&&15.0&266.4&0.95 \tabularnewline
&Short-stacking: CLS 2&-33.3&819.9&0.95&&-2.2&273.2&0.95&&203.8&892.2&0.95&&18.0&263.1&0.95 \tabularnewline
&Short-stacking: Single-best 2&-31.3&823.0&0.96&&-4.2&276.0&0.95&&99.6&906.8&0.96&&13.6&267.7&0.95 \tabularnewline
&Pooled stacking: CLS&-24.8&817.8&0.96&&-1.5&273.4&0.95&&251.5&960.1&0.96&&24.8&264.8&0.95 \tabularnewline
&Pooled stacking: Average&-0.1&812.9&0.94&&1.4&273.7&0.95&&-101.7&1102.7&0.94&&60.0&271.9&0.95 \tabularnewline
&Pooled stacking: OLS&-48.1&834.6&0.95&&-2.2&272.1&0.95&&376.8&1068.3&0.95&&16.7&266.5&0.94 \tabularnewline
&Pooled stacking: Single-best&-23.0&829.7&0.96&&-3.3&270.9&0.95&&131.0&952.0&0.96&&15.0&266.4&0.95 \tabularnewline


==> Simul/sim_Advantages/sim_small_bias_wide_folds10.tex <==
&OLS&-246.2&-297.0&248.3&161.8&-20.2&&-2291.4&-2023.2&-2631.2&-2857.2&-2582.1 \tabularnewline
&PDS-Lasso&-1247.5&-1001.1&-159.3&72.0&-18.7&&-2143.2&-2524.0&-3105.3&-3120.1&-2591.5 \tabularnewline
&OLS&-282.8&-308.6&255.4&164.3&-19.9&&-2833.5&-2364.7&-2861.6&-2952.6&-2600.8 \tabularnewline
&Lasso with CV (2nd order poly)&-236.3&-206.1&277.8&174.3&-19.6&&-912.8&-163.8&-82.8&264.4&754.2 \tabularnewline
&Ridge with CV (2nd order poly)&-144.7&-187.2&303.5&151.2&-22.0&&-1803.8&-728.0&122.1&697.7&778.0 \tabularnewline
&Lasso with CV (10th order poly)&6339.9&180.0&1258.7&565.9&2.4&&-7471.8&-3768.5&182.8&4054.5&-951.6 \tabularnewline
&Ridge with CV (10th order poly)&5321.1&4716.5&6706.9&89.8&290.3&&691.7&3137.6&-6506.9&-8867.9&515.8 \tabularnewline
&Random forest (low regularization)&-149.1&-337.2&162.3&78.1&-110.7&&-274.3&233.1&-448.8&-293.4&-15.0 \tabularnewline
&Random forest (high regularization)&633.6&132.6&454.7&288.4&-15.3&&-381.2&185.4&-361.3&-313.4&-74.3 \tabularnewline
&Gradient boosting (low regularization)&-489.1&-498.4&125.6&113.6&-53.5&&-539.0&182.4&-348.5&-209.5&59.7 \tabularnewline
&Gradient boosting (high regularization)&-240.3&-284.2&291.9&257.5&40.8&&-316.7&329.6&-159.4&-32.6&213.5 \tabularnewline
&Neural net&3554.5&3955.7&3570.1&2153.1&129.7&&1277.7&2089.6&1354.8&-132.9&-465.6 \tabularnewline
&Stacking: CLS&96.2&-1300.3&169.5&118.2&-24.9&&-452.0&-1706.0&-1216.1&-73.8&188.5 \tabularnewline
&Stacking: Average&1397.1&386.9&699.9&358.8&-8.2&&650.8&-40.4&-827.2&839.1&339.1 \tabularnewline
&Stacking: OLS&2.1e7&-4686.3&-40.3&-754.1&-125.4&&4.2e6&7211.7&-961.5&-3472.6&253.7 \tabularnewline
&Stacking: Single-best&-366.2&-1414.4&185.2&124.6&-25.2&&-1774.8&-313.1&-622.0&-708.9&112.6 \tabularnewline
&Short-stacking: CLS&-179.0&-258.7&306.6&185.3&-23.0&&-462.7&55.0&-124.6&18.4&138.8 \tabularnewline
&Short-stacking: Average&1397.1&386.9&699.9&358.8&-8.2&&650.8&-40.4&-827.2&839.1&339.1 \tabularnewline
&Short-stacking: OLS&-436.2&-438.4&159.2&119.6&-26.6&&-491.7&-47.8&-228.7&-51.8&103.8 \tabularnewline
&Short-stacking: Single-best&-308.2&-321.7&246.8&148.5&-22.6&&-681.2&-149.9&-217.6&36.4&55.3 \tabularnewline
&Short-stacking: CLS 2&-152.1&-241.5&316.8&190.4&-21.9&&-417.8&97.6&-154.5&17.7&147.1 \tabularnewline
&Short-stacking: Single-best 2&-236.0&-304.9&259.7&158.4&-21.1&&-728.0&-108.6&-179.5&17.7&65.7 \tabularnewline
&Pooled stacking: CLS&-127.3&-192.6&328.1&172.0&-23.3&&-688.8&-70.8&-353.6&-60.2&160.4 \tabularnewline
&Pooled stacking: Average&1397.1&386.9&699.9&358.8&-8.2&&650.8&-40.4&-827.2&839.1&339.1 \tabularnewline
&Pooled stacking: OLS&-295.6&-403.0&229.2&133.8&-24.9&&-625.1&-240.7&-556.9&-221.0&128.4 \tabularnewline
&Pooled stacking: Single-best&-236.5&-341.1&242.8&156.2&-22.5&&-797.4&-215.0&-329.1&13.0&53.6 \tabularnewline


==> Simul/sim_Advantages/sim_small_bias_wide_folds2.tex <==
&OLS&335.4&-195.9&-30.1&-133.4&-24.8&&-2797.6&-2727.5&-2552.2&-2679.7&-2587.3 \tabularnewline
&PDS-Lasso&-596.0&-937.4&-417.4&-229.7&-25.4&&-2894.2&-3329.5&-2986.3&-2970.2&-2598.4 \tabularnewline
&OLS&430.2&-193.4&-30.8&-99.1&-30.5&&-3707.2&-3104.0&-2763.0&-2783.6&-2617.9 \tabularnewline
&Lasso with CV (2nd order poly)&817.0&-19.7&66.0&-76.8&-28.5&&-1395.9&-848.0&-419.8&94.2&746.2 \tabularnewline
&Ridge with CV (2nd order poly)&733.4&-49.6&76.5&-92.4&-25.5&&-2186.6&-1686.8&-830.0&462.4&801.9 \tabularnewline
&Lasso with CV (10th order poly)&1316.1&4638.4&-2105.4&1816.9&187.4&&13719.1&14971.8&-4231.1&-2089.5&-4684.7 \tabularnewline
&Ridge with CV (10th order poly)&-439.7&10587.2&2331.6&3567.1&1069.3&&1555.4&-2129.9&10583.9&-6898.8&-3070.8 \tabularnewline
&Random forest (low regularization)&555.5&-320.3&-112.4&-220.7&-196.5&&-545.3&-94.9&-96.0&-251.8&-64.0 \tabularnewline
&Random forest (high regularization)&2478.4&564.3&335.9&108.2&-28.1&&-45.4&-196.6&-202.1&-188.9&-133.0 \tabularnewline
&Gradient boosting (low regularization)&50.1&-632.3&-159.8&-216.7&-82.2&&-762.7&-276.5&-209.9&-215.9&52.4 \tabularnewline
&Gradient boosting (high regularization)&248.1&-307.0&81.1&-35.9&28.6&&-535.5&-75.8&48.9&-29.5&199.8 \tabularnewline
&Neural net&4141.4&3780.5&4275.4&3359.1&309.2&&1837.4&2111.0&2110.2&1267.0&-620.3 \tabularnewline
&Stacking: CLS&3032.5&1043.6&-618.3&-104.4&8.8&&109.3&-638.7&-275.4&-1462.4&226.8 \tabularnewline
&Stacking: Average&1208.6&-1048.4&46.3&-224.1&-0.1&&1375.0&-1671.6&1046.9&-580.7&-101.7 \tabularnewline
&Stacking: OLS&-3363.0&-8220.1&-4066.3&-1563.1&-33.7&&6.1e7&4.1e7&722.7&-920.4&871.4 \tabularnewline
&Stacking: Single-best&1496.3&-348.9&-111.6&-206.4&-28.6&&-2024.5&-746.4&-38.9&-95.9&179.2 \tabularnewline
&Short-stacking: CLS&730.8&-58.7&25.6&-117.5&-23.8&&-518.0&-382.4&-302.4&-54.6&221.9 \tabularnewline
&Short-stacking: Average&1208.6&-1048.4&46.3&-224.1&-0.1&&1375.0&-1671.6&1046.9&-580.7&-101.7 \tabularnewline
&Short-stacking: OLS&214.9&-261.7&-101.8&-203.7&-27.9&&-554.4&-434.5&-218.4&-96.4&169.0 \tabularnewline
&Short-stacking: Single-best&454.5&-186.4&-33.7&-172.1&-20.7&&-966.8&-665.8&-460.4&-72.0&116.1 \tabularnewline
&Short-stacking: CLS 2&739.6&-103.5&50.9&-55.3&-33.3&&-407.6&-374.2&-245.9&-76.0&203.8 \tabularnewline
&Short-stacking: Single-best 2&497.6&-177.9&10.3&-106.2&-31.3&&-792.8&-556.6&-450.2&-136.1&99.6 \tabularnewline
&Pooled stacking: CLS&827.4&160.8&317.8&-37.1&-24.8&&-719.8&-5280.9&488.6&207.5&251.5 \tabularnewline
&Pooled stacking: Average&1208.6&-1048.4&46.3&-224.1&-0.1&&1375.0&-1671.6&1046.9&-580.7&-101.7 \tabularnewline
&Pooled stacking: OLS&389.2&-1403.6&613.3&-40.9&-48.1&&-14589.5&-6679.2&-4064.4&201.4&376.8 \tabularnewline
&Pooled stacking: Single-best&953.6&-334.9&-17.0&-170.8&-23.0&&-1323.5&-2172.3&-1216.1&109.9&131.0 \tabularnewline


==> Simul/sim_Advantages/sim_small_cover_wide_folds10.tex <==
&OLS&0.95&0.95&0.96&0.96&0.95&&0.94&0.95&0.92&0.91&0.59 \tabularnewline
&PDS-Lasso&0.94&0.95&0.95&0.95&0.95&&0.94&0.95&0.91&0.89&0.59 \tabularnewline
&OLS&0.94&0.95&0.95&0.95&0.95&&0.93&0.94&0.93&0.91&0.59 \tabularnewline
&Lasso with CV (2nd order poly)&0.95&0.95&0.95&0.95&0.95&&0.95&0.95&0.95&0.95&0.90 \tabularnewline
&Ridge with CV (2nd order poly)&0.95&0.95&0.95&0.95&0.95&&0.95&0.95&0.95&0.94&0.89 \tabularnewline
&Lasso with CV (10th order poly)&0.90&0.92&0.93&0.93&0.95&&0.87&0.85&0.85&0.88&0.95 \tabularnewline
&Ridge with CV (10th order poly)&0.81&0.89&0.87&0.89&0.95&&0.82&0.82&0.83&0.87&0.94 \tabularnewline
&Random forest (low regularization)&0.92&0.92&0.93&0.92&0.91&&0.93&0.92&0.93&0.93&0.91 \tabularnewline
&Random forest (high regularization)&0.95&0.95&0.95&0.95&0.94&&0.95&0.95&0.95&0.95&0.93 \tabularnewline
&Gradient boosting (low regularization)&0.92&0.93&0.94&0.94&0.95&&0.92&0.93&0.95&0.96&0.94 \tabularnewline
&Gradient boosting (high regularization)&0.93&0.94&0.95&0.95&0.95&&0.94&0.94&0.96&0.96&0.94 \tabularnewline
&Neural net&0.94&0.92&0.90&0.91&0.95&&0.94&0.95&0.95&0.97&0.94 \tabularnewline
&Stacking: CLS&0.93&0.94&0.95&0.95&0.95&&0.94&0.93&0.94&0.94&0.94 \tabularnewline
&Stacking: Average&0.93&0.94&0.95&0.94&0.95&&0.91&0.92&0.93&0.95&0.94 \tabularnewline
&Stacking: OLS&0.84&0.89&0.91&0.92&0.93&&0.83&0.85&0.86&0.90&0.93 \tabularnewline
&Stacking: Single-best&0.93&0.94&0.95&0.95&0.95&&0.94&0.95&0.95&0.94&0.94 \tabularnewline
&Short-stacking: CLS&0.95&0.95&0.96&0.95&0.95&&0.96&0.96&0.95&0.95&0.94 \tabularnewline
&Short-stacking: Average&0.93&0.94&0.95&0.94&0.95&&0.91&0.92&0.93&0.95&0.94 \tabularnewline
&Short-stacking: OLS&0.95&0.95&0.96&0.95&0.95&&0.95&0.96&0.95&0.95&0.94 \tabularnewline
&Short-stacking: Single-best&0.95&0.95&0.96&0.95&0.95&&0.95&0.96&0.95&0.94&0.94 \tabularnewline
&Short-stacking: CLS 2&0.95&0.95&0.95&0.95&0.95&&0.95&0.95&0.96&0.95&0.94 \tabularnewline
&Short-stacking: Single-best 2&0.95&0.95&0.95&0.95&0.95&&0.95&0.95&0.96&0.96&0.94 \tabularnewline
&Pooled stacking: CLS&0.95&0.95&0.96&0.95&0.95&&0.96&0.95&0.96&0.96&0.94 \tabularnewline
&Pooled stacking: Average&0.93&0.94&0.95&0.94&0.95&&0.91&0.92&0.93&0.95&0.94 \tabularnewline
&Pooled stacking: OLS&0.95&0.95&0.96&0.95&0.95&&0.95&0.96&0.95&0.95&0.94 \tabularnewline
&Pooled stacking: Single-best&0.95&0.95&0.96&0.95&0.95&&0.95&0.96&0.95&0.95&0.94 \tabularnewline


==> Simul/sim_Advantages/sim_small_cover_wide_folds2.tex <==
&OLS&0.95&0.96&0.93&0.95&0.95&&0.94&0.95&0.93&0.91&0.58 \tabularnewline
&PDS-Lasso&0.95&0.96&0.93&0.95&0.95&&0.93&0.95&0.93&0.90&0.57 \tabularnewline
&OLS&0.90&0.93&0.92&0.94&0.95&&0.88&0.93&0.91&0.91&0.58 \tabularnewline
&Lasso with CV (2nd order poly)&0.93&0.94&0.93&0.94&0.96&&0.92&0.95&0.94&0.94&0.89 \tabularnewline
&Ridge with CV (2nd order poly)&0.94&0.95&0.93&0.94&0.95&&0.93&0.95&0.94&0.93&0.89 \tabularnewline
&Lasso with CV (10th order poly)&0.86&0.88&0.88&0.92&0.95&&0.85&0.84&0.82&0.84&0.90 \tabularnewline
&Ridge with CV (10th order poly)&0.72&0.76&0.82&0.84&0.94&&0.73&0.79&0.80&0.81&0.87 \tabularnewline
&Random forest (low regularization)&0.91&0.92&0.90&0.92&0.91&&0.89&0.93&0.92&0.94&0.90 \tabularnewline
&Random forest (high regularization)&0.93&0.95&0.92&0.95&0.95&&0.93&0.95&0.95&0.95&0.94 \tabularnewline
&Gradient boosting (low regularization)&0.90&0.92&0.92&0.94&0.95&&0.89&0.93&0.93&0.95&0.93 \tabularnewline
&Gradient boosting (high regularization)&0.92&0.94&0.93&0.95&0.96&&0.91&0.94&0.94&0.95&0.94 \tabularnewline
&Neural net&0.88&0.83&0.80&0.81&0.94&&0.92&0.89&0.90&0.91&0.91 \tabularnewline
&Stacking: CLS&0.90&0.94&0.91&0.94&0.95&&0.92&0.93&0.93&0.94&0.93 \tabularnewline
&Stacking: Average&0.89&0.93&0.91&0.94&0.94&&0.89&0.92&0.92&0.93&0.93 \tabularnewline
&Stacking: OLS&0.70&0.80&0.86&0.90&0.94&&0.68&0.80&0.85&0.87&0.93 \tabularnewline
&Stacking: Single-best&0.92&0.95&0.91&0.94&0.96&&0.92&0.94&0.94&0.95&0.92 \tabularnewline
&Short-stacking: CLS&0.93&0.95&0.92&0.95&0.96&&0.93&0.95&0.94&0.96&0.93 \tabularnewline
&Short-stacking: Average&0.89&0.93&0.91&0.94&0.94&&0.89&0.92&0.92&0.93&0.93 \tabularnewline
&Short-stacking: OLS&0.95&0.96&0.93&0.95&0.96&&0.94&0.95&0.94&0.95&0.93 \tabularnewline
&Short-stacking: Single-best&0.93&0.95&0.92&0.94&0.96&&0.93&0.96&0.94&0.96&0.94 \tabularnewline
&Short-stacking: CLS 2&0.94&0.94&0.92&0.95&0.95&&0.94&0.95&0.94&0.95&0.93 \tabularnewline
&Short-stacking: Single-best 2&0.94&0.94&0.93&0.95&0.96&&0.94&0.95&0.94&0.95&0.93 \tabularnewline
&Pooled stacking: CLS&0.93&0.95&0.92&0.95&0.96&&0.93&0.94&0.94&0.95&0.93 \tabularnewline
&Pooled stacking: Average&0.89&0.93&0.91&0.94&0.94&&0.89&0.92&0.92&0.93&0.93 \tabularnewline
&Pooled stacking: OLS&0.88&0.92&0.90&0.93&0.95&&0.87&0.88&0.91&0.93&0.93 \tabularnewline
&Pooled stacking: Single-best&0.93&0.95&0.91&0.94&0.96&&0.93&0.95&0.95&0.95&0.93 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_grad.tex <==
OLS&0.011&0.015&&0.007&0.013&&0.004&0.010 \tabularnewline
Lasso with CV (2nd order poly)&0.036&0.059&&0.028&0.054&&0.016&0.038 \tabularnewline
Ridge with CV (2nd order poly)&0.153&0.231&&0.185&0.267&&0.123&0.230 \tabularnewline
Lasso with CV (10th order poly)&0.060&0.076&&0.051&0.068&&0.052&0.063 \tabularnewline
Ridge with CV (10th order poly)&0.074&0.061&&0.063&0.027&&0.061&0.056 \tabularnewline
Random forest (low regularization)&0.042&0.012&&0.041&0.007&&0.043&0.006 \tabularnewline
Random forest (high regularization)&0.021&0.076&&0.010&0.073&&0.014&0.063 \tabularnewline
Gradient boosting (low regularization)&0.523&0.229&&0.552&0.250&&0.615&0.346 \tabularnewline
Gradient boosting (high regularization)&0.014&0.192&&0.005&0.201&&0.005&0.139 \tabularnewline
Neural net&0.067&0.049&&0.059&0.040&&0.066&0.050 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_grad_large.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (2nd order poly)&0.\phantom{000}&0.034&&0.\phantom{000}&0.035&&0.\phantom{000}&0.026 \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.001&&0.\phantom{000}&0.001&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.038&&0.\phantom{000}&0.037&&0.\phantom{000}&0.027 \tabularnewline
Random forest (low regularization)&0.153&0.003&&0.154&0.001&&0.180&0.001 \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.061&&0.\phantom{000}&0.065&&0.\phantom{000}&0.070 \tabularnewline
Gradient boosting (low regularization)&0.845&0.852&&0.846&0.856&&0.820&0.870 \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.002&0.011&&0.\phantom{000}&0.006&&0.\phantom{000}&0.006 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_grad_large_nopooled.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (2nd order poly)&0.\phantom{000}&0.034&&0.\phantom{000}&0.026 \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.001&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.038&&0.\phantom{000}&0.027 \tabularnewline
Random forest (low regularization)&0.153&0.003&&0.180&0.001 \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.061&&0.\phantom{000}&0.070 \tabularnewline
Gradient boosting (low regularization)&0.845&0.852&&0.820&0.870 \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.002&0.011&&0.\phantom{000}&0.006 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_grad_nopooled.tex <==
OLS&0.011&0.015&&0.004&0.010 \tabularnewline
Lasso with CV (2nd order poly)&0.036&0.059&&0.016&0.038 \tabularnewline
Ridge with CV (2nd order poly)&0.153&0.231&&0.123&0.230 \tabularnewline
Lasso with CV (10th order poly)&0.060&0.076&&0.052&0.063 \tabularnewline
Ridge with CV (10th order poly)&0.074&0.061&&0.061&0.056 \tabularnewline
Random forest (low regularization)&0.042&0.012&&0.043&0.006 \tabularnewline
Random forest (high regularization)&0.021&0.076&&0.014&0.063 \tabularnewline
Gradient boosting (low regularization)&0.523&0.229&&0.615&0.346 \tabularnewline
Gradient boosting (high regularization)&0.014&0.192&&0.005&0.139 \tabularnewline
Neural net&0.067&0.049&&0.066&0.050 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_ols.tex <==
OLS&0.680&0.494&&0.749&0.570&&0.677&0.485 \tabularnewline
Lasso with CV (2nd order poly)&0.096&0.138&&0.087&0.123&&0.114&0.135 \tabularnewline
Ridge with CV (2nd order poly)&0.068&0.058&&0.048&0.042&&0.080&0.069 \tabularnewline
Lasso with CV (10th order poly)&0.030&0.074&&0.020&0.065&&0.022&0.076 \tabularnewline
Ridge with CV (10th order poly)&0.028&0.043&&0.016&0.024&&0.027&0.055 \tabularnewline
Random forest (low regularization)&0.013&0.011&&0.010&0.007&&0.008&0.007 \tabularnewline
Random forest (high regularization)&0.018&0.028&&0.013&0.022&&0.012&0.024 \tabularnewline
Gradient boosting (low regularization)&0.028&0.045&&0.021&0.037&&0.025&0.043 \tabularnewline
Gradient boosting (high regularization)&0.020&0.062&&0.021&0.072&&0.019&0.061 \tabularnewline
Neural net&0.019&0.047&&0.014&0.038&&0.016&0.044 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_ols_large.tex <==
OLS&0.768&0.329&&0.820&0.349&&0.768&0.287 \tabularnewline
Lasso with CV (2nd order poly)&0.069&0.021&&0.057&0.011&&0.069&0.015 \tabularnewline
Ridge with CV (2nd order poly)&0.072&0.041&&0.057&0.028&&0.093&0.051 \tabularnewline
Lasso with CV (10th order poly)&0.016&0.206&&0.013&0.221&&0.012&0.198 \tabularnewline
Ridge with CV (10th order poly)&0.023&0.112&&0.017&0.098&&0.020&0.128 \tabularnewline
Random forest (low regularization)&0.003&0.003&&0.002&0.002&&0.002&0.002 \tabularnewline
Random forest (high regularization)&0.007&0.009&&0.005&0.006&&0.005&0.006 \tabularnewline
Gradient boosting (low regularization)&0.018&0.162&&0.014&0.178&&0.013&0.190 \tabularnewline
Gradient boosting (high regularization)&0.004&0.007&&0.003&0.004&&0.002&0.002 \tabularnewline
Neural net&0.020&0.110&&0.011&0.104&&0.015&0.122 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_ols_large_nopooled.tex <==
OLS&0.768&0.329&&0.768&0.287 \tabularnewline
Lasso with CV (2nd order poly)&0.069&0.021&&0.069&0.015 \tabularnewline
Ridge with CV (2nd order poly)&0.072&0.041&&0.093&0.051 \tabularnewline
Lasso with CV (10th order poly)&0.016&0.206&&0.012&0.198 \tabularnewline
Ridge with CV (10th order poly)&0.023&0.112&&0.020&0.128 \tabularnewline
Random forest (low regularization)&0.003&0.003&&0.002&0.002 \tabularnewline
Random forest (high regularization)&0.007&0.009&&0.005&0.006 \tabularnewline
Gradient boosting (low regularization)&0.018&0.162&&0.013&0.190 \tabularnewline
Gradient boosting (high regularization)&0.004&0.007&&0.002&0.002 \tabularnewline
Neural net&0.020&0.110&&0.015&0.122 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_ols_nopooled.tex <==
OLS&0.680&0.494&&0.677&0.485 \tabularnewline
Lasso with CV (2nd order poly)&0.096&0.138&&0.114&0.135 \tabularnewline
Ridge with CV (2nd order poly)&0.068&0.058&&0.080&0.069 \tabularnewline
Lasso with CV (10th order poly)&0.030&0.074&&0.022&0.076 \tabularnewline
Ridge with CV (10th order poly)&0.028&0.043&&0.027&0.055 \tabularnewline
Random forest (low regularization)&0.013&0.011&&0.008&0.007 \tabularnewline
Random forest (high regularization)&0.018&0.028&&0.012&0.024 \tabularnewline
Gradient boosting (low regularization)&0.028&0.045&&0.025&0.043 \tabularnewline
Gradient boosting (high regularization)&0.020&0.062&&0.019&0.061 \tabularnewline
Neural net&0.019&0.047&&0.016&0.044 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_grad.tex <==
OLS&0.012&0.049&&0.\phantom{000}&0.040&&--0.044&0.028 \tabularnewline
Lasso with CV (2nd order poly)&--0.125&--0.319&&--0.136&--0.202&&0.016&--0.375 \tabularnewline
Ridge with CV (2nd order poly)&0.369&0.534&&0.395&0.453&&0.166&0.564 \tabularnewline
Lasso with CV (10th order poly)&--0.008&0.122&&0.019&0.106&&0.095&0.109 \tabularnewline
Ridge with CV (10th order poly)&0.066&0.027&&0.047&0.001&&--0.017&0.034 \tabularnewline
Random forest (low regularization)&0.048&--0.015&&0.052&--0.016&&0.052&--0.017 \tabularnewline
Random forest (high regularization)&--0.097&0.071&&--0.102&0.077&&--0.096&0.065 \tabularnewline
Gradient boosting (low regularization)&1.114&0.024&&1.167&0.054&&1.345&0.164 \tabularnewline
Gradient boosting (high regularization)&--0.551&0.525&&--0.618&0.506&&--0.715&0.429 \tabularnewline
Neural net&--11.432&0.028&&0.156&0.040&&0.173&0.052 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_grad_large.tex <==
OLS&--0.014&0.009&&--0.017&0.008&&0.002&0.008 \tabularnewline
Lasso with CV (2nd order poly)&0.075&--0.820&&0.086&--0.816&&--0.037&--0.731 \tabularnewline
Ridge with CV (2nd order poly)&--0.157&0.803&&--0.164&0.801&&--0.042&0.706 \tabularnewline
Lasso with CV (10th order poly)&0.284&--0.245&&0.227&--0.230&&0.359&--0.307 \tabularnewline
Ridge with CV (10th order poly)&--0.337&0.320&&--0.279&0.304&&--0.426&0.369 \tabularnewline
Random forest (low regularization)&0.142&--0.012&&0.143&--0.012&&0.167&--0.013 \tabularnewline
Random forest (high regularization)&--0.111&0.073&&--0.109&0.074&&--0.124&0.078 \tabularnewline
Gradient boosting (low regularization)&2.364&1.229&&2.353&1.232&&2.359&1.327 \tabularnewline
Gradient boosting (high regularization)&--1.439&--0.402&&--1.432&--0.405&&--1.428&--0.495 \tabularnewline
Neural net&--14.059&0.031&&0.078&0.034&&0.063&0.041 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_grad_large_nopooled.tex <==
OLS&--0.014&0.009&&0.002&0.008 \tabularnewline
Lasso with CV (2nd order poly)&0.075&--0.820&&--0.037&--0.731 \tabularnewline
Ridge with CV (2nd order poly)&--0.157&0.803&&--0.042&0.706 \tabularnewline
Lasso with CV (10th order poly)&0.284&--0.245&&0.359&--0.307 \tabularnewline
Ridge with CV (10th order poly)&--0.337&0.320&&--0.426&0.369 \tabularnewline
Random forest (low regularization)&0.142&--0.012&&0.167&--0.013 \tabularnewline
Random forest (high regularization)&--0.111&0.073&&--0.124&0.078 \tabularnewline
Gradient boosting (low regularization)&2.364&1.229&&2.359&1.327 \tabularnewline
Gradient boosting (high regularization)&--1.439&--0.402&&--1.428&--0.495 \tabularnewline
Neural net&--14.059&0.031&&0.063&0.041 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_grad_nopooled.tex <==
OLS&0.012&0.049&&--0.044&0.028 \tabularnewline
Lasso with CV (2nd order poly)&--0.125&--0.319&&0.016&--0.375 \tabularnewline
Ridge with CV (2nd order poly)&0.369&0.534&&0.166&0.564 \tabularnewline
Lasso with CV (10th order poly)&--0.008&0.122&&0.095&0.109 \tabularnewline
Ridge with CV (10th order poly)&0.066&0.027&&--0.017&0.034 \tabularnewline
Random forest (low regularization)&0.048&--0.015&&0.052&--0.017 \tabularnewline
Random forest (high regularization)&--0.097&0.071&&--0.096&0.065 \tabularnewline
Gradient boosting (low regularization)&1.114&0.024&&1.345&0.164 \tabularnewline
Gradient boosting (high regularization)&--0.551&0.525&&--0.715&0.429 \tabularnewline
Neural net&--11.432&0.028&&0.173&0.052 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_ols.tex <==
OLS&1.180&0.937&&1.042&0.820&&0.910&0.692 \tabularnewline
Lasso with CV (2nd order poly)&--0.025&0.004&&0.035&0.049&&0.144&0.074 \tabularnewline
Ridge with CV (2nd order poly)&--0.145&--0.186&&--0.093&--0.128&&--0.062&--0.076 \tabularnewline
Lasso with CV (10th order poly)&--0.018&0.107&&--0.017&0.089&&--0.042&0.096 \tabularnewline
Ridge with CV (10th order poly)&--0.025&--0.021&&--0.007&--0.005&&0.023&0.036 \tabularnewline
Random forest (low regularization)&0.002&--0.006&&0.002&--0.007&&0.003&--0.007 \tabularnewline
Random forest (high regularization)&--0.011&0.003&&--0.008&0.007&&--0.016&0.011 \tabularnewline
Gradient boosting (low regularization)&--0.065&--0.132&&--0.052&--0.120&&--0.032&--0.081 \tabularnewline
Gradient boosting (high regularization)&0.101&0.292&&0.097&0.292&&0.079&0.249 \tabularnewline
Neural net&--248.176&0.015&&0.008&0.031&&0.\phantom{000}&0.033 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_ols_large.tex <==
OLS&1.291&0.949&&1.130&0.781&&1.010&0.694 \tabularnewline
Lasso with CV (2nd order poly)&--0.119&--0.504&&--0.052&--0.377&&--0.003&--0.414 \tabularnewline
Ridge with CV (2nd order poly)&--0.154&--0.059&&--0.077&--0.033&&--0.013&0.054 \tabularnewline
Lasso with CV (10th order poly)&0.071&0.409&&0.034&0.359&&0.015&0.351 \tabularnewline
Ridge with CV (10th order poly)&--0.078&--0.121&&--0.034&--0.059&&--0.009&--0.052 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&--0.002&&--0.000&--0.002&&0.\phantom{000}&--0.001 \tabularnewline
Random forest (high regularization)&--0.001&--0.002&&--0.000&--0.001&&--0.001&--0.003 \tabularnewline
Gradient boosting (low regularization)&--0.039&0.161&&--0.027&0.181&&--0.020&0.229 \tabularnewline
Gradient boosting (high regularization)&0.036&0.072&&0.029&0.057&&0.023&0.019 \tabularnewline
Neural net&--11.370&0.112&&--0.001&0.107&&0.\phantom{000}&0.134 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_ols_large_nopooled.tex <==
OLS&1.291&0.949&&1.010&0.694 \tabularnewline
Lasso with CV (2nd order poly)&--0.119&--0.504&&--0.003&--0.414 \tabularnewline
Ridge with CV (2nd order poly)&--0.154&--0.059&&--0.013&0.054 \tabularnewline
Lasso with CV (10th order poly)&0.071&0.409&&0.015&0.351 \tabularnewline
Ridge with CV (10th order poly)&--0.078&--0.121&&--0.009&--0.052 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&--0.002&&0.\phantom{000}&--0.001 \tabularnewline
Random forest (high regularization)&--0.001&--0.002&&--0.001&--0.003 \tabularnewline
Gradient boosting (low regularization)&--0.039&0.161&&--0.020&0.229 \tabularnewline
Gradient boosting (high regularization)&0.036&0.072&&0.023&0.019 \tabularnewline
Neural net&--11.370&0.112&&0.\phantom{000}&0.134 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_ols_nopooled.tex <==
OLS&1.180&0.937&&0.910&0.692 \tabularnewline
Lasso with CV (2nd order poly)&--0.025&0.004&&0.144&0.074 \tabularnewline
Ridge with CV (2nd order poly)&--0.145&--0.186&&--0.062&--0.076 \tabularnewline
Lasso with CV (10th order poly)&--0.018&0.107&&--0.042&0.096 \tabularnewline
Ridge with CV (10th order poly)&--0.025&--0.021&&0.023&0.036 \tabularnewline
Random forest (low regularization)&0.002&--0.006&&0.003&--0.007 \tabularnewline
Random forest (high regularization)&--0.011&0.003&&--0.016&0.011 \tabularnewline
Gradient boosting (low regularization)&--0.065&--0.132&&--0.032&--0.081 \tabularnewline
Gradient boosting (high regularization)&0.101&0.292&&0.079&0.249 \tabularnewline
Neural net&--248.176&0.015&&0.\phantom{000}&0.033 \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_grad.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.097&0.152&&0.072&0.142&&0.051&0.079 \tabularnewline
Ridge with CV (2nd order poly)&0.104&0.116&&0.100&0.095&&0.059&0.080 \tabularnewline
Lasso with CV (10th order poly)&0.089&0.055&&0.052&0.031&&0.044&0.033 \tabularnewline
Ridge with CV (10th order poly)&0.022&0.045&&0.007&0.012&&0.004&0.035 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.002&0.001&&0.001&0.\phantom{000}&&0.001&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.672&0.364&&0.766&0.409&&0.831&0.637 \tabularnewline
Gradient boosting (high regularization)&0.014&0.268&&0.002&0.311&&0.008&0.136 \tabularnewline
Neural net&0.001&0.001&&0.\phantom{000}&0.\phantom{000}&&0.002&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_grad_large.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&1.\phantom{000}&1.\phantom{000}&&1.\phantom{000}&1.\phantom{000}&&1.\phantom{000}&1.\phantom{000} \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_grad_large_nopooled.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&1.\phantom{000}&1.\phantom{000}&&1.\phantom{000}&1.\phantom{000} \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_grad_nopooled.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.097&0.152&&0.051&0.079 \tabularnewline
Ridge with CV (2nd order poly)&0.104&0.116&&0.059&0.080 \tabularnewline
Lasso with CV (10th order poly)&0.089&0.055&&0.044&0.033 \tabularnewline
Ridge with CV (10th order poly)&0.022&0.045&&0.004&0.035 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.002&0.001&&0.001&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.672&0.364&&0.831&0.637 \tabularnewline
Gradient boosting (high regularization)&0.014&0.268&&0.008&0.136 \tabularnewline
Neural net&0.001&0.001&&0.002&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_ols.tex <==
OLS&0.825&0.649&&0.901&0.758&&0.793&0.665 \tabularnewline
Lasso with CV (2nd order poly)&0.155&0.271&&0.097&0.228&&0.174&0.251 \tabularnewline
Ridge with CV (2nd order poly)&0.016&0.019&&0.002&0.003&&0.031&0.032 \tabularnewline
Lasso with CV (10th order poly)&0.002&0.040&&0.\phantom{000}&0.009&&0.001&0.023 \tabularnewline
Ridge with CV (10th order poly)&0.002&0.014&&0.\phantom{000}&0.001&&0.001&0.028 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.\phantom{000}&0.004&&0.\phantom{000}&0.001&&0.\phantom{000}&0.001 \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.004&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_ols_large.tex <==
OLS&0.890&0.294&&0.956&0.278&&0.882&0.167 \tabularnewline
Lasso with CV (2nd order poly)&0.086&0.093&&0.041&0.076&&0.081&0.074 \tabularnewline
Ridge with CV (2nd order poly)&0.025&0.012&&0.003&0.002&&0.037&0.021 \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.193&&0.\phantom{000}&0.149&&0.\phantom{000}&0.148 \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.402&&0.\phantom{000}&0.495&&0.\phantom{000}&0.590 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.\phantom{000}&0.006&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.001&&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_ols_large_nopooled.tex <==
OLS&0.890&0.294&&0.882&0.167 \tabularnewline
Lasso with CV (2nd order poly)&0.086&0.093&&0.081&0.074 \tabularnewline
Ridge with CV (2nd order poly)&0.025&0.012&&0.037&0.021 \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.193&&0.\phantom{000}&0.148 \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.402&&0.\phantom{000}&0.590 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.\phantom{000}&0.006&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.001&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_ols_nopooled.tex <==
OLS&0.825&0.649&&0.793&0.665 \tabularnewline
Lasso with CV (2nd order poly)&0.155&0.271&&0.174&0.251 \tabularnewline
Ridge with CV (2nd order poly)&0.016&0.019&&0.031&0.032 \tabularnewline
Lasso with CV (10th order poly)&0.002&0.040&&0.001&0.023 \tabularnewline
Ridge with CV (10th order poly)&0.002&0.014&&0.001&0.028 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.\phantom{000}&0.004&&0.\phantom{000}&0.001 \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.004&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/timing_long.tex <==
2&200&&24.69&6.34&0.0072&0.0617&0.2567 \tabularnewline
&400&&26.02&6.76&0.0073&0.0640&0.2597 \tabularnewline
&800&&29.51&7.67&0.0074&0.0665&0.2598 \tabularnewline
&1600&&41.23&10.53&0.0082&0.0780&0.2554 \tabularnewline
&9915&&210.78&53.01&0.0170&0.2131&0.2515 \tabularnewline
&99150&&3434.07&778.17&0.1094&1.6571&0.2266 \tabularnewline
5&200&&59.41&13.46&0.0069&0.0588&0.2266 \tabularnewline
&400&&69.18&15.76&0.0070&0.0617&0.2278 \tabularnewline
&800&&88.57&20.77&0.0074&0.0662&0.2345 \tabularnewline
&1600&&137.77&31.92&0.0082&0.0781&0.2317 \tabularnewline
&9915&&848.27&196.97&0.0148&0.1841&0.2322 \tabularnewline
10&200&&120.47&26.01&0.0068&0.0583&0.2159 \tabularnewline
&400&&141.29&30.95&0.0070&0.0608&0.2191 \tabularnewline
&800&&189.87&42.98&0.0075&0.0677&0.2264 \tabularnewline
&1600&&295.87&68.22&0.0082&0.0778&0.2306 \tabularnewline
&9915&&1962.00&453.13&0.0159&0.1998&0.2310 \tabularnewline


==> Simul/sim_ID_AE/dgp_linear.tex <==
0&&0.048&0.048&0.065&0.048&0.009&&1.159&1.154&1.180&&0.993&0.993&0.980 \tabularnewline
.01&&0.174&0.166&0.102&0.166&0.028&&0.685&0.693&0.966&&0.990&0.988&0.980 \tabularnewline
.025&&0.776&0.768&0.422&0.768&0.192&&0.281&0.287&0.447&&0.966&0.964&0.976 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.984&1.\phantom{000}&0.836&&0.135&0.135&0.152&&0.962&0.960&0.960 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&0.992&&0.088&0.088&0.094&&0.956&0.954&0.948 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&0.998&&0.067&0.065&0.066&&0.956&0.952&0.950 \tabularnewline


==> Simul/sim_ID_AE/dgp_linear_pres.tex <==
0&&0.048&0.048&0.009&&1.159&1.154&&0.993&0.993 \tabularnewline
.01&&0.174&0.166&0.028&&0.685&0.693&&0.990&0.988 \tabularnewline
.025&&0.776&0.768&0.192&&0.281&0.287&&0.966&0.964 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.836&&0.135&0.135&&0.962&0.960 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&0.992&&0.088&0.088&&0.956&0.954 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&0.998&&0.067&0.065&&0.956&0.952 \tabularnewline


==> Simul/sim_ID_AE/dgp_linear_vsmall.tex <==
0&&0.048&0.048&&1.159&1.154&&0.993&0.993 \tabularnewline
.01&&0.174&0.166&&0.685&0.693&&0.990&0.988 \tabularnewline
.025&&0.776&0.768&&0.281&0.287&&0.966&0.964 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&&0.135&0.135&&0.962&0.960 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&&0.088&0.088&&0.956&0.954 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&&0.067&0.065&&0.956&0.952 \tabularnewline


==> Simul/sim_ID_AE/dgp_xgb.tex <==
0&&0.038&0.038&0.097&0.038&0.013&&1.076&1.089&0.945&&0.990&0.993&0.980 \tabularnewline
.01&&0.213&0.215&0.086&0.215&0.042&&0.692&0.667&1.023&&0.980&0.983&0.995 \tabularnewline
.025&&0.805&0.795&0.449&0.795&0.263&&0.282&0.279&0.462&&0.961&0.963&0.971 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.980&1.\phantom{000}&0.890&&0.130&0.136&0.155&&0.958&0.961&0.963 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&0.995&&0.083&0.085&0.098&&0.946&0.946&0.956 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&&0.065&0.066&0.074&&0.956&0.951&0.949 \tabularnewline


==> Simul/sim_ID_AE/dgp_xgb_pres.tex <==
0&&0.038&0.038&0.013&&1.076&1.089&&0.990&0.993 \tabularnewline
.01&&0.213&0.215&0.042&&0.692&0.667&&0.980&0.983 \tabularnewline
.025&&0.805&0.795&0.263&&0.282&0.279&&0.961&0.963 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&0.890&&0.130&0.136&&0.958&0.961 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&0.995&&0.083&0.085&&0.946&0.946 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&1.\phantom{000}&&0.065&0.066&&0.956&0.951 \tabularnewline


==> Simul/sim_ID_AE/dgp_xgb_vsmall.tex <==
0&&0.038&0.038&&1.076&1.089&&0.990&0.993 \tabularnewline
.01&&0.213&0.215&&0.692&0.667&&0.980&0.983 \tabularnewline
.025&&0.805&0.795&&0.282&0.279&&0.961&0.963 \tabularnewline
.05&&1.\phantom{000}&1.\phantom{000}&&0.130&0.136&&0.958&0.961 \tabularnewline
.075&&1.\phantom{000}&1.\phantom{000}&&0.083&0.085&&0.946&0.946 \tabularnewline
.1&&1.\phantom{000}&1.\phantom{000}&&0.065&0.066&&0.956&0.951 \tabularnewline


==> Simul/sim_OOB2/bias_100.tex <==
&0.207&0.213&0.417&&0.205&0.208&0.463 \tabularnewline
&0.209&0.211&0.631&&0.216&0.213&0.613 \tabularnewline
&0.233&0.233&0.559&&0.237&0.230&0.562 \tabularnewline
&0.184&0.191&0.672&&0.220&0.220&0.598 \tabularnewline
&0.249&0.251&0.506&&0.279&0.276&0.445 \tabularnewline
&0.189&0.206&0.672&&0.583&0.244&0.531 \tabularnewline
&0.050&0.133&0.790&&235.475&0.409&0.387 \tabularnewline
&0.227&0.231&0.600&&0.209&0.211&0.650 \tabularnewline
&0.228&0.232&0.596&&0.189&0.191&0.613 \tabularnewline
&0.251&0.254&0.541&&0.235&0.234&0.497 \tabularnewline
&--0.006&0.113&0.896&&--0.136&0.202&0.651 \tabularnewline
&0.038&0.115&0.897&&--0.130&0.200&0.633 \tabularnewline
&0.115&0.140&0.830&&0.041&0.127&0.835 \tabularnewline
&0.054&0.103&0.873&&--0.211&0.377&0.373 \tabularnewline
&0.156&0.164&0.763&&350.537&0.455&0.373 \tabularnewline
&0.142&0.156&0.785&&.&.&. \tabularnewline


==> Simul/sim_OOB2/bias_1000.tex <==
&0.212&0.214&0.003&&0.212&0.213&0.005 \tabularnewline
&0.213&0.214&0.006&&0.213&0.213&0.005 \tabularnewline
&0.223&0.223&0.002&&0.211&0.212&0.009 \tabularnewline
&0.197&0.196&0.016&&0.195&0.193&0.020 \tabularnewline
&0.225&0.225&0.002&&0.225&0.224&0.003 \tabularnewline
&0.242&0.242&0.005&&0.185&0.184&0.044 \tabularnewline
&0.071&0.070&0.675&&0.262&0.271&0.154 \tabularnewline
&0.114&0.113&0.418&&0.086&0.085&0.531 \tabularnewline
&0.143&0.143&0.213&&0.125&0.124&0.260 \tabularnewline
&0.234&0.234&0.001&&0.232&0.231&0.001 \tabularnewline
&--0.011&0.040&0.926&&--0.074&0.083&0.638 \tabularnewline
&0.015&0.037&0.948&&--0.003&0.043&0.893 \tabularnewline
&0.056&0.059&0.822&&0.045&0.050&0.852 \tabularnewline
&--0.025&0.038&0.889&&--0.213&0.221&0.050 \tabularnewline
&0.040&0.046&0.882&&--0.126&0.135&0.243 \tabularnewline
&0.037&0.044&0.890&&.&.&. \tabularnewline


==> Simul/sim_SJ/bias_1.tex <==
&Oracle&0.113&0.915&0.036&0.944&&0.090&0.915&0.032&0.934&&0.117&0.890&0.036&0.944 \tabularnewline
&OLS (Base)&0.130&0.886&0.037&0.942&&0.286&0.375&0.288&0.\phantom{000}&&0.224&0.617&0.209&0.007 \tabularnewline
&PDS-Lasso (Base)&0.133&0.840&0.037&0.941&&0.295&0.276&0.287&0.\phantom{000}&&0.227&0.588&0.209&0.006 \tabularnewline
&PDS-Lasso (Poly 5)&0.148&0.768&0.038&0.935&&0.219&0.465&0.106&0.327&&0.228&0.583&0.198&0.016 \tabularnewline
&PDS-Lasso (Poly 2 + Inter.)&0.158&0.742&0.039&0.931&&0.200&0.549&0.033&0.922&&0.231&0.591&0.176&0.058 \tabularnewline
&OLS&0.134&0.710&0.038&0.930&&0.286&0.226&0.288&0.\phantom{000}&&0.226&0.424&0.209&0.006 \tabularnewline
&Lasso with CV (Base)&0.116&0.893&0.037&0.950&&0.286&0.312&0.288&0.\phantom{000}&&0.221&0.617&0.210&0.008 \tabularnewline
&Ridge with CV (Base)&0.123&0.888&0.038&0.941&&0.291&0.288&0.289&0.\phantom{000}&&0.246&0.542&0.219&0.002 \tabularnewline
&Lasso with CV (Poly 5)&0.127&0.843&0.039&0.940&&0.144&0.762&0.092&0.458&&0.202&0.635&0.193&0.025 \tabularnewline
&Ridge with CV (Poly 5)&0.139&0.794&0.050&0.864&&0.178&0.620&0.125&0.188&&0.265&0.478&0.221&0.002 \tabularnewline
&Lasso with CV (Poly 2 + Inter.)&0.137&0.816&0.042&0.925&&0.155&0.718&0.036&0.925&&0.214&0.623&0.184&0.048 \tabularnewline
&Ridge with CV (Poly 2 + Inter.)&0.158&0.695&0.095&0.505&&0.152&0.685&0.112&0.308&&0.191&0.645&0.265&0.\phantom{000} \tabularnewline
&Random forest (Low)&0.179&0.728&0.098&0.566&&0.249&0.438&0.196&0.015&&0.229&0.619&0.110&0.447 \tabularnewline
&Random forest (Medium)&0.186&0.718&0.128&0.317&&0.252&0.431&0.222&0.005&&0.232&0.612&0.140&0.227 \tabularnewline
&Random forest (High)&0.237&0.565&0.227&0.007&&0.270&0.362&0.269&0.\phantom{000}&&0.259&0.520&0.230&0.002 \tabularnewline
&Gradient boosting (Low)&0.103&0.906&0.039&0.924&&0.126&0.802&0.080&0.578&&0.118&0.885&0.038&0.938 \tabularnewline
&Gradient boosting (Medium)&0.126&0.860&0.048&0.881&&0.197&0.598&0.144&0.125&&0.137&0.838&0.045&0.906 \tabularnewline
&Gradient boosting (High)&0.239&0.544&0.154&0.142&&0.277&0.338&0.258&0.\phantom{000}&&0.205&0.665&0.079&0.715 \tabularnewline
&Neural net&0.137&0.773&0.152&0.131&&0.106&0.843&0.075&0.534&&0.107&0.882&0.037&0.865 \tabularnewline
&Stacking: CLS&0.117&0.898&0.037&0.949&&0.169&0.683&0.037&0.918&&0.169&0.742&0.048&0.892 \tabularnewline
&Stacking: Single best&0.119&0.907&0.037&0.949&&0.149&0.744&0.036&0.925&&0.157&0.781&0.045&0.902 \tabularnewline
&Short-stacking: CLS&0.116&0.892&0.037&0.948&&0.170&0.671&0.037&0.920&&0.165&0.754&0.046&0.897 \tabularnewline
&Short-stacking: Single best&0.117&0.899&0.037&0.950&&0.141&0.756&0.036&0.925&&0.157&0.784&0.045&0.908 \tabularnewline
&Pooled stacking: CLS&0.117&0.895&0.038&0.949&&0.188&0.625&0.037&0.922&&0.181&0.731&0.047&0.896 \tabularnewline
&Pooled stacking: Single best&0.117&0.894&0.037&0.950&&0.173&0.656&0.036&0.925&&0.181&0.725&0.045&0.906 \tabularnewline


==> Simul/sim_SJ/bias_2.tex <==
&Oracle&0.100&0.928&0.032&0.944&&0.100&0.912&0.031&0.956 \tabularnewline
&OLS (Base)&0.127&0.855&0.078&0.613&&0.113&0.858&0.077&0.615 \tabularnewline
&PDS-Lasso (Base)&0.119&0.833&0.078&0.611&&0.115&0.852&0.077&0.611 \tabularnewline
&PDS-Lasso (Poly 5)&0.128&0.808&0.050&0.843&&0.113&0.839&0.041&0.884 \tabularnewline
&PDS-Lasso (Poly 2 + Inter.)&0.132&0.802&0.050&0.828&&0.113&0.859&0.036&0.918 \tabularnewline
&OLS&0.133&0.678&0.078&0.582&&0.117&0.839&0.077&0.608 \tabularnewline
&Lasso with CV (Base)&0.121&0.851&0.081&0.605&&0.115&0.853&0.077&0.614 \tabularnewline
&Ridge with CV (Base)&0.161&0.712&0.078&0.583&&0.115&0.850&0.077&0.608 \tabularnewline
&Lasso with CV (Poly 5)&0.121&0.852&0.040&0.916&&0.125&0.853&0.035&0.928 \tabularnewline
&Ridge with CV (Poly 5)&0.171&0.687&0.104&0.376&&0.141&0.795&0.047&0.898 \tabularnewline
&Lasso with CV (Poly 2 + Inter.)&0.130&0.818&0.043&0.900&&0.110&0.877&0.036&0.926 \tabularnewline
&Ridge with CV (Poly 2 + Inter.)&0.143&0.736&0.148&0.107&&0.133&0.818&0.035&0.914 \tabularnewline
&Random forest (Low)&0.201&0.618&0.117&0.294&&0.121&0.842&0.046&0.845 \tabularnewline
&Random forest (Medium)&0.203&0.609&0.141&0.151&&0.125&0.838&0.066&0.701 \tabularnewline
&Random forest (High)&0.244&0.477&0.226&0.001&&0.174&0.727&0.171&0.038 \tabularnewline
&Gradient boosting (Low)&0.098&0.905&0.033&0.941&&0.101&0.899&0.033&0.936 \tabularnewline
&Gradient boosting (Medium)&0.121&0.842&0.049&0.844&&0.105&0.888&0.041&0.896 \tabularnewline
&Gradient boosting (High)&0.218&0.552&0.127&0.234&&0.171&0.718&0.114&0.311 \tabularnewline
&Neural net&0.094&0.893&0.127&0.186&&0.108&0.875&0.034&0.927 \tabularnewline
&Stacking: CLS&0.114&0.864&0.040&0.915&&0.106&0.879&0.035&0.935 \tabularnewline
&Stacking: Single best&0.114&0.875&0.038&0.925&&0.107&0.888&0.034&0.940 \tabularnewline
&Short-stacking: CLS&0.114&0.869&0.040&0.914&&0.105&0.887&0.033&0.945 \tabularnewline
&Short-stacking: Single best&0.114&0.869&0.039&0.923&&0.103&0.898&0.034&0.938 \tabularnewline
&Pooled stacking: CLS&0.117&0.856&0.040&0.912&&0.106&0.882&0.034&0.944 \tabularnewline
&Pooled stacking: Single best&0.119&0.854&0.039&0.922&&0.102&0.884&0.035&0.942 \tabularnewline


==> Simul/sim_SJ/psw_D.tex <==
&OLS&.0158872&.0837686&.0111304&9.40e-16&.0273159&.0009659&.0327529&.0154967&.242624&.0074395 \tabularnewline
&Lasso with CV (Base)&.1664726&.7682732&.0097534&1.04e-15&.2467202&1.75e-15&.5371254&.0065727&.147541&.0062742 \tabularnewline
&Ridge with CV (Base)&.5066003&.0103315&.0007243&8.98e-16&.0168052&1.85e-15&.0327482&.0090213&.0080128&.0159039 \tabularnewline
&Lasso with CV (Poly 5)&.0352897&.0338133&.1859743&.0347182&.0288578&1.79e-15&.1109617&.5849553&.0656686&.286189 \tabularnewline
&Ridge with CV (Poly 5)&.0349362&.0458112&.105194&.0026362&.0085788&3.15e-15&.0189261&.0000545&.0758593&.0239043 \tabularnewline
&Lasso with CV (Poly 2 + Inter.)&.0276898&.0102469&.2711155&.9621329&.0563394&.0044802&.0630886&.320792&.0918754&.4004852 \tabularnewline
&Ridge with CV (Poly 2 + Inter.)&.0823986&.0081447&.0381471&.0000886&.0243044&2.24e-15&.0408341&.0000418&.0523524&.0784924 \tabularnewline
&Random forest (Low regularization)&.0574114&.0037441&.1845031&6.26e-16&.1223523&.0329975&.0541481&.0000146&.114848&.0625394 \tabularnewline
&Random forest (Medium regularization)&.0104037&7.74e-06&.0811526&6.32e-16&.1112274&6.61e-16&.0179799&3.72e-16&.031622&.000825 \tabularnewline
&Random forest (High regularization)&.000577&2.00e-16&.0360659&7.25e-16&.0350932&1.26e-15&.0016861&4.93e-16&.0233057&.0000113 \tabularnewline
&Gradient boosting (Low regularization)&.032979&.013916&.0286989&.0000814&.2071891&.1334506&.0675183&.0405494&.0260771&.0195481 \tabularnewline
&Gradient boosting (Medium regularization)&.0029345&.0042783&.0109189&1.00e-15&.0916581&.8182238&.0060314&.0085373&.0012673&.002882 \tabularnewline
&Gradient boosting (High regularization)&.0006229&3.59e-16&.0183193&9.53e-16&.0067779&.0054401&.0003587&4.77e-16&.0013514&2.00e-16 \tabularnewline
&Neural net&.0257972&.0176643&.0183023&.0003428&.0167803&.0044419&.0158405&.0139645&.1175949&.0955056 \tabularnewline


==> Simul/sim_SJ/psw_Y.tex <==
&OLS&.0135509&.0815498&.0111926&1.32e-15&.027541&.0008331&.0304471&.01662&.2346664&.0077989 \tabularnewline
&Lasso with CV (Base)&.1820874&.7725515&.0135412&1.30e-15&.2798621&1.75e-15&.5454502&.0086116&.1480531&.0058864 \tabularnewline
&Ridge with CV (Base)&.5051364&.0110841&.0015269&1.31e-15&.0179855&1.74e-15&.0357833&.0102446&.0082218&.0146988 \tabularnewline
&Lasso with CV (Poly 5)&.0352734&.0344347&.1727345&.0353685&.0300388&.0000487&.111107&.5636162&.0579837&.2857173 \tabularnewline
&Ridge with CV (Poly 5)&.0377672&.0427639&.1076168&.0042565&.0082947&3.21e-15&.016323&.0002908&.0856919&.0253541 \tabularnewline
&Lasso with CV (Poly 2 + Inter.)&.0246921&.0104916&.2481337&.9598258&.0586604&.0056311&.0606584&.3355087&.0811703&.407582 \tabularnewline
&Ridge with CV (Poly 2 + Inter.)&.0851105&.0080526&.0405827&.0000642&.0247005&2.15e-15&.0411468&.0000319&.0514828&.0714551 \tabularnewline
&Random forest (Low regularization)&.0468791&.0031821&.2179099&8.32e-16&.1217394&.0545122&.0525093&.0000964&.125343&.05968 \tabularnewline
&Random forest (Medium regularization)&.007523&2.71e-16&.079182&7.73e-16&.1079177&7.94e-16&.0155232&5.08e-16&.0368583&.0005705 \tabularnewline
&Random forest (High regularization)&.0003606&2.65e-16&.0317144&1.00e-15&.0260662&1.32e-15&.0008844&6.07e-16&.0157284&.0000782 \tabularnewline
&Gradient boosting (Low regularization)&.0328898&.0125405&.0281342&.0001482&.1976724&.1169323&.0654207&.0379119&.0216249&.019914 \tabularnewline
&Gradient boosting (Medium regularization)&.001878&.0054407&.0099963&1.36e-15&.0745628&.7836894&.0063052&.0107003&.0027525&.0027213 \tabularnewline
&Gradient boosting (High regularization)&.0010361&4.59e-16&.020214&1.37e-15&.0066646&.0324654&.0008543&5.46e-16&.0014807&2.19e-16 \tabularnewline
&Neural net&.0258154&.0179084&.0175206&.0003369&.0182939&.0058878&.0175873&.0163677&.1289423&.0985434 \tabularnewline


==> Simul/sim_SJ/ssw_D.tex <==
&OLS&.0364592&.097405&.0175067&3.19e-16&.0416793&.0005204&.0545231&.0083069&.1410212&.0029081 \tabularnewline
&Lasso with CV (Base)&.1874215&.6645907&.0117895&3.58e-16&.1623308&4.19e-16&.3961703&.0026154&.1328388&.0059486 \tabularnewline
&Ridge with CV (Base)&.3517502&.0441657&.0024854&3.52e-16&.0145191&4.60e-16&.0216873&.0080542&.0506908&.0100504 \tabularnewline
&Lasso with CV (Poly 5)&.0620936&.0612446&.2371242&.0269362&.0521112&.0000397&.1688424&.5570484&.1203138&.255223 \tabularnewline
&Ridge with CV (Poly 5)&.0502006&.0408376&.0968765&.0019557&.0109667&5.99e-16&.0262994&.0001854&.0714759&.0822194 \tabularnewline
&Lasso with CV (Poly 2 + Inter.)&.0551464&.0218104&.2873931&.9677024&.0831751&.0033348&.1048952&.3404824&.1279158&.3605145 \tabularnewline
&Ridge with CV (Poly 2 + Inter.)&.0809677&.0116083&.0602013&.0004108&.0274317&4.88e-16&.045553&.0004127&.0397265&.0948115 \tabularnewline
&Random forest (Low regularization)&.0267514&.0043339&.07861&2.39e-16&.0815851&.0282759&.0240491&.0002363&.0652839&.0490498 \tabularnewline
&Random forest (Medium regularization)&.0141708&.000187&.0650984&2.36e-16&.0840545&2.07e-16&.0147686&1.48e-16&.0265952&.0024512 \tabularnewline
&Random forest (High regularization)&.0005404&1.09e-16&.0128769&2.80e-16&.014694&3.40e-16&.0007037&1.89e-16&.0104117&.0002869 \tabularnewline
&Gradient boosting (Low regularization)&.052651&.0220443&.055045&.0006493&.2003697&.1565859&.0754345&.0456565&.0557553&.0322048 \tabularnewline
&Gradient boosting (Medium regularization)&.0244373&.0101817&.0273641&2.90e-16&.1700748&.7852128&.0326016&.0184585&.026573&.0123737 \tabularnewline
&Gradient boosting (High regularization)&.0022492&1.50e-16&.0126575&3.45e-16&.0233384&.0192613&.0008913&2.06e-16&.0032113&.0001056 \tabularnewline
&Neural net&.0551609&.0215908&.0349713&.0023455&.0336696&.0067691&.0335805&.0185433&.1281869&.0918526 \tabularnewline


==> Simul/sim_SJ/ssw_Y.tex <==
&OLS&.0323108&.095877&.018134&3.99e-16&.0416098&.0003775&.0515796&.0095417&.1322253&.0032791 \tabularnewline
&Lasso with CV (Base)&.2003479&.6558712&.0169013&4.20e-16&.1855361&5.45e-16&.407111&.0038991&.1343242&.0085246 \tabularnewline
&Ridge with CV (Base)&.3499946&.053688&.0013892&4.61e-16&.0153954&.0000133&.0257363&.0101725&.0518767&.0101594 \tabularnewline
&Lasso with CV (Poly 5)&.0647247&.0591255&.2341462&.0284356&.0597988&.0000213&.1668543&.5427072&.1183251&.2576331 \tabularnewline
&Ridge with CV (Poly 5)&.0555318&.0378597&.1016609&.0022702&.0086117&7.66e-16&.024691&.0003086&.076725&.0784735 \tabularnewline
&Lasso with CV (Poly 2 + Inter.)&.0478489&.0230998&.2578032&.9637466&.0794822&.0030961&.0994492&.3467089&.109911&.3649835 \tabularnewline
&Ridge with CV (Poly 2 + Inter.)&.0853002&.0122545&.0622161&.0008429&.0281077&2.04e-06&.0427504&.0006971&.034254&.0837306 \tabularnewline
&Random forest (Low regularization)&.0219459&.0037805&.0915363&3.07e-16&.0861837&.0398639&.022256&.0002564&.0629977&.0479298 \tabularnewline
&Random forest (Medium regularization)&.009744&.0002258&.0563391&3.11e-16&.0715795&2.71e-16&.0157703&1.68e-16&.0349089&.0016989 \tabularnewline
&Random forest (High regularization)&.0007569&1.28e-16&.014749&3.53e-16&.0092187&4.16e-16&.0001836&2.16e-16&.0075228&.0002704 \tabularnewline
&Gradient boosting (Low regularization)&.047661&.0241999&.0599078&.001565&.1881991&.1536709&.075325&.0458865&.0548517&.0309133 \tabularnewline
&Gradient boosting (Medium regularization)&.0226551&.0107316&.0333577&.0000733&.1681196&.7421989&.031835&.0187496&.0216058&.0108225 \tabularnewline
&Gradient boosting (High regularization)&.0026419&.0000268&.0156607&4.33e-16&.0223155&.0524128&.0011025&2.42e-16&.0037286&.0000799 \tabularnewline
&Neural net&.0585363&.0232595&.0361986&.0030664&.0358421&.0083431&.0353559&.0210724&.156743&.1015013 \tabularnewline


==> Simul/sim_WZ/bias_ddml_candidate_f10.tex <==
&OLS&963&-150.8&210&-161.7&-235.5&31.8 \tabularnewline
&Lasso with CV (TWI)&5948.6&3223.1&2589.1&1706.2&872.2&734.1 \tabularnewline
&Ridge with CV (TWI)&4137.3&1853.8&1617.5&951.8&657.5&879.2 \tabularnewline
&Lasso with CV (QSI)&297.5&-343.9&-311.9&-551.8&-597.1&-239.8 \tabularnewline
&Ridge with CV (QSI)&426.1&-111&85.3&-240.8&-294.4&-7.8 \tabularnewline
&Random forest (low regularization)&1852.8&618.3&709.6&259.7&7.7&95.5 \tabularnewline
&Random forest (high regularization)&9987.4&4270.1&2940.2&1919.5&1037.8&925 \tabularnewline
&Gradient boosting (low regularization)&772.3&-25&306.3&70.7&-127.2&113 \tabularnewline
&Gradient boosting (high regularization)&1060.8&94.3&564.6&292.5&44.2&228.6 \tabularnewline
&Neural net&8892.3&7481.2&6915.4&5653.2&3716.5&2224.2 \tabularnewline


==> Simul/sim_WZ/bias_ddml_candidate_f2.tex <==
&OLS&-509.4&440.4&-643.7&-270.5&243.3&192 \tabularnewline
&Lasso with CV (TWI)&7184.1&5485.8&3408.9&2998&2509.6&1848 \tabularnewline
&Ridge with CV (TWI)&4659.4&3674.3&1888.4&1649.9&1433.4&1189.6 \tabularnewline
&Lasso with CV (QSI)&911.3&191.9&-874.5&-628.5&-207.1&-286.3 \tabularnewline
&Ridge with CV (QSI)&213.3&269.4&-533.9&-304.8&154&49.3 \tabularnewline
&Random forest (low regularization)&1689.7&1136.3&-88.2&311.6&652&455.5 \tabularnewline
&Random forest (high regularization)&14334.3&8404.1&4923.6&3493.2&2704.6&1982.3 \tabularnewline
&Gradient boosting (low regularization)&-391.8&32.1&-668.6&-185&373.4&314.6 \tabularnewline
&Gradient boosting (high regularization)&-95.5&301.8&-370.1&85.5&615.4&519.8 \tabularnewline
&Neural net&9433.7&9725&7407.1&7627.3&6552.1&5595.1 \tabularnewline


==> Simul/sim_WZ/bias_ddml_meta_f10.tex <==
&Short-stacking: CLS&1355.1&342.2&403.3&34.2&-103.9&43.8 \tabularnewline
&Short-stacking: Single-best&669.2&113.5&144.6&-182.3&-272.6&48.9 \tabularnewline
&Pooled stacking: CLS&2849.3&1345.7&1197&383.8&-102.3&-10.6 \tabularnewline
&Pooled stacking: Single-best&724.1&-69.4&45&-250.7&-309&-19.4 \tabularnewline
&Stacking: CLS&1394.1&296.9&344.5&2.8&-168.5&56.9 \tabularnewline
&Stacking: Single-best&718.4&-47&104.3&-141.5&-318.6&42.5 \tabularnewline


==> Simul/sim_WZ/bias_ddml_meta_f2.tex <==
&Short-stacking: CLS&1842.3&1078.3&-144.4&61.2&446.7&282.9 \tabularnewline
&Short-stacking: Single-best&1303.5&582.3&-436.4&-248.8&194&111.1 \tabularnewline
&Pooled stacking: CLS&2799&1471.3&159.5&209.8&572.7&508.8 \tabularnewline
&Pooled stacking: Single-best&1791.9&622.9&-542.3&-296.3&144.7&84.8 \tabularnewline
&Stacking: CLS&1924.6&1196.1&-191.2&59.4&390.3&310.9 \tabularnewline
&Stacking: Single-best&1173.4&549.6&-604.2&-285&181.8&138.3 \tabularnewline


==> Simul/sim_WZ/bias_olspds_f10.tex <==
&OLS QSI&-2083.5&-910.2&-806.4&-809.9&-677.2&-626.5 \tabularnewline
&OLS TWI&-1694.5&-475.4&13.2&-366&-320.3&-91.3 \tabularnewline
&Post double Lasso QSI c=0.5&409.2&-308.9&-204&-503.1&-571.6&-354.1 \tabularnewline
&Post double Lasso QSI c=1&-179.1&-1113.5&-639.4&-1063.2&-1000.5&-523.5 \tabularnewline
&Post double Lasso QSI c=1.5&8021.3&739.9&-1526.2&-2434.4&-2255.4&-1863.5 \tabularnewline
&Post double Lasso TWI c=0.5&3611.2&2484.4&2347.2&1748.3&1270.4&1197.5 \tabularnewline
&Post double Lasso TWI c=1&6303.3&3501.1&3453.1&2523.9&1702.4&1871.8 \tabularnewline
&Post double Lasso TWI c=1.5&14386.1&8981.9&6317.9&4802.2&3939&3094.5 \tabularnewline


==> Simul/sim_WZ/bias_olspds_f2.tex <==
&OLS QSI&-2532.3&-1311.4&-1421.9&-961.6&-399&-282.2 \tabularnewline
&OLS TWI&-2100.3&-448&-936.5&-531.8&23.1&244.7 \tabularnewline
&Post double Lasso QSI c=0.5&-154.7&-120.1&-1019.8&-628.9&-50.5&-161.7 \tabularnewline
&Post double Lasso QSI c=1&-600.6&-1053&-1576.5&-1079&-485.1&-424.9 \tabularnewline
&Post double Lasso QSI c=1.5&7836.3&1064&-2253.4&-2434.8&-1644.7&-1698.3 \tabularnewline
&Post double Lasso TWI c=0.5&2868.8&2792.2&1635.4&1595.6&1767.6&1460.7 \tabularnewline
&Post double Lasso TWI c=1&5201.7&3964.3&2742&2328.1&2174.8&1975.8 \tabularnewline
&Post double Lasso TWI c=1.5&13619.4&9399.4&5610&4277&4150.8&3065.3 \tabularnewline


==> Simul/sim_WZ/fullsample_ddml.tex <==
&Neural net&6433.092 \tabularnewline
&OLS&6463.73 \tabularnewline
&Lasso with CV (TWI)&6780.161 \tabularnewline
&Ridge with CV (TWI)&6760.134 \tabularnewline
&Lasso with CV (QSI)&5722.624 \tabularnewline
&Ridge with CV (QSI)&5995.346 \tabularnewline
&Random forest (low regularization)&6089.389 \tabularnewline
&Random forest (high regularization)&6552.221 \tabularnewline
&Gradient boosting (low regularization)&7003.373 \tabularnewline
&Gradient boosting (high regularization)&7992.538 \tabularnewline


==> Simul/sim_WZ/fullsample_meta.tex <==
&Pooled stacking: CLS&5822.695 \tabularnewline
&Pooled stacking: Single-best&5717.825 \tabularnewline
&Short-stacking: CLS&5803.858 \tabularnewline
&Short-stacking: Single-best&5697.312 \tabularnewline
&Stacking: CLS&5767.291 \tabularnewline
&Stacking: Single-best&5661.027 \tabularnewline


==> Simul/sim_WZ/fullsample_olspds.tex <==
&OLS TWI&6751.907 \tabularnewline
&OLS QSI&5988.413 \tabularnewline
&Post double Lasso TWI c=0.5&6562.923 \tabularnewline
&Post double Lasso QSI c=0.5&5648.14 \tabularnewline
&Post double Lasso TWI c=1&6630.751 \tabularnewline
&Post double Lasso QSI c=1&4646.575 \tabularnewline
&Post double Lasso TWI c=1.5&7474.508 \tabularnewline
&Post double Lasso QSI c=1.5&4472.324 \tabularnewline


==> Simul/sim_WZ/psw_d_nnls1_folds10.tex <==
&OLS&.129&.207&.257&.279&.252&.221&.007 \tabularnewline
&Neural net&.013&.013&.012&.012&.01&.013&.043 \tabularnewline
&Lasso with CV (TWI)&.028&.017&.014&.01&.008&.007&.104 \tabularnewline
&Ridge with CV (TWI)&.037&.011&.005&.008&.008&.008&.001 \tabularnewline
&Lasso with CV (QSI)&.129&.205&.261&.281&.304&.296&.452 \tabularnewline
&Ridge with CV (QSI)&.239&.169&.085&.046&.049&.058&.011 \tabularnewline
&Random forest (low regularization)&.106&.117&.133&.168&.221&.271&.007 \tabularnewline
&Random forest (high regularization)&.257&.189&.155&.133&.087&.066&.131 \tabularnewline
&Gradient boosting (low regularization)&.021&.025&.032&.028&.029&.036&.241 \tabularnewline
&Gradient boosting (high regularization)&.041&.047&.048&.035&.033&.024&.003 \tabularnewline


==> Simul/sim_WZ/psw_d_nnls1_folds2.tex <==
&OLS&.078&.142&.189&.226&.261&.279&.143 \tabularnewline
&Neural net&.041&.031&.036&.033&.03&.028&.043 \tabularnewline
&Lasso with CV (TWI)&.059&.029&.016&.017&.012&.009&.028 \tabularnewline
&Ridge with CV (TWI)&.075&.033&.016&.011&.008&.006&.002 \tabularnewline
&Lasso with CV (QSI)&.128&.147&.202&.231&.27&.273&.424 \tabularnewline
&Ridge with CV (QSI)&.176&.227&.178&.132&.061&.044&.005 \tabularnewline
&Random forest (low regularization)&.111&.093&.1&.108&.14&.174&.01 \tabularnewline
&Random forest (high regularization)&.258&.22&.178&.158&.14&.117&.173 \tabularnewline
&Gradient boosting (low regularization)&.026&.028&.032&.033&.033&.035&.169 \tabularnewline
&Gradient boosting (high regularization)&.05&.051&.052&.051&.044&.035&.003 \tabularnewline


==> Simul/sim_WZ/psw_d_singlebest_folds10.tex <==
&OLS&.015&.076&.135&.184&.174&.128&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.023&.009&.007&.002&0&0&0 \tabularnewline
&Ridge with CV (TWI)&.087&.008&.002&.006&.001&.001&0 \tabularnewline
&Lasso with CV (QSI)&.19&.313&.355&.335&.32&.212&.95 \tabularnewline
&Ridge with CV (QSI)&.299&.175&.034&.011&.025&.026&0 \tabularnewline
&Random forest (low regularization)&.084&.018&.005&.002&0&0&0 \tabularnewline
&Random forest (high regularization)&.256&.309&.344&.376&.396&.555&0 \tabularnewline
&Gradient boosting (low regularization)&.001&.002&.006&.011&.038&.065&.05 \tabularnewline
&Gradient boosting (high regularization)&.044&.09&.112&.073&.044&.012&0 \tabularnewline


==> Simul/sim_WZ/psw_d_singlebest_folds2.tex <==
&OLS&.001&.019&.056&.084&.152&.188&.237 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.055&.02&.009&.008&.004&.002&0 \tabularnewline
&Ridge with CV (TWI)&.213&.074&.012&.005&.002&.002&0 \tabularnewline
&Lasso with CV (QSI)&.174&.222&.322&.362&.358&.299&.586 \tabularnewline
&Ridge with CV (QSI)&.158&.3&.197&.094&.011&.009&0 \tabularnewline
&Random forest (low regularization)&.169&.051&.021&.005&.001&0&0 \tabularnewline
&Random forest (high regularization)&.192&.246&.284&.323&.35&.39&.011 \tabularnewline
&Gradient boosting (low regularization)&.001&.002&.001&.002&.01&.026&.166 \tabularnewline
&Gradient boosting (high regularization)&.037&.065&.098&.115&.111&.082&0 \tabularnewline


==> Simul/sim_WZ/psw_y_nnls1_folds10.tex <==
&OLS&.151&.147&.12&.093&.048&.026&0 \tabularnewline
&Neural net&.232&.238&.248&.191&.117&.039&.07 \tabularnewline
&Lasso with CV (TWI)&.023&.017&.02&.021&.021&.025&.072 \tabularnewline
&Ridge with CV (TWI)&.033&.034&.035&.025&.016&.013&.061 \tabularnewline
&Lasso with CV (QSI)&.179&.204&.193&.209&.229&.259&.607 \tabularnewline
&Ridge with CV (QSI)&.167&.21&.242&.308&.38&.416&.175 \tabularnewline
&Random forest (low regularization)&.095&.076&.087&.103&.142&.181&.008 \tabularnewline
&Random forest (high regularization)&.085&.039&.019&.017&.023&.022&.003 \tabularnewline
&Gradient boosting (low regularization)&.02&.022&.027&.025&.023&.017&.002 \tabularnewline
&Gradient boosting (high regularization)&.017&.012&.01&.007&.001&.001&.003 \tabularnewline


==> Simul/sim_WZ/psw_y_nnls1_folds2.tex <==
&OLS&.124&.168&.177&.16&.122&.086&0 \tabularnewline
&Neural net&.123&.084&.097&.087&.095&.123&.034 \tabularnewline
&Lasso with CV (TWI)&.038&.033&.026&.025&.021&.022&.133 \tabularnewline
&Ridge with CV (TWI)&.049&.037&.04&.035&.028&.019&.003 \tabularnewline
&Lasso with CV (QSI)&.184&.234&.263&.271&.263&.25&.501 \tabularnewline
&Ridge with CV (QSI)&.189&.217&.212&.259&.305&.334&.304 \tabularnewline
&Random forest (low regularization)&.165&.095&.087&.085&.101&.112&.022 \tabularnewline
&Random forest (high regularization)&.072&.081&.05&.033&.021&.017&.003 \tabularnewline
&Gradient boosting (low regularization)&.028&.029&.032&.032&.035&.03&.001 \tabularnewline
&Gradient boosting (high regularization)&.029&.021&.017&.014&.009&.006&0 \tabularnewline


==> Simul/sim_WZ/psw_y_singlebest_folds10.tex <==
&OLS&.114&.141&.095&.039&.006&.001&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.01&.006&.004&.004&.004&.011&0 \tabularnewline
&Ridge with CV (TWI)&.053&.062&.081&.072&.042&.019&0 \tabularnewline
&Lasso with CV (QSI)&.293&.375&.355&.347&.331&.344&1 \tabularnewline
&Ridge with CV (QSI)&.271&.333&.4&.488&.574&.577&0 \tabularnewline
&Random forest (low regularization)&.213&.06&.04&.033&.029&.023&0 \tabularnewline
&Random forest (high regularization)&.026&.005&0&0&0&0&0 \tabularnewline
&Gradient boosting (low regularization)&.004&.008&.02&.015&.015&.025&0 \tabularnewline
&Gradient boosting (high regularization)&.015&.01&.005&.001&0&0&0 \tabularnewline


==> Simul/sim_WZ/psw_y_singlebest_folds2.tex <==
&OLS&.019&.104&.136&.098&.048&.014&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.017&.014&.008&.007&.004&.006&.002 \tabularnewline
&Ridge with CV (TWI)&.094&.059&.056&.057&.06&.042&0 \tabularnewline
&Lasso with CV (QSI)&.22&.322&.4&.407&.391&.371&.762 \tabularnewline
&Ridge with CV (QSI)&.244&.299&.293&.356&.447&.521&.237 \tabularnewline
&Random forest (low regularization)&.367&.16&.076&.048&.029&.023&0 \tabularnewline
&Random forest (high regularization)&.009&.013&.006&.002&0&0&0 \tabularnewline
&Gradient boosting (low regularization)&.008&.007&.009&.014&.017&.02&0 \tabularnewline
&Gradient boosting (high regularization)&.023&.023&.016&.011&.005&.002&0 \tabularnewline


==> Simul/sim_WZ/ssw_d_nnls1_folds10.tex <==
&OLS&.132&.196&.234&.252&.245&.257&.163 \tabularnewline
&Neural net&.04&.041&.038&.036&.031&.029&.038 \tabularnewline
&Lasso with CV (TWI)&.053&.031&.025&.02&.016&.012&.106 \tabularnewline
&Ridge with CV (TWI)&.038&.018&.013&.015&.008&.005&.029 \tabularnewline
&Lasso with CV (QSI)&.173&.225&.25&.248&.25&.228&.413 \tabularnewline
&Ridge with CV (QSI)&.202&.124&.072&.06&.068&.064&0 \tabularnewline
&Random forest (low regularization)&.103&.123&.144&.187&.249&.307&.006 \tabularnewline
&Random forest (high regularization)&.159&.129&.107&.09&.051&.031&.102 \tabularnewline
&Gradient boosting (low regularization)&.043&.046&.054&.047&.045&.041&.144 \tabularnewline
&Gradient boosting (high regularization)&.059&.065&.064&.046&.038&.025&0 \tabularnewline


==> Simul/sim_WZ/ssw_d_nnls1_folds2.tex <==
&OLS&.108&.185&.224&.253&.27&.275&.295 \tabularnewline
&Neural net&.048&.038&.038&.034&.032&.031&.033 \tabularnewline
&Lasso with CV (TWI)&.044&.02&.014&.011&.007&.007&.046 \tabularnewline
&Ridge with CV (TWI)&.063&.031&.015&.012&.01&.008&0 \tabularnewline
&Lasso with CV (QSI)&.131&.17&.223&.248&.27&.265&.356 \tabularnewline
&Ridge with CV (QSI)&.214&.206&.144&.1&.048&.049&0 \tabularnewline
&Random forest (low regularization)&.107&.104&.117&.13&.172&.208&.007 \tabularnewline
&Random forest (high regularization)&.211&.167&.148&.134&.116&.089&.161 \tabularnewline
&Gradient boosting (low regularization)&.031&.032&.035&.04&.038&.039&.101 \tabularnewline
&Gradient boosting (high regularization)&.042&.046&.042&.038&.037&.03&0 \tabularnewline


==> Simul/sim_WZ/ssw_d_singlebest_folds10.tex <==
&OLS&.038&.108&.17&.189&.173&.132&.005 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.058&.032&.017&.011&.005&.003&.002 \tabularnewline
&Ridge with CV (TWI)&.06&.013&.009&.01&.002&.001&0 \tabularnewline
&Lasso with CV (QSI)&.232&.309&.313&.287&.261&.168&.754 \tabularnewline
&Ridge with CV (QSI)&.242&.105&.032&.034&.05&.032&0 \tabularnewline
&Random forest (low regularization)&.079&.028&.011&.008&.004&.003&0 \tabularnewline
&Random forest (high regularization)&.185&.249&.256&.304&.344&.507&0 \tabularnewline
&Gradient boosting (low regularization)&.009&.022&.048&.064&.115&.141&.24 \tabularnewline
&Gradient boosting (high regularization)&.098&.135&.143&.092&.046&.013&0 \tabularnewline


==> Simul/sim_WZ/ssw_d_singlebest_folds2.tex <==
&OLS&.022&.094&.157&.208&.242&.248&.382 \tabularnewline
&Neural net&.001&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.031&.012&.009&.003&.002&.001&.002 \tabularnewline
&Ridge with CV (TWI)&.177&.039&.004&.002&.004&.006&0 \tabularnewline
&Lasso with CV (QSI)&.164&.234&.317&.338&.316&.256&.438 \tabularnewline
&Ridge with CV (QSI)&.257&.268&.13&.053&.009&.025&0 \tabularnewline
&Random forest (low regularization)&.119&.043&.021&.007&.002&0&0 \tabularnewline
&Random forest (high regularization)&.189&.226&.261&.275&.31&.35&.005 \tabularnewline
&Gradient boosting (low regularization)&.001&.003&.005&.012&.031&.059&.173 \tabularnewline
&Gradient boosting (high regularization)&.039&.081&.095&.103&.084&.054&0 \tabularnewline


==> Simul/sim_WZ/ssw_y_nnls1_folds10.tex <==
&OLS&.164&.152&.115&.079&.037&.019&0 \tabularnewline
&Neural net&.047&.045&.048&.067&.098&.05&.076 \tabularnewline
&Lasso with CV (TWI)&.043&.034&.034&.035&.03&.033&.091 \tabularnewline
&Ridge with CV (TWI)&.056&.048&.041&.025&.011&.006&.032 \tabularnewline
&Lasso with CV (QSI)&.252&.274&.266&.264&.271&.297&.639 \tabularnewline
&Ridge with CV (QSI)&.194&.252&.297&.328&.341&.357&.153 \tabularnewline
&Random forest (low regularization)&.095&.097&.113&.131&.161&.2&.01 \tabularnewline
&Random forest (high regularization)&.081&.04&.025&.021&.018&.016&0 \tabularnewline
&Gradient boosting (low regularization)&.041&.04&.049&.041&.03&.021&0 \tabularnewline
&Gradient boosting (high regularization)&.028&.019&.013&.009&.002&.001&0 \tabularnewline


==> Simul/sim_WZ/ssw_y_nnls1_folds2.tex <==
&OLS&.154&.159&.149&.124&.092&.059&0 \tabularnewline
&Neural net&.056&.046&.048&.049&.053&.066&.047 \tabularnewline
&Lasso with CV (TWI)&.041&.034&.03&.026&.027&.026&.092 \tabularnewline
&Ridge with CV (TWI)&.042&.047&.045&.039&.027&.018&.035 \tabularnewline
&Lasso with CV (QSI)&.234&.286&.306&.304&.291&.285&.554 \tabularnewline
&Ridge with CV (QSI)&.207&.212&.229&.275&.32&.347&.249 \tabularnewline
&Random forest (low regularization)&.12&.089&.092&.096&.117&.138&.019 \tabularnewline
&Random forest (high regularization)&.082&.068&.047&.037&.028&.024&.003 \tabularnewline
&Gradient boosting (low regularization)&.037&.039&.039&.036&.036&.03&0 \tabularnewline
&Gradient boosting (high regularization)&.026&.02&.015&.012&.008&.006&0 \tabularnewline


==> Simul/sim_WZ/ssw_y_singlebest_folds10.tex <==
&OLS&.122&.098&.066&.026&.003&.001&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.03&.022&.01&.013&.014&.023&0 \tabularnewline
&Ridge with CV (TWI)&.074&.077&.079&.052&.03&.013&0 \tabularnewline
&Lasso with CV (QSI)&.323&.376&.361&.381&.393&.405&.995 \tabularnewline
&Ridge with CV (QSI)&.239&.314&.379&.428&.478&.479&.005 \tabularnewline
&Random forest (low regularization)&.129&.058&.05&.049&.049&.044&0 \tabularnewline
&Random forest (high regularization)&.022&.005&.001&.001&0&.001&0 \tabularnewline
&Gradient boosting (low regularization)&.025&.033&.046&.046&.032&.034&0 \tabularnewline
&Gradient boosting (high regularization)&.035&.016&.009&.004&0&0&0 \tabularnewline


==> Simul/sim_WZ/ssw_y_singlebest_folds2.tex <==
&OLS&.07&.124&.101&.072&.034&.012&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.015&.014&.013&.009&.009&.011&0 \tabularnewline
&Ridge with CV (TWI)&.067&.058&.067&.063&.054&.039&0 \tabularnewline
&Lasso with CV (QSI)&.282&.383&.43&.424&.394&.38&.808 \tabularnewline
&Ridge with CV (QSI)&.261&.251&.281&.35&.441&.498&.192 \tabularnewline
&Random forest (low regularization)&.238&.111&.06&.042&.036&.033&0 \tabularnewline
&Random forest (high regularization)&.029&.019&.014&.009&.004&.003&0 \tabularnewline
&Gradient boosting (low regularization)&.013&.016&.019&.022&.023&.024&0 \tabularnewline
&Gradient boosting (high regularization)&.025&.024&.015&.009&.005&.001&0 \tabularnewline


==> Simul/sim_WZ/stw_d_nnls1_folds10.tex <==
&OLS&.119&.184&.227&.247&.244&.242&.168 \tabularnewline
&Neural net&.047&.044&.041&.039&.034&.033&.046 \tabularnewline
&Lasso with CV (TWI)&.048&.029&.024&.018&.015&.012&.097 \tabularnewline
&Ridge with CV (TWI)&.05&.021&.013&.014&.011&.008&.001 \tabularnewline
&Lasso with CV (QSI)&.152&.205&.241&.253&.263&.247&.402 \tabularnewline
&Ridge with CV (QSI)&.214&.16&.096&.064&.064&.067&.001 \tabularnewline
&Random forest (low regularization)&.1&.114&.129&.16&.21&.265&.009 \tabularnewline
&Random forest (high regularization)&.181&.144&.124&.114&.076&.054&.121 \tabularnewline
&Gradient boosting (low regularization)&.036&.04&.047&.044&.043&.042&.155 \tabularnewline
&Gradient boosting (high regularization)&.053&.059&.06&.047&.04&.03&.001 \tabularnewline


==> Simul/sim_WZ/stw_d_nnls1_folds2.tex <==
&OLS&.081&.129&.167&.199&.234&.251&.175 \tabularnewline
&Neural net&.056&.044&.046&.043&.041&.039&.05 \tabularnewline
&Lasso with CV (TWI)&.072&.044&.03&.029&.023&.017&.04 \tabularnewline
&Ridge with CV (TWI)&.073&.044&.023&.018&.014&.014&.005 \tabularnewline
&Lasso with CV (QSI)&.128&.155&.198&.218&.248&.247&.389 \tabularnewline
&Ridge with CV (QSI)&.176&.212&.177&.141&.079&.061&.019 \tabularnewline
&Random forest (low regularization)&.105&.097&.108&.112&.137&.165&.013 \tabularnewline
&Random forest (high regularization)&.22&.181&.151&.135&.126&.11&.147 \tabularnewline
&Gradient boosting (low regularization)&.035&.037&.041&.042&.045&.048&.157 \tabularnewline
&Gradient boosting (high regularization)&.053&.056&.058&.062&.054&.046&.005 \tabularnewline


==> Simul/sim_WZ/stw_d_singlebest_folds10.tex <==
&OLS&.03&.102&.161&.198&.193&.164&.087 \tabularnewline
&Neural net&.002&.001&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.046&.024&.016&.01&.004&.003&.006 \tabularnewline
&Ridge with CV (TWI)&.099&.015&.007&.011&.007&.002&0 \tabularnewline
&Lasso with CV (QSI)&.201&.286&.324&.312&.288&.214&.601 \tabularnewline
&Ridge with CV (QSI)&.259&.163&.051&.025&.042&.042&0 \tabularnewline
&Random forest (low regularization)&.092&.036&.015&.01&.004&.003&0 \tabularnewline
&Random forest (high regularization)&.187&.239&.261&.288&.313&.428&.001 \tabularnewline
&Gradient boosting (low regularization)&.005&.012&.026&.04&.079&.115&.305 \tabularnewline
&Gradient boosting (high regularization)&.078&.122&.138&.107&.07&.029&0 \tabularnewline


==> Simul/sim_WZ/stw_d_singlebest_folds2.tex <==
&OLS&.011&.042&.081&.112&.172&.205&.233 \tabularnewline
&Neural net&.007&.002&.001&.001&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.068&.042&.025&.025&.014&.006&0 \tabularnewline
&Ridge with CV (TWI)&.171&.082&.024&.013&.01&.012&0 \tabularnewline
&Lasso with CV (QSI)&.161&.203&.272&.307&.323&.29&.507 \tabularnewline
&Ridge with CV (QSI)&.181&.256&.202&.127&.036&.026&0 \tabularnewline
&Random forest (low regularization)&.156&.08&.05&.027&.011&.007&0 \tabularnewline
&Random forest (high regularization)&.18&.2&.219&.242&.277&.299&.049 \tabularnewline
&Gradient boosting (low regularization)&.005&.006&.011&.016&.029&.056&.211 \tabularnewline
&Gradient boosting (high regularization)&.06&.088&.116&.13&.128&.1&0 \tabularnewline


==> Simul/sim_WZ/stw_y_nnls1_folds10.tex <==
&OLS&.163&.159&.133&.1&.055&.029&0 \tabularnewline
&Neural net&.054&.052&.058&.052&.096&.069&.082 \tabularnewline
&Lasso with CV (TWI)&.044&.034&.034&.032&.028&.03&.059 \tabularnewline
&Ridge with CV (TWI)&.054&.049&.045&.032&.017&.011&.056 \tabularnewline
&Lasso with CV (QSI)&.239&.271&.266&.273&.269&.285&.597 \tabularnewline
&Ridge with CV (QSI)&.19&.235&.271&.316&.337&.358&.187 \tabularnewline
&Random forest (low regularization)&.099&.092&.104&.118&.14&.169&.018 \tabularnewline
&Random forest (high regularization)&.087&.048&.027&.021&.019&.02&0 \tabularnewline
&Gradient boosting (low regularization)&.039&.04&.047&.045&.035&.027&.001 \tabularnewline
&Gradient boosting (high regularization)&.03&.019&.016&.011&.005&.002&0 \tabularnewline


==> Simul/sim_WZ/stw_y_nnls1_folds2.tex <==
&OLS&.129&.161&.168&.154&.124&.094&0 \tabularnewline
&Neural net&.073&.052&.058&.05&.054&.07&.043 \tabularnewline
&Lasso with CV (TWI)&.051&.044&.037&.035&.033&.032&.122 \tabularnewline
&Ridge with CV (TWI)&.059&.052&.051&.048&.039&.029&.007 \tabularnewline
&Lasso with CV (QSI)&.205&.246&.27&.276&.272&.271&.474 \tabularnewline
&Ridge with CV (QSI)&.177&.193&.202&.241&.288&.312&.316 \tabularnewline
&Random forest (low regularization)&.146&.097&.095&.096&.108&.122&.031 \tabularnewline
&Random forest (high regularization)&.078&.083&.056&.04&.024&.02&.005 \tabularnewline
&Gradient boosting (low regularization)&.04&.04&.04&.041&.045&.041&.003 \tabularnewline
&Gradient boosting (high regularization)&.042&.031&.023&.019&.013&.009&0 \tabularnewline


==> Simul/sim_WZ/stw_y_singlebest_folds10.tex <==
&OLS&.108&.123&.087&.045&.012&.002&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.028&.018&.015&.014&.012&.017&0 \tabularnewline
&Ridge with CV (TWI)&.073&.072&.08&.065&.043&.022&0 \tabularnewline
&Lasso with CV (QSI)&.31&.374&.372&.382&.384&.396&.935 \tabularnewline
&Ridge with CV (QSI)&.232&.286&.338&.401&.47&.491&.065 \tabularnewline
&Random forest (low regularization)&.162&.071&.054&.048&.043&.038&0 \tabularnewline
&Random forest (high regularization)&.03&.011&.003&.001&.001&.001&0 \tabularnewline
&Gradient boosting (low regularization)&.02&.025&.037&.038&.035&.034&0 \tabularnewline
&Gradient boosting (high regularization)&.036&.02&.013&.006&.001&0&0 \tabularnewline


==> Simul/sim_WZ/stw_y_singlebest_folds2.tex <==
&OLS&.042&.109&.134&.111&.066&.035&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.034&.029&.021&.02&.015&.015&.003 \tabularnewline
&Ridge with CV (TWI)&.098&.072&.073&.071&.08&.063&0 \tabularnewline
&Lasso with CV (QSI)&.238&.319&.366&.378&.376&.383&.682 \tabularnewline
&Ridge with CV (QSI)&.217&.238&.246&.295&.364&.416&.314 \tabularnewline
&Random forest (low regularization)&.286&.147&.095&.07&.051&.044&0 \tabularnewline
&Random forest (high regularization)&.024&.027&.019&.008&.002&.002&0 \tabularnewline
&Gradient boosting (low regularization)&.019&.022&.021&.027&.035&.037&0 \tabularnewline
&Gradient boosting (high regularization)&.042&.036&.025&.02&.011&.004&0 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_candidate_f10.tex <==
&OLS (TWI)&-1810.9&267&605.1&2.9&-131.9&32.1 \tabularnewline
&OLS (QSI)&-3061.5&7054.9&-770&-7856.9&-1419.2&-6851.3 \tabularnewline
&Lasso with CV (TWI)&5943.6&3195.8&2589.1&1706.2&872.2&734.1 \tabularnewline
&Lasso with CV (QSI)&260.2&-322.1&-311.9&-551.8&-597.1&-239.8 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_candidate_f2.tex <==
&OLS (TWI)&-1133.5&-243.4&-198&-516.4&574.3&359.2 \tabularnewline
&OLS (QSI)&-2675.8&-3137.7&-3563.3&7023&-2604.8&-9974.5 \tabularnewline
&Lasso with CV (TWI)&7184.1&5485.8&3408.9&2998&2509.6&1848 \tabularnewline
&Lasso with CV (QSI)&911.3&191.9&-874.5&-628.5&-207.1&-286.3 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_meta_f10.tex <==
&Short-stacking: CLS&1020&-113.8&-181.1&-538.2&-575.6&-292.4 \tabularnewline
&Short-stacking: Single-best&1002.3&-122.2&-270.1&-499.7&-550.3&-197.7 \tabularnewline
&Pooled stacking: CLS&925.7&-237.3&-319.1&-628.1&-711&-370.5 \tabularnewline
&Pooled stacking: Single-best&782.3&-200.5&-358.9&-541.2&-580.2&-237.5 \tabularnewline
&Stacking: CLS&1155.8&-254.7&-266.9&-645&-633&-315.1 \tabularnewline
&Stacking: Single-best&999.5&-23.6&-184.9&-503.9&-571.1&-248.2 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_meta_f2.tex <==
&Short-stacking: CLS&2186.3&878.7&-463.4&-335.8&-96.4&-207.7 \tabularnewline
&Short-stacking: Single-best&2395.8&611.2&-628.4&-525.6&-187.5&-284.1 \tabularnewline
&Pooled stacking: CLS&1753.2&501.9&-706.5&-487.3&-173.1&-304.2 \tabularnewline
&Pooled stacking: Single-best&2161.3&729.3&-638&-480.8&-150.3&-230.2 \tabularnewline
&Stacking: CLS&1012.5&167.8&-713&-528&-198.9&-264.4 \tabularnewline
&Stacking: Single-best&2010.6&903.1&-573.3&-399.8&-97&-200.3 \tabularnewline


==> Simul/sim_WZ_linear/bias_olspds_f10.tex <==
&OLS QSI&-2113.4&-936.2&-806.4&-809.9&-677.2&-626.5 \tabularnewline
&OLS TWI&-1747.3&-479.9&13.2&-366&-320.3&-91.3 \tabularnewline
&Post double Lasso QSI c=0.5&381.6&-297.1&-204&-503.1&-571.6&-354.1 \tabularnewline
&Post double Lasso QSI c=1&-215.1&-1104.2&-639.4&-1063.2&-1000.5&-523.5 \tabularnewline
&Post double Lasso QSI c=1.5&8040.9&754.4&-1526.2&-2434.4&-2255.4&-1863.5 \tabularnewline
&Post double Lasso TWI c=0.5&3577.5&2490.3&2347.2&1748.3&1270.4&1197.5 \tabularnewline
&Post double Lasso TWI c=1&6270.2&3476.2&3453.1&2523.9&1702.4&1871.8 \tabularnewline
&Post double Lasso TWI c=1.5&14382.3&8943.3&6317.9&4802.2&3939&3094.5 \tabularnewline


==> Simul/sim_WZ_linear/bias_olspds_f2.tex <==
&OLS QSI&-2532.3&-1311.4&-1421.9&-961.6&-399&-282.2 \tabularnewline
&OLS TWI&-2100.3&-448&-936.5&-531.8&23.1&244.7 \tabularnewline
&Post double Lasso QSI c=0.5&-154.7&-120.1&-1019.8&-628.9&-50.5&-161.7 \tabularnewline
&Post double Lasso QSI c=1&-600.6&-1053&-1576.5&-1079&-485.1&-424.9 \tabularnewline
&Post double Lasso QSI c=1.5&7836.3&1064&-2253.4&-2434.8&-1644.7&-1698.3 \tabularnewline
&Post double Lasso TWI c=0.5&2869.2&2790.9&1635.4&1595.6&1767.6&1460.7 \tabularnewline
&Post double Lasso TWI c=1&5189.7&3966.8&2742&2328.1&2174.8&1975.8 \tabularnewline
&Post double Lasso TWI c=1.5&13651.1&9399.4&5610&4277&4150.8&3065.3 \tabularnewline


==> Simul/sim_WZ_linear/fullsample_ddml.tex <==
&OLS (TWI)&6796.682 \tabularnewline
&OLS (QSI)&4853.811 \tabularnewline
&Lasso with CV (TWI)&6780.161 \tabularnewline
&Lasso with CV (QSI)&5722.624 \tabularnewline


==> Simul/sim_WZ_linear/fullsample_meta.tex <==
&Pooled stacking: CLS&6009.779 \tabularnewline
&Pooled stacking: Single-best&5722.624 \tabularnewline
&Short-stacking: CLS&6044.902 \tabularnewline
&Short-stacking: Single-best&5722.396 \tabularnewline
&Stacking: CLS&6014.819 \tabularnewline
&Stacking: Single-best&5719.905 \tabularnewline


==> Simul/sim_WZ_linear/fullsample_olspds.tex <==
&OLS TWI&6751.907 \tabularnewline
&OLS QSI&5988.413 \tabularnewline
&Post double Lasso TWI c=0.5&6562.923 \tabularnewline
&Post double Lasso QSI c=0.5&5648.14 \tabularnewline
&Post double Lasso TWI c=1&6630.751 \tabularnewline
&Post double Lasso QSI c=1&4646.575 \tabularnewline
&Post double Lasso TWI c=1.5&7474.508 \tabularnewline
&Post double Lasso QSI c=1.5&4472.324 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_nnls1_folds10.tex <==
&OLS (TWI)&.002&.058&.055&.062&.069&.08&.111 \tabularnewline
&OLS (QSI)&0&0&0&0&.004&.007&.108 \tabularnewline
&Lasso with CV (TWI)&.264&.153&.125&.109&.11&.116&.234 \tabularnewline
&Lasso with CV (QSI)&.734&.789&.82&.829&.817&.796&.547 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_nnls1_folds2.tex <==
&OLS (TWI)&.016&.001&.061&.051&.05&.06&.091 \tabularnewline
&OLS (QSI)&.001&.038&0&0&0&0&.046 \tabularnewline
&Lasso with CV (TWI)&.376&.24&.165&.154&.124&.111&.167 \tabularnewline
&Lasso with CV (QSI)&.607&.722&.773&.795&.826&.829&.696 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.173&.064&.043&.04&.021&.017&0 \tabularnewline
&Lasso with CV (QSI)&.827&.936&.957&.96&.979&.983&1 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.349&.169&.084&.069&.034&.022&0 \tabularnewline
&Lasso with CV (QSI)&.651&.831&.916&.931&.966&.978&1 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_nnls1_folds10.tex <==
&OLS (TWI)&.007&.054&.075&.074&.078&.081&.031 \tabularnewline
&OLS (QSI)&0&0&0&0&.005&.012&.093 \tabularnewline
&Lasso with CV (TWI)&.248&.208&.209&.193&.177&.164&.19 \tabularnewline
&Lasso with CV (QSI)&.744&.738&.716&.733&.74&.743&.686 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_nnls1_folds2.tex <==
&OLS (TWI)&.035&.001&.046&.053&.072&.079&.083 \tabularnewline
&OLS (QSI)&.005&.004&0&0&0&.001&.043 \tabularnewline
&Lasso with CV (TWI)&.272&.25&.221&.203&.19&.177&.12 \tabularnewline
&Lasso with CV (QSI)&.688&.746&.732&.743&.738&.744&.754 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.157&.092&.088&.074&.059&.053&0 \tabularnewline
&Lasso with CV (QSI)&.843&.908&.912&.926&.941&.947&1 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.233&.165&.121&.094&.084&.075&.002 \tabularnewline
&Lasso with CV (QSI)&.767&.835&.879&.906&.916&.925&.998 \tabularnewline


==> Simul/sim_WZ_linear/ssw_d_nnls1_folds10.tex <==
&OLS (TWI)&.005&.037&.055&.074&.1&.127&.13 \tabularnewline
&OLS (QSI)&0&0&.001&.003&.011&.022&.134 \tabularnewline
&Lasso with CV (TWI)&.264&.163&.137&.119&.114&.111&.232 \tabularnewline
&Lasso with CV (QSI)&.731&.8&.807&.803&.775&.74&.504 \tabularnewline


==> Simul/sim_WZ_linear/ssw_d_nnls1_folds2.tex <==
&OLS (TWI)&.007&.007&.023&.035&.06&.079&.112 \tabularnewline
&OLS (QSI)&0&0&0&0&.001&.004&.069 \tabularnewline
&Lasso with CV (TWI)&.323&.203&.155&.136&.116&.104&.194 \tabularnewline
&Lasso with CV (QSI)&.67&.79&.822&.829&.823&.813&.625 \tabularnewline


==> Simul/sim_WZ_linear/ssw_d_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.239&.126&.098&.079&.06&.068&.003 \tabularnewline
&Lasso with CV (QSI)&.761&.874&.902&.921&.94&.932&.997 \tabularnewline


==> Simul/sim_WZ_linear/ssw_d_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.289&.139&.084&.07&.039&.03&.006 \tabularnewline
&Lasso with CV (QSI)&.711&.861&.916&.93&.961&.97&.994 \tabularnewline


==> Simul/sim_WZ_linear/ssw_y_nnls1_folds10.tex <==
&OLS (TWI)&.01&.042&.062&.078&.098&.113&.013 \tabularnewline
&OLS (QSI)&0&0&.002&.008&.023&.032&.128 \tabularnewline
&Lasso with CV (TWI)&.249&.2&.196&.171&.158&.14&.214 \tabularnewline
&Lasso with CV (QSI)&.74&.758&.74&.742&.721&.716&.645 \tabularnewline


==> Simul/sim_WZ_linear/ssw_y_nnls1_folds2.tex <==
&OLS (TWI)&.011&.015&.032&.044&.065&.079&.085 \tabularnewline
&OLS (QSI)&.001&0&0&0&.003&.008&.061 \tabularnewline
&Lasso with CV (TWI)&.255&.228&.212&.188&.172&.159&.118 \tabularnewline
&Lasso with CV (QSI)&.732&.757&.756&.768&.759&.754&.736 \tabularnewline


==> Simul/sim_WZ_linear/ssw_y_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&.001&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.186&.141&.128&.112&.09&.081&0 \tabularnewline
&Lasso with CV (QSI)&.814&.859&.872&.888&.909&.919&1 \tabularnewline


==> Simul/sim_WZ_linear/ssw_y_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.215&.149&.127&.107&.095&.084&0 \tabularnewline
&Lasso with CV (QSI)&.785&.851&.873&.893&.905&.916&1 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_nnls1_folds10.tex <==
&OLS (TWI)&.005&.051&.049&.062&.081&.104&.121 \tabularnewline
&OLS (QSI)&0&0&0&.001&.005&.012&.107 \tabularnewline
&Lasso with CV (TWI)&.285&.178&.146&.128&.114&.111&.225 \tabularnewline
&Lasso with CV (QSI)&.709&.771&.804&.81&.799&.773&.548 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_nnls1_folds2.tex <==
&OLS (TWI)&.025&.001&.054&.047&.053&.064&.096 \tabularnewline
&OLS (QSI)&.003&.024&0&0&0&.001&.051 \tabularnewline
&Lasso with CV (TWI)&.381&.267&.19&.175&.144&.127&.16 \tabularnewline
&Lasso with CV (QSI)&.592&.708&.756&.778&.803&.807&.693 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.256&.135&.097&.075&.056&.05&.025 \tabularnewline
&Lasso with CV (QSI)&.744&.865&.903&.924&.944&.95&.975 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.385&.24&.152&.132&.094&.072&.022 \tabularnewline
&Lasso with CV (QSI)&.615&.76&.848&.868&.906&.928&.978 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_nnls1_folds10.tex <==
&OLS (TWI)&.012&.055&.07&.079&.086&.098&.052 \tabularnewline
&OLS (QSI)&0&0&0&.002&.012&.021&.1 \tabularnewline
&Lasso with CV (TWI)&.255&.212&.208&.183&.164&.149&.165 \tabularnewline
&Lasso with CV (QSI)&.733&.734&.722&.737&.737&.732&.683 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_nnls1_folds2.tex <==
&OLS (TWI)&.044&.003&.048&.057&.074&.08&.085 \tabularnewline
&OLS (QSI)&.009&.003&0&0&0&.003&.055 \tabularnewline
&Lasso with CV (TWI)&.277&.259&.23&.211&.199&.182&.131 \tabularnewline
&Lasso with CV (QSI)&.67&.735&.722&.732&.726&.735&.729 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&.001&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.209&.146&.136&.113&.095&.084&0 \tabularnewline
&Lasso with CV (QSI)&.791&.854&.864&.886&.904&.916&1 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&.001&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.27&.207&.167&.142&.131&.113&.005 \tabularnewline
&Lasso with CV (QSI)&.73&.793&.833&.858&.868&.886&.995 \tabularnewline


==> Text_as_data/mspe.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Wed Aug 23 18:04:57 2023
id & coded.x & coded.y & text.x & text.y \\ 
 SS CLS & 2169.476 & 0.067 & 2170.251 & 0.095 \\ 
  SS SB & 2194.020 & 0.067 & 2223.633 & 0.096 \\ 
  CV-lasso & 2237.376 & 0.076 & 2293.658 & 0.097 \\ 
  CV-Ridge & 2225.681 & 0.076 & 2829.188 & 0.099 \\ 
  XGBoost 1 & 2206.927 & 0.067 & 2343.072 & 0.096 \\ 
  XGBoost 2 & 2194.101 & 0.068 & 2315.487 & 0.102 \\ 
  XGBoost 3 & 2341.143 & 0.073 & 2322.874 & 0.109 \\ 
  XGBoost 4 & 2467.231 & 0.070 & 2249.085 & 0.099 \\ 
  XGBoost 5 & 3029.791 & 0.085 & 2223.633 & 0.107 \\ 
  XGBoost 6 & 3895.228 & 0.110 & 2276.479 & 0.109 \\ 
  Neural net 1 & 2767.599 & 0.142 & 3169.797 & 0.366 \\ 
  Neural net 2 & 2766.972 & 0.158 & 3145.763 & 0.385 \\ 
  Neural net 3 & 2744.836 & 0.103 & 3152.201 & 0.211 \\ 
  

==> Text_as_data/regression_results.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Wed Aug 23 17:54:25 2023
gap1 & estimator & Hand-coded & Only text \\ 
  & OLS & -7.527 &  \\ 
   &  & (2.326)* &  \\ 
   & One-step lasso & -7.53 & -6.44 \\ 
   &  & (2.324)* & (1.981)* \\ 
   & PDS lasso & -7.65 & -7.94 \\ 
   &  & (2.242)* & (2.117)* \\ 
   & Lasso & -7.513 & -7.225 \\ 
   &  & (3.385)* & (3.097)* \\ 
   & Ridge & -7.558 & -6.965 \\ 
   &  & (3.379)* & (3.444)* \\ 
   & XGBoost 1 & -6.771 & -7.032 \\ 
   &  & (3.609)* & (3.146)* \\ 
   & XGBoost 2 & -5.867 & -6.044 \\ 
   &  & (3.576) & (3.126)* \\ 
   & XGBoost 3 & -4.743 & -5.457 \\ 
   &  & (3.582) & (3.229)* \\ 
   & XGBoost 4 & -3.995 & -5.824 \\ 
   &  & (3.751) & (3.107)* \\ 
   & XGBoost 5 & -1.386 & -4.918 \\ 
   &  & (3.882) & (3.112) \\ 
   & XGBoost 6 & -0.222 & -5.802 \\ 
   &  & (4.222) & (3.294)* \\ 
   & Neural net 1 & -5.645 & -2.632 \\ 
   &  & (2.982)* & (4.269) \\ 
   & Neural net 2 & -6.079 & -1.773 \\ 
   &  & (4.043) & (5.484) \\ 
   & Neural net 3 & -6.353 & -4.664 \\ 
   &  & (3.19)* & (3.413) \\ 
   & Short-stacking:
Single-best & -6.644 & -6.323 \\ 
   &  & (3.616)* & (3.125)* \\ 
   & Short-stacking:
CLS & -6.323 & -6.869 \\ 
   &  & (3.57)* & (3.005)* \\ 
   & Stacking:
Single-best & -6.62 & -6.792 \\ 
   &  & (3.62)* & (3.034)* \\ 
   & Stacking:
CLS & -6.399 & -6.975 \\ 
   &  & (3.593)* & (3.009)* \\ 
  

==> Text_as_data/weights.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Wed Aug 23 17:54:26 2023
did & yreg\_coded & dreg\_coded & gap1 & yss\_coded & dss\_coded & gap2 & yreg\_text & dreg\_text & gap3 & yss\_text & dss\_text \\ 
 Lasso & 0.000 & 0.001 &  & 0.000 & 0.000 &  & 0.443 & 0.530 &  & 0.353 & 0.492 \\ 
  Ridge & 0.407 & 0.000 &  & 0.333 & 0.000 &  & 0.005 & 0.099 &  & 0.000 & 0.009 \\ 
  XGBoost 1 & 0.179 & 0.891 &  & 0.088 & 0.901 &  & 0.000 & 0.124 &  & 0.000 & 0.232 \\ 
  XGBoost 2 & 0.226 & 0.000 &  & 0.422 & 0.000 &  & 0.009 & 0.064 &  & 0.003 & 0.017 \\ 
  XGBoost 3 & 0.081 & 0.002 &  & 0.043 & 0.000 &  & 0.198 & 0.079 &  & 0.148 & 0.135 \\ 
  XGBoost 4 & 0.024 & 0.103 &  & 0.081 & 0.097 &  & 0.001 & 0.022 &  & 0.000 & 0.000 \\ 
  XGBoost 5 & 0.006 & 0.001 &  & 0.004 & 0.000 &  & 0.220 & 0.022 &  & 0.350 & 0.019 \\ 
  XGBoost 6 & 0.019 & 0.002 &  & 0.000 & 0.000 &  & 0.119 & 0.038 &  & 0.146 & 0.062 \\ 
  Neural net 1 & 0.026 & 0.000 &  & 0.013 & 0.001 &  & 0.002 & 0.002 &  & 0.000 & 0.000 \\ 
  Neural net 2 & 0.021 & 0.000 &  & 0.000 & 0.001 &  & 0.001 & 0.009 &  & 0.000 & 0.032 \\ 
  Neural net 3 & 0.011 & 0.000 &  & 0.015 & 0.000 &  & 0.002 & 0.012 &  & 0.000 & 0.001 \\ 
  

==> partialinput.tex <==
\makeatletter
\newread\pin@file
\newcounter{pinlineno}
\newcommand\pin@accu{}
\newcommand\pin@ext{pintmp}
% inputs #3, selecting only lines #1 to #2 (inclusive)
\newcommand*\partialinput [3] {%
\IfFileExists{#3}{%
\openin\pin@file #3%
% skip lines 1 to #1 (exclusive)
\setcounter{pinlineno}{1}%
\@whilenum\value{pinlineno}<#1 \do{%
\read\pin@file to\pin@line%
\stepcounter{pinlineno}%
}%
% prepare reading lines #1 to #2 inclusive
\addtocounter{pinlineno}{-1}%
\let\pin@accu\empty%
\begingroup%
\endlinechar\newlinechar
\@whilenum\value{pinlineno}<#2 \do{%
% use safe catcodes provided by e-TeX's \readline
\readline\pin@file to\pin@line%
\edef\pin@accu{\pin@accu\pin@line}%
\stepcounter{pinlineno}%
}%
\closein\pin@file%
\expandafter\endgroup%
\scantokens\expandafter{\pin@accu}%
}{%
\errmessage{File `#3' doesn't exist!}%
}%
}
\makeatother

==> scopus_cites/mspe_levels.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 16:55:33 2023
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 57744.2 & 57599.8 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & OLS \& BERT &  & 58321.1 & 57823.5 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-lasso \& Unigrams &  & 57614.9 & 57496.1 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-lasso \& BERT &  & 56856.1 & 56686.6 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-ridge \& Unigrams &  & 57639.6 & 57530.2 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-ridge \& BERT &  & 56749.1 & 56629.3 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & XGBoost \& Unigrams &  & 67792.\phantom{0} & 67486.1 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & XGBoost \& BERT &  & 67465.8 & 67236.3 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Random forest \& Unigrams &  & 58356.4 & 58208.6 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Random forest \& BERT &  & 61190.5 & 61098.9 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Neural net \& Unigrams &  & 67554.8 & 65769.7 &  & 238.4 & 0.9 &  & 8.2 & 0.2 \\ 
   & Neural net \& BERT &  & 69864.2 & 69781.3 &  &   0.1 & 0.1 &  & 0.2 & 0.2 \\ 
  

==> scopus_cites/mspe_log.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 16:55:33 2023
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 1.335 & 1.332 &  & 0.058 & 0.058 &  & 0.169 & 0.169 \\ 
   & OLS \& BERT &  & 1.287 & 1.274 &  & 0.058 & 0.057 &  & 0.168 & 0.167 \\ 
   & CV-lasso \& Unigrams &  & 1.334 & 1.331 &  & 0.057 & 0.057 &  & 0.168 & 0.168 \\ 
   & CV-lasso \& BERT &  & 1.268 & 1.262 &  & 0.056 & 0.056 &  & 0.164 & 0.164 \\ 
   & CV-ridge \& Unigrams &  & 1.335 & 1.332 &  & 0.057 & 0.057 &  & 0.168 & 0.168 \\ 
   & CV-ridge \& BERT &  & 1.276 & 1.274 &  & 0.056 & 0.056 &  & 0.164 & 0.164 \\ 
   & XGBoost \& Unigrams &  & 1.428 & 1.397 &  & 0.074 & 0.072 &  & 0.198 & 0.194 \\ 
   & XGBoost \& BERT &  & 1.517 & 1.496 &  & 0.068 & 0.068 &  & 0.196 & 0.194 \\ 
   & Random forest \& Unigrams &  & 1.347 & 1.335 &  & 0.059 & 0.059 &  & 0.17\phantom{0} & 0.17\phantom{0} \\ 
   & Random forest \& BERT &  & 1.629 & 1.613 &  & 0.059 & 0.059 &  & 0.172 & 0.172 \\ 
   & Neural net \& Unigrams &  & 4.269 & 3.304 &  & 0.149 & 0.058 &  & 1.424 & 3.805 \\ 
   & Neural net \& BERT &  & 5.576 & 5.292 &  & 0.058 & 0.058 &  & 0.184 & 0.184 \\ 
  

==> scopus_cites/mspe_log_joined.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 16:55:33 2023
gap0 & learner & gap1 & y_X_Conventional & gap2 & D1_X_Conventional & gap3 & D2_X_Conventional \\ 
  & OLS \& Unigrams &  & \multicolumn{2}{c}{1.335} &  & \multicolumn{2}{c}{0.058} &  & \multicolumn{2}{c}{0.169} \\ 
   & OLS \& BERT &  & \multicolumn{2}{c}{1.287} &  & \multicolumn{2}{c}{0.058} &  & \multicolumn{2}{c}{0.168} \\ 
   & CV-lasso \& Unigrams &  & \multicolumn{2}{c}{1.334} &  & \multicolumn{2}{c}{0.057} &  & \multicolumn{2}{c}{0.168} \\ 
   & CV-lasso \& BERT &  & \multicolumn{2}{c}{1.268} &  & \multicolumn{2}{c}{0.056} &  & \multicolumn{2}{c}{0.164} \\ 
   & CV-ridge \& Unigrams &  & \multicolumn{2}{c}{1.335} &  & \multicolumn{2}{c}{0.057} &  & \multicolumn{2}{c}{0.168} \\ 
   & CV-ridge \& BERT &  & \multicolumn{2}{c}{1.276} &  & \multicolumn{2}{c}{0.056} &  & \multicolumn{2}{c}{0.164} \\ 
   & XGBoost \& Unigrams &  & \multicolumn{2}{c}{1.428} &  & \multicolumn{2}{c}{0.074} &  & \multicolumn{2}{c}{0.198} \\ 
   & XGBoost \& BERT &  & \multicolumn{2}{c}{1.517} &  & \multicolumn{2}{c}{0.068} &  & \multicolumn{2}{c}{0.196} \\ 
   & Random forest \& Unigrams &  & \multicolumn{2}{c}{1.347} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.17\phantom{0}} \\ 
   & Random forest \& BERT &  & \multicolumn{2}{c}{1.629} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.172} \\ 
   & Neural net \& Unigrams &  & \multicolumn{2}{c}{4.269} &  & \multicolumn{2}{c}{0.149} &  & \multicolumn{2}{c}{1.424} \\ 
   & Neural net \& BERT &  & \multicolumn{2}{c}{5.576} &  & \multicolumn{2}{c}{0.058} &  & \multicolumn{2}{c}{0.184} \\ 
  

==> scopus_cites/results_tab.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 16:55:33 2023
 OLS \& base controls & 0.007 & 0.212* & -9.839** & 11.368* \\ 
   & (0.029) & (0.017) & (4.299) & (2.889) \\ 
  PDS-lasso \& base controls & 0.009 & 0.214* & -9.608** & 11.558* \\ 
   & (0.029) & (0.017) & (4.293) & (2.886) \\ 
  PDS-lasso \& Unigrams & -0.069** & 0.097* & -15.77* & 2.809 \\ 
   & (0.028) & (0.016) & (4.141) & (2.896) \\ 
  PDS-lasso \& BERT & -0.081* & 0.086* & -14.634* & 2.459 \\ 
   & (0.028) & (0.016) & (4.236) & (2.89) \\ 
  OLS \& Unigrams & -0.062** & 0.094* & -12.227** & 2.464 \\ 
   & (0.029) & (0.017) & (5.957) & (3.48) \\ 
  OLS \& BERT & -0.082* & 0.061* & -10.43** & 1.58 \\ 
   & (0.029) & (0.017) & (5.968) & (3.608) \\ 
  CV-lasso \& Unigrams & -0.061** & 0.093* & -12.512** & 2.359 \\ 
   & (0.029) & (0.017) & (5.948) & (3.477) \\ 
  CV-lasso \& BERT & -0.077* & 0.063* & -10.055** & 2.054 \\ 
   & (0.029) & (0.017) & (5.967) & (3.495) \\ 
  CV-ridge \& Unigrams & -0.062** & 0.093* & -12.398** & 1.859 \\ 
   & (0.029) & (0.017) & (5.947) & (3.479) \\ 
  CV-ridge \& BERT & -0.074* & 0.066* & -10.108** & 1.893 \\ 
   & (0.029) & (0.017) & (5.961) & (3.499) \\ 
  XGBoost \& Unigrams & -0.087* & 0.058* & 32.376* & 19.504* \\ 
   & (0.029) & (0.018) & (6.153) & (3.622) \\ 
  XGBoost \& BERT & -0.075** & 0.053* & 7.336 & 7.883** \\ 
   & (0.031) & (0.018) & (7.049) & (3.894) \\ 
  Random forest \& Unigrams & -0.11* & 0.034** & 0.037 & 4.672 \\ 
   & (0.029) & (0.017) & (5.912) & (3.469) \\ 
  Random forest \& BERT & -0.134* & 0.002 & 6.671 & 6.319** \\ 
   & (0.032) & (0.018) & (6.025) & (3.53) \\ 
  Neural net \& Unigrams & -0.042 & -0.029 & -15.544 & -11.383** \\ 
   & (0.043) & (0.057) & (10.062) & (5.62) \\ 
  Neural net \& BERT & -0.061 & -0.044 & -17.923* & -11.332* \\ 
   & (0.08) & (0.143) & (6.154) & (3.682) \\ 
  Single-best \& stacking & -0.077* & 0.064* & -10.177** & 1.981 \\ 
   & (0.028) & (0.017) & (5.969) & (3.512) \\ 
  CLS \& stacking & -0.077* & 0.057* & -13.085** & -2.618 \\ 
   & (0.028) & (0.016) & (5.978) & (3.454) \\ 
  Single-best \& short-stacking & -0.076* & 0.063* & -10.108** & 1.893 \\ 
   & (0.029) & (0.017) & (5.961) & (3.499) \\ 
  CLS \& short-stacking & -0.075* & 0.054* & -9.556 & 1.507 \\ 
   & (0.028) & (0.016) & (5.933) & (3.492) \\ 
  

==> scopus_cites/weights_levels.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 16:55:33 2023
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 0.128 & 0.206 &  & 0.018 & 0.139 &  & 0.005 & 0.103 \\ 
   & OLS \& BERT &  & 0.132 & 0.213 &  & 0.064 & 0.106 &  & 0.15\phantom{0} & 0.202 \\ 
   & CV-lasso \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.008 &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-lasso \& BERT &  & 0.075 & 0.243 &  & 0.132 & 0.224 &  & 0.055 & 0.279 \\ 
   & CV-ridge \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-ridge \& BERT &  & 0.054 & 0.108 &  & 0.117 & 0.48\phantom{0} &  & 0.081 & 0.228 \\ 
   & XGBoost \& Unigrams &  & 0.054 & 0.071 &  & 0.014 & 0.022 &  & 0.035 & 0.028 \\ 
   & XGBoost \& BERT &  & 0.036 & 0.032 &  & 0.004 & 0.019 &  & 0.02\phantom{0} & 0.019 \\ 
   & Random forest \& Unigrams &  & 0.\phantom{000} & 0.166 &  & 0.\phantom{000} & 0.022 &  & 0.\phantom{000} & 0.159 \\ 
   & Random forest \& BERT &  & 0.083 & 0.\phantom{000} &  & 0.16\phantom{0} & 0.\phantom{000} &  & 0.028 & 0.\phantom{000} \\ 
   & Neural net \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.013 & 0.\phantom{000} &  & 0.15\phantom{0} & 0.\phantom{000} \\ 
   & Neural net \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.001 & 0.\phantom{000} &  & 0.059 & 0.\phantom{000} \\ 
  

==> scopus_cites/weights_log.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 16:55:33 2023
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 0.109 & 0.053 &  & 0.026 & 0.158 &  & 0.004 & 0.128 \\ 
   & OLS \& BERT &  & 0.307 & 0.389 &  & 0.063 & 0.105 &  & 0.153 & 0.216 \\ 
   & CV-lasso \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-lasso \& BERT &  & 0.207 & 0.142 &  & 0.138 & 0.336 &  & 0.079 & 0.28\phantom{0} \\ 
   & CV-ridge \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-ridge \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.118 & 0.378 &  & 0.066 & 0.192 \\ 
   & XGBoost \& Unigrams &  & 0.212 & 0.256 &  & 0.011 & 0.002 &  & 0.039 & 0.026 \\ 
   & XGBoost \& BERT &  & 0.052 & 0.07\phantom{0} &  & 0.005 & 0.015 &  & 0.016 & 0.036 \\ 
   & Random forest \& Unigrams &  & 0.037 & 0.093 &  & 0.\phantom{000} & 0.024 &  & 0.\phantom{000} & 0.139 \\ 
   & Random forest \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.164 & 0.\phantom{000} &  & 0.022 & 0.\phantom{000} \\ 
   & Neural net \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.081 & 0.\phantom{000} \\ 
   & Neural net \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.124 & 0.\phantom{000} \\ 
  
